How Developers Adopt, Use, and Evolve CI/CD Caching: An Empirical Study on GitHub Actions

Continuous Integration/Continuous Delivery (CI/CD) caching is widely used to reduce repeated computation and improve CI/CD efficiency, yet maintaining effective caching requires ongoing maintenance effort. In this paper, we present the first empirical study on how developers configure and evolve caching in CI/CD workflows on GitHub Actions. We analyze 952 GitHub repositories (266 cache adopters and 686 non-adopters), to compare repository characteristics, characterize caching usage at the job and step levels, uncover patterns in caching configuration evolution, and identify the drivers of cache-related changes. Our analysis spans 1,556 workflow files, 10,373 commits, and 17,185 workflow configuration changes, including an average of 9.37 cache-related changes per repository. Our main observations are: (1) cache-adopting repositories are more active and popular than non-adopters; (2) caching is used across multiple CI/CD job types through a variety of caching mechanisms rather than a single standardized approach; (3) caching configurations evolve through frequent, repetitive maintenance patterns, with rapid updates in build and test jobs and slower evolution in other job types; and (4) cache-related modifications are driven by distinct maintenance needs: parameter updates are mainly human-driven to fix issues, while version updates occur later and are often bot-driven for dependency maintenance. Our findings quantify the substantial maintenance effort involved in CI/CD caching and highlight opportunities to improve reliability and tool support.

==> appen_old.tex <==


\begin{table}[h]
\centering
\caption{Build-phase transition statistics (days). Abbreviations: P\_up = Parameter update, P\_add = Parameter added, P\_rm = Parameter removed, C\_up = Cache update, C\_add = Cache added, C\_rm = Cache removed, EC = Enable cache. \textbf{Rows are grouped (clustered) by the source state (left-hand side of the transition), and sorted within each cluster (not globally across the whole table).}}
\label{tab:build_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba} & \textbf{Proba (\%)} \\ \hline

\multicolumn{10}{|c|}{\textbf{Cluster 1}} \\ \hline
T1  & C\_add $\rightarrow$ C\_add           & 26  & 28.03  & 0.00   & 0.00  & 462.91  & 93.91  & 0.35 & 34.67\% \\ \hline
T2  & C\_add $\rightarrow$ C\_rm            & 19  & 112.31 & 0.00   & 0.00  & 750.21  & 219.41 & 0.25 & 25.33\% \\ \hline
T3  & C\_add $\rightarrow$ P\_up            & 16  & 106.70 & 51.16  & 0.05  & 419.07  & 132.88 & 0.21 & 21.33\% \\ \hline
T4  & C\_add $\rightarrow$ C\_up            & 14  & 373.24 & 309.69 & 0.00  & 1080.84 & 342.69 & 0.19 & 18.67\% \\ \hline

\multicolumn{10}{|c|}{\textbf{Cluster 2}} \\ \hline
T5  & P\_add $\rightarrow$ C\_up            & 3   & 59.94  & 0.00   & 0.00  & 179.82  & 103.82 & 0.43 & 42.86\% \\ \hline
T6  & P\_add $\rightarrow$ P\_up            & 2   & 3.16   & 3.16   & 0.00  & 6.31    & 4.46   & 0.29 & 28.57\% \\ \hline
T7  & P\_add $\rightarrow$ P\_add           & 1   & 0.00   & 0.00   & 0.00  & 0.00    & --     & 0.14 & 14.29\% \\ \hline
T8  & P\_add $\rightarrow$ P\_rm            & 1   & 0.00   & 0.00   & 0.00  & 0.00    & --     & 0.14 & 14.29\% \\ \hline

\multicolumn{10}{|c|}{\textbf{Cluster 3}} \\ \hline
T9  & C\_up $\rightarrow$ C\_up             & 177 & 59.56  & 0.00   & 0.00  & 668.08  & 138.32 & 0.78 & 77.63\% \\ \hline
T10 & C\_up $\rightarrow$ P\_up             & 27  & 148.09 & 79.07  & 0.00  & 592.69  & 179.24 & 0.12 & 11.84\% \\ \hline
T11 & C\_up $\rightarrow$ C\_rm             & 18  & 270.58 & 328.70 & 0.00  & 707.67  & 225.37 & 0.08 & 7.89\% \\ \hline

\multicolumn{10}{|c|}{\textbf{Cluster 4}} \\ \hline
T12 & EC $\rightarrow$ C\_up                & 69  & 637.14 & 587.98 & 6.35  & 1615.93 & 448.74 & 0.29 & 29.49\% \\ \hline
T13 & EC $\rightarrow$ EC                   & 62  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.26 & 26.50\% \\ \hline
T14 & EC $\rightarrow$ P\_up                & 40  & 173.07 & 105.93 & 0.00  & 874.04  & 221.14 & 0.17 & 17.09\% \\ \hline
T15 & EC $\rightarrow$ C\_rm                & 39  & 422.58 & 343.82 & 0.00  & 1514.81 & 428.02 & 0.17 & 16.67\% \\ \hline
T16 & EC $\rightarrow$ C\_add               & 21  & 153.44 & 53.14  & 0.00  & 504.87  & 177.26 & 0.09 & 8.97\% \\ \hline

\multicolumn{10}{|c|}{\textbf{Cluster 5}} \\ \hline
T17 & C\_rm $\rightarrow$ C\_rm             & 48  & 13.73  & 0.00   & 0.00  & 390.89  & 66.32  & 0.55 & 55.17\% \\ \hline
T18 & C\_rm $\rightarrow$ C\_add            & 19  & 47.11  & 0.01   & 0.00  & 445.13  & 105.93 & 0.22 & 21.84\% \\ \hline
T19 & C\_rm $\rightarrow$ P\_up             & 9   & 55.79  & 30.82  & 0.00  & 321.98  & 101.96 & 0.10 & 10.34\% \\ \hline
T20 & C\_rm $\rightarrow$ C\_up             & 7   & 220.73 & 0.00   & 0.00  & 1374.41 & 510.42 & 0.08 & 8.05\% \\ \hline

\multicolumn{10}{|c|}{\textbf{Cluster 6}} \\ \hline
T21 & P\_rm $\rightarrow$ C\_rm             & 2   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.50 & 50.00\% \\ \hline
T22 & P\_rm $\rightarrow$ P\_up             & 2   & 117.53 & 117.53 & 0.00  & 235.06  & 166.21 & 0.50 & 50.00\% \\ \hline

\multicolumn{10}{|c|}{\textbf{Cluster 7}} \\ \hline
T23 & P\_up $\rightarrow$ P\_up             & 135 & 45.40  & 4.08   & 0.00  & 941.90  & 105.61 & 0.66 & 65.53\% \\ \hline
T24 & P\_up $\rightarrow$ C\_up             & 31  & 173.03 & 104.80 & 0.00  & 1366.00 & 277.52 & 0.15 & 15.05\% \\ \hline
T25 & P\_up $\rightarrow$ C\_rm             & 24  & 152.99 & 43.29  & 0.00  & 902.66  & 222.58 & 0.12 & 11.65\% \\ \hline
T26 & P\_up $\rightarrow$ C\_add            & 11  & 25.17  & 4.73   & 1.74  & 177.96  & 52.00  & 0.05 & 5.34\%  \\ \hline

\end{tabular}}
\end{table}


\begin{table}[h]
\centering
\caption{Transitions of states in the test phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache).}
\label{tab:test_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 142 & 62.75  & 2.93   & 0.00  & 986.95  & 156.46 & 0.66  & 66.05 \\ \hline
T2  & C\_up $\rightarrow$ C\_up             & 114 & 58.67  & 0.00   & 0.00  & 713.59  & 137.94 & 0.68  & 68.26 \\ \hline
T3  & C\_add $\rightarrow$ C\_add           & 48  & 24.83  & 0.00   & 0.00  & 463.22  & 93.51  & 0.36  & 36.09 \\ \hline
T4  & EC $\rightarrow$ P\_up                & 45  & 263.33 & 85.03  & 0.00  & 981.44  & 347.74 & 0.24  & 24.32 \\ \hline
T5  & C\_rm $\rightarrow$ C\_rm             & 44  & 39.12  & 0.00   & 0.00  & 448.01  & 105.53 & 0.42  & 41.51 \\ \hline
T6  & C\_add $\rightarrow$ C\_rm            & 42  & 112.53 & 32.49  & 0.00  & 485.66  & 152.93 & 0.32  & 31.58 \\ \hline
T7  & EC $\rightarrow$ C\_up                & 41  & 515.49 & 351.05 & 0.20  & 1549.93 & 457.35 & 0.22  & 22.16 \\ \hline
T8  & EC $\rightarrow$ EC                   & 38  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.21  & 20.54 \\ \hline
T9  & C\_up $\rightarrow$ P\_up             & 33  & 76.46  & 0.00   & 0.00  & 433.71  & 120.17 & 0.20  & 19.76 \\ \hline
T10 & C\_rm $\rightarrow$ C\_add            & 32  & 21.35  & 0.00   & 0.00  & 445.13  & 80.79  & 0.30  & 30.19 \\ \hline
T11 & P\_up $\rightarrow$ C\_up             & 31  & 111.24 & 31.50  & 0.00  & 584.03  & 152.83 & 0.14  & 14.42 \\ \hline
T12 & EC $\rightarrow$ C\_rm                & 30  & 243.13 & 120.77 & 0.00  & 1271.64 & 304.07 & 0.16  & 16.22 \\ \hline
T13 & EC $\rightarrow$ C\_add               & 29  & 172.12 & 41.97  & 0.01  & 962.46  & 243.45 & 0.16  & 15.68 \\ \hline
T14 & C\_add $\rightarrow$ P\_up            & 21  & 105.59 & 8.47   & 0.00  & 973.79  & 219.12 & 0.16  & 15.79 \\ \hline
T15 & P\_up $\rightarrow$ C\_rm             & 19  & 221.16 & 7.24   & 0.00  & 1154.81 & 393.51 & 0.09  & 8.84  \\ \hline
T16 & P\_up $\rightarrow$ C\_add            & 16  & 64.67  & 43.66  & 0.00  & 323.27  & 85.87  & 0.07  & 7.44  \\ \hline
T17 & C\_add $\rightarrow$ C\_up            & 15  & 340.95 & 231.83 & 0.01  & 1294.85 & 356.57 & 0.11  & 11.28 \\ \hline
T18 & C\_up $\rightarrow$ C\_rm             & 12  & 150.41 & 94.56  & 0.00  & 435.59  & 148.67 & 0.07  & 7.19  \\ \hline
T19 & C\_rm $\rightarrow$ P\_rm             & 10  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.09  & 9.43  \\ \hline
T20 & C\_rm $\rightarrow$ P\_up             & 9   & 85.85  & 13.21  & 0.00  & 584.88  & 189.00 & 0.08  & 8.49  \\ \hline
T21 & P\_rm $\rightarrow$ C\_add            & 8   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.62  & 61.54 \\ \hline
T22 & C\_rm $\rightarrow$ C\_up             & 8   & 265.57 & 269.97 & 0.00  & 557.51  & 180.03 & 0.08  & 7.55  \\ \hline
T23 & C\_add $\rightarrow$ P\_add           & 7   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.05  & 5.26  \\ \hline
T24 & P\_add $\rightarrow$ C\_add           & 5   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.28  & 27.78 \\ \hline
T25 & P\_add $\rightarrow$ P\_up            & 5   & 186.87 & 140.78 & 0.00  & 628.32  & 257.22 & 0.28  & 27.78 \\ \hline
T26 & P\_rm $\rightarrow$ C\_rm             & 3   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.23  & 23.08 \\ \hline
T27 & P\_add $\rightarrow$ P\_add           & 3   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.17  & 16.67 \\ \hline
T28 & P\_add $\rightarrow$ C\_up            & 3   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.17  & 16.67 \\ \hline
T29 & P\_rm $\rightarrow$ C\_up             & 2   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.15  & 15.38 \\ \hline
T30 & P\_add $\rightarrow$ C\_rm            & 1   & 875.94 & 875.94 & 875.94& 875.94  & -      & 0.06  & 5.56  \\ \hline
T31 & P\_add $\rightarrow$ EC               & 1   & 0.00   & 0.00   & 0.00  & 0.00    & -      & 0.06  & 5.56  \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Transitions of states of integration phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:integration_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 25 & 137.45 & 87.25  & 13.03 & 538.19 & 124.44 & 67.57 \\ \hline
T2  & P\_up $\rightarrow$ C\_up             & 10 & 235.11 & 141.92 & 0.00  & 1366.00 & 405.25 & 27.03 \\ \hline
T3  & C\_up $\rightarrow$ P\_up             & 9  & 78.27  & 64.22  & 0.00  & 292.84 & 97.34  & 90.00 \\ \hline
T4  & EC $\rightarrow$ P\_up                & 8  & 180.66 & 203.39 & 0.00  & 300.88 & 91.09  & 50.00 \\ \hline
T5  & C\_rm $\rightarrow$ C\_add            & 4  & 19.20  & 0.00   & 0.00  & 76.79  & 38.39  & 80.00 \\ \hline
T6  & C\_add $\rightarrow$ C\_rm            & 4  & 82.21  & 1.54   & 0.00  & 325.75 & 162.37 & 50.00 \\ \hline
T7  & EC $\rightarrow$ C\_up                & 3  & 474.73 & 326.13 & 273.13& 824.91 & 304.42 & 18.75 \\ \hline
T8  & EC $\rightarrow$ C\_rm                & 3  & 184.33 & 252.89 & 46.30 & 253.81 & 119.54 & 18.75 \\ \hline
T9  & C\_add $\rightarrow$ C\_add           & 2  & 5.21   & 5.21   & 0.00  & 10.42  & 7.37   & 25.00 \\ \hline
T10 & EC $\rightarrow$ C\_add               & 2  & 438.48 & 438.48 & 261.21& 615.76 & 250.70 & 12.50 \\ \hline
T11 & P\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 100.00 \\ \hline
T12 & P\_add $\rightarrow$ C\_up            & 1  & 584.03 & 584.03 & 584.03& 584.03 & 0.00   & 50.00 \\ \hline
T13 & P\_add $\rightarrow$ P\_up            & 1  & 161.81 & 161.81 & 161.81& 161.81 & 0.00   & 50.00 \\ \hline
T14 & C\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 20.00 \\ \hline
T15 & C\_add $\rightarrow$ C\_up            & 1  & 584.03 & 584.03 & 584.03& 584.03 & 0.00   & 12.50 \\ \hline
T16 & C\_add $\rightarrow$ P\_up            & 1  & 8.47   & 8.47   & 8.47  & 8.47   & 0.00   & 12.50 \\ \hline
T17 & C\_up $\rightarrow$ C\_rm             & 1  & 285.92 & 285.92 & 285.92& 285.92 & 0.00   & 10.00 \\ \hline
\end{tabular}
}
\end{table}


\begin{table}[h]
\centering
\caption{Transitions of states of release phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:release_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 30 & 90.86  & 61.95  & 0.00  & 311.97 & 86.46  & 63.83 \\ \hline
T2  & EC $\rightarrow$ C\_rm                & 18 & 273.29 & 85.34  & 0.00  & 1170.03& 377.79 & 33.96 \\ \hline
T3  & C\_up $\rightarrow$ C\_up             & 13 & 137.12 & 0.00   & 0.00  & 520.81 & 200.97 & 50.00 \\ \hline
T4  & EC $\rightarrow$ C\_up                & 13 & 445.71 & 270.37 & 0.25  & 1298.49& 473.25 & 24.53 \\ \hline
T5  & EC $\rightarrow$ P\_up                & 12 & 203.64 & 125.98 & 0.00  & 512.00 & 197.30 & 22.64 \\ \hline
T6  & P\_up $\rightarrow$ C\_up             & 11 & 166.19 & 137.67 & 0.00  & 557.50 & 153.70 & 23.40 \\ \hline
T7  & C\_rm $\rightarrow$ C\_rm             & 10 & 14.50  & 0.00   & 0.00  & 145.03 & 45.86  & 55.56 \\ \hline
T8  & C\_up $\rightarrow$ P\_up             & 8  & 70.56  & 18.06  & 0.00  & 292.02 & 107.20 & 30.77 \\ \hline
T9  & C\_rm $\rightarrow$ C\_add            & 6  & 74.19  & 0.00   & 0.00  & 445.13 & 181.73 & 33.33 \\ \hline
T10 & EC $\rightarrow$ C\_add               & 5  & 71.33  & 11.93  & 1.08  & 309.99 & 133.69 & 9.43  \\ \hline
T11 & EC $\rightarrow$ EC                   & 5  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 9.43  \\ \hline
T12 & C\_add $\rightarrow$ C\_add           & 4  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 33.33 \\ \hline
T13 & C\_add $\rightarrow$ C\_up            & 4  & 150.73 & 117.86 & 0.04  & 367.15 & 172.97 & 33.33 \\ \hline
T14 & C\_up $\rightarrow$ C\_rm             & 4  & 371.48 & 429.10 & 34.54 & 593.18 & 238.07 & 15.38 \\ \hline
T15 & P\_up $\rightarrow$ C\_rm             & 4  & 91.89  & 85.88  & 59.81 & 135.99 & 31.95  & 8.51  \\ \hline
T16 & C\_add $\rightarrow$ C\_rm            & 2  & 0.49   & 0.49   & 0.00  & 0.99   & 0.70   & 16.67 \\ \hline
T17 & P\_add $\rightarrow$ C\_up            & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 100.00\\ \hline
T18 & C\_add $\rightarrow$ P\_add           & 1  & 0.42   & 0.42   & 0.42  & 0.42   & 0.00   & 8.33  \\ \hline
T19 & C\_add $\rightarrow$ P\_up            & 1  & 55.04  & 55.04  & 55.04 & 55.04  & 0.00   & 8.33  \\ \hline
T20 & C\_rm $\rightarrow$ C\_up             & 1  & 35.09  & 35.09  & 35.09 & 35.09  & 0.00   & 5.56  \\ \hline
T21 & C\_rm $\rightarrow$ P\_up             & 1  & 36.92  & 36.92  & 36.92 & 36.92  & 0.00   & 5.56  \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Transitions of states of lint phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:lint_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & EC $\rightarrow$ C\_up                & 11 & 476.04 & 160.59 & 0.01  & 1413.24 & 530.04 & 47.83 \\ \hline
T2  & P\_up $\rightarrow$ C\_up             & 8  & 244.19 & 134.07 & 11.38 & 648.94  & 247.46 & 44.44 \\ \hline
T3  & P\_up $\rightarrow$ P\_up             & 8  & 116.10 & 103.77 & 27.75 & 263.80  & 83.99  & 44.44 \\ \hline
T4  & C\_up $\rightarrow$ C\_up             & 8  & 188.50 & 190.79 & 0.00  & 508.01  & 185.58 & 38.10 \\ \hline
T5  & C\_rm $\rightarrow$ C\_rm             & 7  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 58.33 \\ \hline
T6  & C\_up $\rightarrow$ P\_up             & 7  & 60.67  & 0.03   & 0.00  & 224.30  & 88.67  & 33.33 \\ \hline
T7  & EC $\rightarrow$ C\_rm                & 4  & 428.71 & 340.82 & 115.27& 917.91  & 382.73 & 17.39 \\ \hline
T8  & EC $\rightarrow$ P\_up                & 4  & 263.36 & 99.76  & 23.89 & 830.04  & 380.50 & 17.39 \\ \hline
T9  & C\_add $\rightarrow$ C\_add           & 3  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 42.86 \\ \hline
T10 & P\_add $\rightarrow$ C\_up            & 2  & 814.58 & 814.58 & 263.15& 1366.00 & 779.83 & 50.00 \\ \hline
T11 & P\_rm $\rightarrow$ C\_up             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 50.00 \\ \hline
T12 & P\_rm $\rightarrow$ C\_rm             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 50.00 \\ \hline
T13 & C\_add $\rightarrow$ C\_up            & 2  & 201.12 & 201.12 & 35.09 & 367.15  & 234.80 & 28.57 \\ \hline
T14 & C\_rm $\rightarrow$ C\_add            & 2  & 222.57 & 222.57 & 0.00  & 445.13  & 314.76 & 16.67 \\ \hline
T15 & C\_rm $\rightarrow$ P\_rm             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 16.67 \\ \hline
T16 & P\_up $\rightarrow$ C\_rm             & 2  & 535.55 & 535.55 & 202.90& 868.20  & 470.44 & 11.11 \\ \hline
T17 & C\_up $\rightarrow$ C\_rm             & 2  & 2.04   & 2.04   & 0.00  & 4.08    & 2.88   & 9.52  \\ \hline
T18 & C\_up $\rightarrow$ P\_rm             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 9.52  \\ \hline
T19 & EC $\rightarrow$ EC                   & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 8.70  \\ \hline
T20 & P\_add $\rightarrow$ C\_add           & 1  & 89.77  & 89.77  & 89.77 & 89.77   & 0.00   & 25.00 \\ \hline
T21 & P\_add $\rightarrow$ P\_up            & 1  & 0.15   & 0.15   & 0.15  & 0.15    & 0.00   & 25.00 \\ \hline
T22 & C\_add $\rightarrow$ P\_add           & 1  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 14.29 \\ \hline
T23 & C\_add $\rightarrow$ C\_rm            & 1  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 14.29 \\ \hline
T24 & C\_rm $\rightarrow$ C\_up             & 1  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 8.33  \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Transitions of states of analyze phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:analyze_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 46 & 120.01 & 26.14  & 0.20 & 611.55 & 173.33 & 92.00 \\ \hline
T2  & EC $\rightarrow$ P\_up                & 19 & 151.56 & 94.53  & 0.01 & 369.06 & 133.79 & 54.29 \\ \hline
T3  & EC $\rightarrow$ C\_up                & 10 & 517.14 & 384.02 & 0.01 & 1549.93 & 542.26 & 28.57 \\ \hline
T4  & C\_up $\rightarrow$ C\_up             & 6  & 199.45 & 190.42 & 0.00 & 431.84 & 218.27 & 60.00 \\ \hline
T5  & C\_rm $\rightarrow$ C\_rm             & 5  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 50.00 \\ \hline
T6  & C\_rm $\rightarrow$ C\_add            & 4  & 56.72  & 3.91   & 0.00 & 219.07 & 108.25 & 40.00 \\ \hline
T7  & C\_add $\rightarrow$ C\_rm            & 3  & 251.84 & 250.30 & 119.62 & 385.59 & 132.99 & 50.00 \\ \hline
T8  & EC $\rightarrow$ C\_rm                & 3  & 196.91 & 3.48   & 0.01 & 587.24 & 338.04 & 8.57  \\ \hline
T9  & P\_up $\rightarrow$ C\_up             & 3  & 269.95 & 257.62 & 0.00 & 552.24 & 276.33 & 6.00  \\ \hline
T10 & C\_add $\rightarrow$ C\_up            & 2  & 250.48 & 250.48 & 0.00 & 500.96 & 354.23 & 33.33 \\ \hline
T11 & C\_up $\rightarrow$ C\_add            & 2  & 7.10   & 7.10   & 0.00 & 14.21  & 10.05  & 20.00 \\ \hline
T12 & EC $\rightarrow$ EC                   & 2  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 5.71  \\ \hline
T13 & P\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 100.00 \\ \hline
T14 & C\_add $\rightarrow$ P\_up            & 1  & 217.80 & 217.80 & 217.80 & 217.80 & 0.00   & 16.67 \\ \hline
T15 & C\_up $\rightarrow$ C\_rm             & 1  & 4.08   & 4.08   & 4.08 & 4.08   & 0.00   & 10.00 \\ \hline
T16 & C\_up $\rightarrow$ P\_up             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 10.00 \\ \hline
T17 & C\_rm $\rightarrow$ P\_rm             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 10.00 \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Transitions of states of linux phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:linux_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1 & C\_up $\rightarrow$ C\_up          & 4 & 230.93 & 196.61 & 0.00  & 530.50 & 272.48 & 80.00 \\ \hline
T2 & EC $\rightarrow$ C\_up              & 4 & 452.34 & 476.09 & 15.77 & 841.42 & 442.51 & 57.14 \\ \hline
T3 & P\_up $\rightarrow$ P\_up           & 3 & 191.71 & 200.53 & 110.81& 263.80 & 76.88  & 60.00 \\ \hline
T4 & P\_up $\rightarrow$ C\_up           & 2 & 150.85 & 150.85 & 104.80& 196.90 & 65.13  & 40.00 \\ \hline
T5 & EC $\rightarrow$ C\_add             & 2 & 71.45  & 71.45  & 0.96  & 141.95 & 99.70  & 28.57 \\ \hline
T6 & C\_add $\rightarrow$ C\_up          & 1 & 282.87 & 282.87 & 282.87& 282.87 & 0.00   & 100.00 \\ \hline
T7 & C\_up $\rightarrow$ P\_up           & 1 & 210.97 & 210.97 & 210.97& 210.97 & 0.00   & 20.00 \\ \hline
T8 & EC $\rightarrow$ P\_up              & 1 & 133.90 & 133.90 & 133.90& 133.90 & 0.00   & 14.29 \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\caption{Transitions of states of sync phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:sync_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & EC $\rightarrow$ P\_up                & 28 & 250.33 & 72.96  & 0.00 & 693.07 & 284.48 & 90.32 \\ \hline
T2  & P\_up $\rightarrow$ P\_up             & 18 & 409.30 & 288.65 & 0.69 & 698.58 & 220.85 & 48.65 \\ \hline
T3  & C\_add $\rightarrow$ C\_add           & 11 & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 45.83 \\ \hline
T4  & C\_add $\rightarrow$ P\_up            & 11 & 108.01 & 8.47   & 7.78 & 685.42 & 209.03 & 45.83 \\ \hline
T5  & P\_up $\rightarrow$ C\_rm             & 11 & 115.62 & 13.15  & 7.07 & 244.66 & 123.56 & 29.73 \\ \hline
T6  & P\_rm $\rightarrow$ C\_add            & 6  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 54.55 \\ \hline
T7  & C\_rm $\rightarrow$ P\_rm             & 6  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 46.15 \\ \hline
T8  & P\_rm $\rightarrow$ C\_rm             & 5  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 45.45 \\ \hline
T9  & C\_rm $\rightarrow$ C\_add            & 5  & 0.00   & 0.00   & 0.00 & 0.01  & 0.00   & 38.46 \\ \hline
T10 & P\_up $\rightarrow$ P\_rm             & 4  & 23.02  & 7.07   & 7.07 & 70.85  & 31.89  & 10.81 \\ \hline
T11 & C\_up $\rightarrow$ P\_up             & 2  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 100.00 \\ \hline
T12 & EC $\rightarrow$ C\_rm                & 2  & 52.97  & 52.97  & 3.99 & 101.94 & 69.26  & 6.45  \\ \hline
T13 & P\_up $\rightarrow$ C\_add            & 2  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 5.41  \\ \hline
T14 & P\_add $\rightarrow$ C\_add           & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 50.00 \\ \hline
T15 & P\_add $\rightarrow$ C\_up            & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 50.00 \\ \hline
T16 & C\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 7.69  \\ \hline
T17 & C\_rm $\rightarrow$ P\_add            & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 7.69  \\ \hline
\end{tabular}
}
\end{table}

==> dataset_old.tex <==
% \yuan{can we present a figure showing how we collect and process data for each RQ ref.https://arxiv.org/pdf/2601.03780, we need to discuss what to put in this section rather the approach for specific RQ later}


\begin{figure*}
    \centering
    \includegraphics[width=1.1\linewidth]{figures/overall.png}
    \caption{ Overview of our study.}
    \label{fig:overall}
\end{figure*}

In this section, we describe how we collected and prepared data to answer RQ1 to RQ3. Figure \ref{fig:overall} summarizes the overall pipeline and shows how our data preparation outputs connect to each research question.
\vspace{0.2cm}



\noindent \textbf{Data Source:} We build on the repository set released by Bouzenia et al. \cite{bouzenia2024resource}, which contains 952 GitHub repositories and 1.3 million workflow logs. In this study, we use the repository set as our starting point. Our analyses focus on workflow configuration files and their change history in Git, because RQ1 to RQ3 examine caching settings in YAML and how these settings are evolved over time. The workflow logs in the original dataset are not used in our analyses.

\vspace{0.2cm}

\noindent \textbf{Data preprocessing:} Following Figure \ref{fig:overall}, we perform four preprocessing steps.



\subsection{Data Source}
\yuan{too short as a subsection, more details needed.}
This study is based on dataset created by Islem et a \cite{bouzenia2024resource}. The dataset contains 952 repositories with their associated 1.3 millions of workflow runs\yuan{but we did not use the workflow run? Maybe there are other details about this dataset and how it is created, worth mentioning.}

\yuan{rework needed on this section, i will check the refined version}

\subsection{Data preprocessing}
As our analysis exclusively focuses on 'caching' within GA workflows, we only considered the repositories that adopted caching at any point in their history. This filtering step identified 266 repositories (27.9\% of the original dataset) which met this criterion. These 266 repositories form the basis for our subsequent analyses\yuan{a bit confusing as very soon you mentioned taht you collect metadata for all 952 repos, not only those adopted caching. Also, what's the definition of "adopted"}. \amit{I had to collect metadata of all repos because we wanted to compare two groups adopted vs non adopted. And yes, I agree with the point of defining adopted.}

\subsection{Preparing data for RQs}
To address our research questions, we undertook several data preparation steps.

To understand the current characteristics of repositories that adopt caching (RQ1), we collected metadata for all 952 repositories (both adopters and non-adopters) using the  GitHub v4 API\footnote{https://docs.github.com/en/graphql}. This metadata included counts of contributors, commits, closed pull requests, stars, forks, issues, and the primary programming language. As caching configurations is the key focus in our research, we reconstructed the workflow histories of 266 repositories using gigawork \cite{cardoen2024dataset}\footnote{\url{https://github.com/cardoeng/gigawork}}, which extracts workflow files from the Git history. This tool extracts all historical versions of workflow files along with commit-level metadata (hash, timestamp, path). Our dataset spans commits up to May 5, 2025. 


\yuan{very surprised to hear that you categorize jobs, and it is unclear why we need it} We then categorized the jobs within the workflow files based on their job names defined by developers, adapting the CI/CD phase taxonomy from \citet{bouzenia2024resource}. While most of the studies focus solely on actions/cache \citep{zhang2024developers}, we expanded our scope based on official documentation\footnote{https://github.com/actions/cache} to capture other caching strategies\yuan{why suddenly moved to caching strategies while you categorize job}. Our dataset covers both explicit strategies, which require manual parameter inputs, and implicit strategies, where caching is enabled by default. For instance, \textit{setup-go@v4} action enable caching by default to obtain the benefits of caching\footnote{https://github.blog/changelog/2023-03-24-github-actions-the-setup-go-action-now-enables-caching-by-default/}, while other require manual parameter inputs to enable caching. We incorporated these language specific requirements in our study. As a result, our study covers different language specific caching strategies (shown in Table \ref{tab:caching_default}) along with \textit{actions/cache}, resulting in a more comprehensive and representative dataset for our study. 



\begin{table}[h]
\centering
\caption{Different programming languages and their caching settings by default\yuan{confused why there is no language column and why you need to mention setup/go@v4 rather than go, and how it differs from other go@v3, etc.}}
\label{tab:caching_default}
\begin{tabular}{|c|c|}
\hline
             & \textbf{Enabled cache by default} \\ \hline
setup/go@v4  & Yes                               \\ \hline
setup/python & No                                \\ \hline
setup/node   & No                                \\ \hline
setup/ruby   & No                                \\ \hline
setup/ruby   & No                                \\ \hline
setup/java   & No                                \\ \hline
\end{tabular}
\end{table}


For RQ2's transition analysis\yuan{i don't think authors know what is your transition analysis, what do you mean by transition analysis, not enough background provided before reaching here}, we processed the historical git data obtained via Gigawork\yuan{what is this, missing references?} to identify and track only those commits that specifically related to caching configurations within the workflow files. All non-cache-related changes were excluded\yuan{such as? i wonder if it is easy to understand what are non chache related change for readers}. 



Finally, for RQ3's qualitative analysis\yuan{you are using a short name but readers don't know what do you mean, that's why it is better to have an overview figure first}, we performed a manual analysis\yuan{this sounds like methodology of RQ3, rather than preparing for RQ3} of the code changes, commit messages, and associated pull requests for a statistically significant random sample (detailed further in RQ3) of the cache-related commits identified for RQ2.


\begin{table}[h]
\centering
\caption{Setup actions considered in our study and whether caching is enabled by default in the action version we observe in workflow files.}
\label{tab:caching_default}
\small
\begin{tabular}{lll}
\toprule
\textbf{Language/tool} & \textbf{Setup action (example)} & \textbf{Caching enabled by default} \\
\midrule
Go & \texttt{actions/setup-go@v4} & Yes \\
Python & \texttt{actions/setup-python} & No \\
Node.js & \texttt{actions/setup-node} & No \\
Ruby & \texttt{ruby/setup-ruby} & No \\
Java & \texttt{actions/setup-java} & No \\
\bottomrule
\end{tabular}
\end{table}







==> discussion_old.tex <==
\subsection{Implications}

\subsubsection{For CI/CD Practitioners}


\noindent \textbf{Cache action versions are likely stale, representing a form of maintenance debt.} The first version update after enabling a cache often does not occur for over a year (median 384 days) (RQ3, Finding 2). This "set it and forget it" behavior means projects miss out on performance improvements, bug fixes, and security patches. Also, our findings reported in Table \ref{tab:rq3_table_1} represents several important drivers of version updates. If developers do not update the versions, they might encounter avoidable build failures, exposure to known security vulnerabilities that have already been patched in newer releases. Practitioners should schedule regular audits of their cache-related GitHub Actions, similar to how they manage other software dependencies. 


\yuan{why we highlight so much about bot in the beginning rather than talking about actionable insights from evolution analysis, i.e., RQ2 and RQ3}
\noindent \textbf{Developers should not blindly trust version upgrades, even from bots.} Our study identified that cache downgrades (N=4) are a critical, human-led tactic used to recover from failed upgrades (RQ3, Finding 7). This directly proves that upgrades whether manual or bot-driven are not risk-free and can break the pipeline. Practitioners must understand that automated tools (like Dependabot) only handle the simple task of proposing an upgrade. They leave the complex, cognitive work of debugging and reverting that upgrade to humans when it fails. Automated bots are responsible for 100\% of simple "Bot alert" triggers, but these only perform simple version upgrades (RQ3, Finding 3). Practitioners must disabuse themselves of the notion that their CI/CD performance is being "managed" by automation. Bots ensure your cache, language versions are up-to-date, their roles are limited to ensure its effectiveness. Teams must formally schedule periodic, human-led reviews of cache performance, hit rates, and key-design, as our data proves they are the only ones performing this critical optimization work. 
\smallskip

\noindent \textbf{Create closed loop feedback system for bot induced failures.\yuan{could not follow this conclusion}} We identified rare but critical manual "downgrade" actions (RQ3, Finding 7), where humans must intervene to fix a problem introduced by an upgrade (likely from a bot or a human just following bot advice). This is a clear failure of the open-loop automation model. When a bot's PR (e.g., "Bump actions/cache @v4") is merged and followed by either build failures or a human-led revert, the bot must learn. It should flag that version as "potentially problematic" for that repository's context, halt further suggestions, and ideally warn other projects with similar configurations. 


\smallskip

\yuan{I believe this is a separate claim from "create closed loop"}. We found that \textbf{parameter update} is the most common cache modification, accounting for 58.20\% of its target state transitions (Table \ref{tab:rq3}). The median time is 4.29 days which suggests it's rapid and deliberate nature. Our qualitative analysis (RQ3.2, Finding 1) indicates that this is not proactive tuning but is overwhelmingly driven by developers reactively "Fixing caching issues" (69.6\% of that driver's actions are parameter updates) shown in Table 20. Practitioners must stop treating cache configuration as a one-time setup task and re-frame it as a continuous debugging activity. We recommend the formal inclusion of cache specific reviews into agile ceremonies (e.g., sprint planning, retrospectives) to manage this debt. Project managers, in turn, must begin to explicitly budget developer-hours for this hidden, but now quantified, maintenance burden. Also, Bots are completely absent from this activity. The next generation of CI/CD tooling must move from "dependency bots" to "performance bots." These agents should be hooked into the CI/CD logs, detect the P\_up $\rightarrow$ P\_up churn, analyze cache-miss logs to identify the specific file or parameter causing invalidation, and proactively propose a semantic fix.

\smallskip

\noindent \textbf{Developers should adopt phase aware caching strategies.} Our findings show that caching practices and their evolution differ significantly across different CI/CD phases\yuan{i don't see this highlighted in RQ2 or RQ3}. For example, the release phase has a high probability of cache removal (EC → C\_rm at 34\%) and longer maintenance cycles (P\_up → P\_up, median 61.95 days), whereas build and test phases have rapid parameter tuning (median 4.08 and 2.93 days, respectively. Teams should tailor their caching strategies to the specific phase. In critical phases like release, caching should be introduced cautiously, with a focus on stability and reliability. In high-frequency phases like build and test, aggressive caching and frequent tuning are beneficial. This phase-aware approach can optimize both performance and reliability.



\smallskip


 \noindent \textbf{Cache addition is an indicator of strategic engineering task.\yuan{hard to follow this claim}} Our result reveals that the "Add Cache" action (N=362) is driven by fundamentally different motivations than other cache modifications. Unlike parameter updates, which are often reactive bug fixes (fixing caching issues, N=16), or version updates, which are automated maintenance (bot alert, N=40), cache addition is almost exclusively a human-led, strategic activity. The dominant drivers are extending cache (N=28), which corresponds to adding new jobs, and improve cache (N=17), which is a deliberate optimization (RQ3, Finding 5). This aligns with the finding that EC $\rightarrow$ C\_add occurs relatively quickly (medians 40-55 days) in build/test phases (RQ2). Practitioners should, therefore, view these events as key indicators of functional pipeline expansion or active performance refinement, rather than grouping them with other, more mundane maintenance tasks.



\subsubsection{For tool builders}

\noindent \textbf{Tools should focus on debugging cache configurations, not just updating versions.} The most common developer activity identified in this study is fixing  caching issues (RQ3, Finding 1). This is a significant, unaddressed pain point. Tooling must move beyond simple version bumping. CI platforms and IDEs could provide static analysis of workflow files to detect common errors. Dashboards that visualize cache hit/miss rates per job and per key. This would provide immediate feedback, helping developers move beyond the "guess-and-check" parameter update cycle.

\smallskip

\noindent \textbf{Dependency bots should be "phase-aware" and capable of handling failure.\yuan{could not follow this claim}} Maintenance cadences are phase-specific. build/test phases are fast, while release is slow (RQ2, Insight 1). Automated tools should recognize this, perhaps suggesting updates more conservatively or with different priority levels for different jobs. Our study found that humans must manually clean up failed upgrades via downgrades (RQ3, Finding 7). Bots should monitor the build status of the PRs they create. If a cache version bump is merged and the build subsequently fails, the bot could automatically open a new PR to revert the change or post a warning, saving human debugging time.


\noindent Our data on "long-tail" obsolescence (the 384-day update cycle, RQ3, F2) reveals a lack of basic configuration management. Developers should build a repository-level "CI/CD Health" dashboard. This dashboard should flag "Stale Caches" (e.g., "This cache config is 384+ days old and 2 major versions behind"). This turns latent maintenance burdens into an actionable, prioritized list.


\subsubsection{For researchers}

\noindent \textbf{Quantify the performance impact of cache (mis)management.} This study establishes the what and why of cache evolution. The logical next step is to measure the so what. Future work should quantitatively correlate the transition patterns and drivers we identified with concrete CI/CD metrics, such as workflow duration, cost, and failure rates. This would answer critical questions about the tangible return on investment for different caching strategies and the true cost of maintenance.
\smallskip

\noindent \textbf{Investigate the gap between human and bot-led cache management.} A clear divide was found, bots only handle version bumps, while humans perform all complex cognitive tasks such as debugging (fixing caching issues), optimization (improve cache), and migration (RQ3, Finding 3). This presents a rich area for research in AI for DevOps.


\smallskip 
\noindent\textbf{Propose a new research agenda on self adaptive CI/CD caching.} Our study reveals a system that is brittle, manually debugged (RQ3), and prone to correctness risk in critical pipelines (RQ2)\yuan{not sure if i see that in RQ2 and RQ3}. This is a prime target for intelligent automation, yet the existing automation is naive (RQ3, F3). We call for a new research agenda on "Self-Adaptive CI/CD Caching." This moves beyond "smarter bots" and envisions systems that: 1) Learn the project's dependency graph; 2) Automatically A/B test cache-key strategies; 3) Correlate changes with performance data; and 4) Autonomously roll back failed experiments (automating the 4.25-day C\_add $\rightarrow$ C\_rm loop). A key sub-challenge is verifiable caching for release pipelines, which has ties to formal methods and reproducible build research.



==> intro_old.tex <==

Modern software development is characterized by rapid and highly collaborative cycles, enabled by the widespread adoption of Continuous Integration and Continuous Deployment (CI/CD) practices. CI/CD pipelines automate integration, testing, and deployment activities, allowing teams to sustain fast iteration and gradually improve product quality in line with agile development principles. A variety of platforms have been developed to support CI/CD pipelines, including Jenkins, Travis CI, CircleCI, and GitHub Actions (GHA). Despite their benefits, CI/CD pipelines also introduce execution overhead, especially as workflow complexity grows. When workflows become slow, they delay feedback to developers, hinder collaboration, and increase computational costs. To reduce this overhead, platforms such as GHA provide configurable caching support that allows developers to define caching behaviors suited to their workflows. These caching mechanisms accelerate CI/CD by storing and reusing artifacts—such as project dependencies or intermediate build outputs—that remain unchanged across workflow runs.



\yuan{similar to comment on abstract, do we want to highlight GHA from the beginning? I think it is just a target/mined data we choose} Modern software development is characterized by rapid, collaborative cycles, driven by\yuan{"driven by" sounds like the CI/CD is the motivation} the widespread adoption of Continuous Integration and Continuous Deployment (CI/CD). These automated pipelines are no longer niche practices but are now fundamental to the software development lifecycle\yuan{a bit redundent with the prior line}, allowing teams to improve both development velocity and final product quality ~\citep{shahin2017continuous}. GitHub Actions (GHA), introduced in 2019 \footnote{https://github.blog/news-insights/product-news/github-actions-now-supports-ci-cd/}, has rapidly emerged as a dominant platform in this ecosystem\yuan{is it dominant in the market or dominant in github hosted repos?}, with studies confirming its widespread adoption across tens of thousands of open-source projects~\citep{decan2022use, chen2021let}. 

\yuan{Rewrote for above: Modern software development is characterized by rapid and highly collaborative cycles, enabled by the widespread adoption of Continuous Integration and Continuous Deployment (CI/CD) practices. CI/CD pipelines automate integration, testing, and deployment activities, allowing teams to sustain fast iteration and gradually improve product quality in line with agile development principles~\citep{shahin2017continuous}. A variety of platforms have been developed to support CI/CD pipelines, including Jenkins, Travis CI, CircleCI, and GitHub Actions (GHA).}


A critical challenge\yuan{there is no explain why it is a challenge.} for CI/CD pipelines is performance\yuan{"performance" can be multi-aspect, it seems that you are talking about execution of CI/CD pipeline}. Slow workflows delay feedback to developers, hinder collaboration, and increase computational costs~\citep{bouzenia2024resource}. To optimize workflow efficiency, platforms such as GHA provide caching mechanisms designed to accelerate builds by storing and reusing artifacts—such as project dependencies or intermediate build outputs—that remain unchanged across workflow runs~\citep{gallaba2020accelerating}. 

\yuan{Rewrote for above: Despite their benefits, CI/CD pipelines also introduce execution overhead, especially as workflow complexity grows. To reduce this overhead, platforms such as GHA provide configurable caching support that allows developers to define caching behaviors suited to their workflows \yuan{add reference}. When pipelines become slow, they delay feedback to developers, hinder collaboration, and increase computational costs~\citep{bouzenia2024resource}. These caching mechanisms accelerate CI/CD by storing and reusing artifacts, such as project dependencies or intermediate build outputs, that remain unchanged across workflow runs~\citep{gallaba2020accelerating}.}


However, caching is not a simple optimization\yuan{simple toggle}. Implementing an effective caching strategy is notoriously complex. Developers must correctly identify what to cache, define precise cache keys to manage invalidation\yuan{what do you mean by "manage invalidation"}. This process is non-trivial, as an improperly configured cache key can fail to capture build-breaking changes, while an overly broad one provides no performance benefit. Research in the Bazel ecosystem further confirms that caching can yield substantial performance benefits \citep{zheng2024does}\yuan{is this about caching CI/CD? weak connection between this sentence and the prior one.} Consequently, what is intended as a simple performance boost often becomes a significant, yet often overlooked, maintenance burden, adding to the "hidden costs" of CI/CD \citep{valenzuela2024hidden}\yuan{why citing another paper, what is this paper about, CI/CD caching cost?}.



Despite this acknowledged complexity and high maintenance cost\yuan{about CI/CD pipelines or caching?}, a significant research gap exists regarding how development teams actually manage caching in practice within GHA\yuan{i suggest we mention GHA late as our target system, but highlight from general CI/CD perspective}. While prior research has explored GHA evolution holistically  \citep{decan2022use}, \citep{chen2021let}, the specific, fine-grained dynamics of caching configurations remain unstudied\yuan{these papers on GHA are less relevant, we could mention them in background or related work}. \yuan{Major issue: It is unclear why knowing the unknown items you listed is essential to known, which we should highlight.} It is unknown, for example, which CI/CD phases (e.g., build, test) developers prioritize for caching or how these strategies differ across projects. More critically, the evolutionary aspect of these configurations is a "black box."\yuan{wrong formatting of quotes} We do not know how often developers are forced to tune or debug their cache settings, what specific factors drive these changes, and \yuan{unable to follow the remaining part, what do you mean? and why was socio-technical suddenly mentioned} what the socio-technical interplay is between human developers and automated bots in performing this maintenance. 



% Despite its critical role, little is known about how caching is adopted, configured, and maintained in practice within GHA. While existing research has explored GHA evolution holistically, the evolutionary dynamics and maintenance drivers of GHA caching remain unstudied. It is unclear how developers tune these configurations over time, why they make changes, and who (humans or bots) performs this work.

To bridge this gap, we present the first large-scale, cache-centric empirical study of GHA workflows. \yuan{let's describe general dataset used for answering three RQs here} Our empirical study addresses the following three research questions (RQs):


\begin{itemize}
    \item [] \textbf{RQ1: \rqone} \yuan{using "latest snapshot" is our methodology details, should not occur in the RQ title but in your description} In this RQ, we performed a comparative analysis of 266 caching-adopting repositories against 680 non-adopters\yuan{if this is for all RQs, should be moved up}. We found that caching adopters are consistently larger and more active across all repository metrics\yuan{could not understand this sentence, be more specific}. Furthermore, caching is strategically applied in resource-intensive CI/CD phases like build and test, with direct caching being the dominant caching type (70.9\% of all cache configurations)

    \vspace{0.1cm}
    \item [] \textbf{RQ2: \rqtwo} \yuan{the title has no keyword about evolution, which is the key aspect in RQ2} In this RQ, we model the evolution of caching configurations as a first-order Markov model. Our findings reveal that caching practices are highly phase-specific. High-frequency phases like \texttt{build} and \texttt{test} exhibit rapid, iterative tuning, while critical phases like \texttt{release} show slower update cycles and a significant tendency for cache removal after initial adoption.
    \vspace{0.1cm}
    \item [] \textbf{RQ3: \rqthree} \yuan{title contains specific undefined term, i.e., caching transitions} In this RQ, we combined quantitative transition analysis with a qualitative study of commit messages and PR discussions. We developed a taxonomy of change drivers, finding that humans perform all complex debugging and optimization (e.g., `fixing caching issues`)\yuan{i expect you talk about taxonomy or prevalence rather than human-bot}, while bots are confined to simple version updates. The most frequent change,parameter updating occurs on a rapid 4.29 day median and is primarily reactive, aimed at resolving configuration problems.
\end{itemize}

%Our results suggest future researchers \yuan{something from implications should be put here.}

The main contributions of this paper include: 
\begin{itemize}
    % \item [-] We present the first large-scale empirical study of CI caching adoption and evolution in GitHub Actions where we analyzed caching configurations at code level and connect them with assocaited meta data. Our study introduces a detailed taxonomy of the drivers and modification actions (e.g., Upgrade, Downgrade) behind cache evolution.
    \item [-] We present the first large-scale empirical study of CI caching adoption, evolution, and motivating drivers in GitHub Actions. We link code-level configuration changes to their qualitative drivers from commit and PR metadata, introducing taxonomy of modification actions and their underlying developer motivations.

    \item [-] We provide a comprehensive analysis of GHA caching practices by expanding the scope beyond the explicit \texttt{actions/cache} action to include implicit mechanisms.

   \item [-] Our study reveals the multifaceted nature of cache management. We find that caching is not a simple one-time optimization, but a complex, ongoing maintenance task. We show that the most frequent cache changes are not proactive tuning but reactive, human-led debugging, while automated bots only handle simple version updates, leaving all complex cognitive work to developers.
   
   \item [-] We provide concrete implications for developers, researchers, and CI/CD tool builders based on our findings.
   
   \item [-] To foster future research in the area, we have made our replication package
publicly available.
\end{itemize}



We organize the remainder of the paper as follows.  Section~\ref{sec:dataset} introduces our dataset. Section~\ref{sec:rq1}-\ref{sec:rq3} present methodology and answers to each of the three research questions. Section~\ref{sec:disc} discusses the implications of findings for practitioners and researchers. Section~\ref{sec:threats} presents threats to validity, and Section~\ref{sec:related} presents related work. Finally, Section~\ref{sec:conclusion} concludes the paper.

==> rq1_old.tex <==
This research question examines the characteristics of repositories that have adopted caching via GitHub Actions. We investigate project size and activity, language ecosystem, workflow structure, and where/what caching is used in CI/CD. We contrast these characteristics with repositories that have not adopted caching to identify distinguishing characteristics.

\section{Approach}
To characterize repositories that adopt GitHub Actions caching, we combine a repository-level comparative analysis with a configuration-level profiling of adopters’ workflows. We retrieve repository metadata using GitHub GraphQL API (described in section \ref{sec:dataset}) and summarize each metric at the repository level and compare the two groups using group-level descriptive statistics. We reconstructed the history of workflow files (described in section \ref{sec:dataset}) of cache-adopting repositories, and report the distribution of per-repository to quantify how files are distributed across repository and the number of jobs defined in the latest snapshot. To characterize caching usage in cache adopting repositories, we analyze caching at two granularities: 
 

 
\vspace{0.1cm}

\begin{itemize}
    \item [] \textbf{Job-level:} GitHub Actions workflows do not provide any prior guideline for defining the  jobs and in most cases developers name them freely\footnote{https://docs.github.com/en/actions/reference/workflows-and-actions/workflow-syntax}. As a result, aggregating raw job names would not yield interpretable, cross-repository conclusions. To solve this, we categorize each job into a CI/CD jobs based on its developer defined job name using a keyword-based taxonomy refined via several rounds of refinement \citep{bouzenia2024resource}. Then, we identify whether each job uses caching by checking whether it contains at least one cache-related configuration step in their workflows. For each CI/CD job, we then compute job-level caching prevalence as the fraction of jobs in contain at least one cache-related step. 
    
    \item[] \textbf{Step-level:} At step level, we aim to understand how caching is being implemented within the jobs. We extract each cache-related configurations from steps within the workflow file and categorized them based on the type of caching used by developers\footnote{https://www.ubicloud.com/blog/github-actions-transparent-cache}. Caching can be configured and used multiple times within the same job, we captured such cases too and presented in Table xx. 

\end{itemize}



% \subsection{Approach}
% To characterize the repositories that adopt caching, we performed a comparative analysis. \yuan{take a look at the sample paper I mentioned before, the content you described here could be in section 3, here we expect details of how you compare the two groups, assuming you have metadata collected from section3, how you analyze the workflow structure, how you perform an understanding of current caching.}First, we contrasted the repository-level metadata (e.g., contributors, commits, stars) of the 266 caching adopters against the 680 non-adopters to identify differences in project size and activity and programming language. Second, we analyzed the workflow structure of the 266 caching adopters, calculating the distribution of workflow files and jobs per repository. Finally, to understand current caching strategies, we focused on the latest snapshot that are actively using caching. We applied our job classification taxonomy (described in Section \ref{sec:dataset}) to determine where in the CI/CD pipeline caching is used. We also categorized the type of cache (Package Manager, File/Folder, etc.) to determine what is being cached and analyzed the distribution of these types across the CI/CD phases. 


\subsection{Results}



\noindent \textbf{Observation 1.1: \textit{Repositories that adopt caching are larger and more active than non-adopters repository-level activity and popularity metrics.}} Table \ref{tab:repo_stats} / Figure \ref{fig:doublesided} \amit{we may keep just one}shows the  repository-level characteristics for cache adopting and non-cache adopting repositories. Compared to non caching adopted repositories, caching adopted repositories have more contributors, commits, closed PRs, stars, forks and issues. This also exhibit greater community interest, with higher median stars and forks. Higher involvement also indicates the complexity of using caching within the repositories. This reflects that repositories with higher activity and community engagement are more likely to enable caching at one point in their lifecycle to keep CI workloads manageable.

\begin{figure*}
    \centering
    \includegraphics[scale=0.18]{figures/double_sided_repo_v2.png}
    \caption{Distributions of repository characteristics for repositories with and without caching. Values are plotted on a log(1+X) scale for better readability, and annotated medians are in original counts.}
    \label{fig:doublesided}
\end{figure*}

\vspace{0.1cm}

\noindent \textbf{Observation 1.3:\textit{Caching adoption differs across primary languages within our dataset.}} Table~\ref{tab:language_stats} compares the primary programming languages of repositories with and without caching. To account for differences in language prevalence in our sample, we report the \emph{within-language adoption rate}, which captures the proportion of repositories in each language category that adopt caching. PHP and Java show the highest adoption rates (54.2\% and 50.7\%), whereas Python (22.3\%), Ruby (17.6\%). We use this result to contextualize caching adoption in our GitHub Actions sample and do not generalize it beyond the studied repositories.

\begin{table}[h]
\caption{Primary programming languages of repositories with and without caching in our GitHub Actions sample. We report the within-language adoption rate (proportion of repositories in each language category that adopt caching) to account for differences in language prevalence within the dataset.}
\centering
\label{tab:language_stats}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Language} &
\textbf{\begin{tabular}[c]{@{}c@{}}With caching \\ (n=266)\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Without caching \\ (n=680)\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Adoption rate \end{tabular}} \\ \hline
Python      & 42 & 146 & 22.3\% \\ \hline
TypeScript  & 45 & 79  & 36.3\% \\ \hline
JavaScript  & 37 & 109 & 25.3\% \\ \hline
Java        & 36 & 35  & 50.7\% \\ \hline
PHP         & 26 & 22  & 54.2\% \\ \hline
Go          & 22 & 54  & 28.9\% \\ \hline
C++         & 17 & 52  & 24.6\% \\ \hline
Kotlin      & 12 & 21  & 36.4\% \\ \hline
C           & 9  & 38  & 19.1\% \\ \hline
Ruby        & 6  & 28  & 17.6\% \\ \hline
Shell       & 4  & 17  & 19.0\% \\ \hline
Others      & 10 & 79  & 11.2\% \\ \hline
\end{tabular}
\end{table}


\vspace{0.1cm}

\noindent \textbf{Observation 1.3: \textit{Cache-adopting repositories typically have one workflow file and job, with a small set of long-tail cases.}} Table \ref{tab:dist_files_jobs} represents per-repository workflow structure for cache adopting repositories. The median number of workflow files per repository is 1, and the 75th percentile is also 1, indicating that at least 75\% of adopters keep their workflow configuration within a single workflow file. This result is consistent with the minimal setup required to enable caching in GitHub Actions\footnote{https://github.com/actions/cache}. We also observe long tail distribution, with some repositories maintaining up to 8 workflow files. A similar pattern appears in job structure. The median number of jobs per repository in the latest snapshot is 1. However, the maximum reaches 57 jobs, showing that a small subset of repositories operate substantially more complex workflow structure. Overall, these results suggest that caching adoption starts by using single workflow files and it can be further used in in repositories with much more elaborate CI configurations. 


\begin{table}[h]
\caption{Statistical distribution of files and jobs per repository.}
\label{tab:dist_files_jobs}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
                                    & \textbf{Min} & \textbf{Mean} & \textbf{std} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \textbf{Max} \\ \hline
\textbf{\# of files per repository} & 1            & 1             & 1.1          & 1             & 1             & 1             & 8            \\ \hline
\textbf{\# of jobs per repository}  & 1            & 2.46          & 3.98         & 1             & 1             & 3             & 57           \\ \hline
\end{tabular}
\end{table}

\vspace{0.1cm}

\noindent \textbf{Observation 1.4: \textit{At job level, caching is most prevalent in build, integration, lint, and test oriented jobs.}} Table \ref{tab:cicd_phase} reports the highest job-level caching prevalence in build (37.31\%) and integration (36.58\%). Test (25.96\%) and lint (27.84\%) also show notable prevalence. By contrast, analyze remains lower (15.87\%), and sync is rare (5.08\%). These phase differences indicate that caching is primarily deployed in phases where repeated dependency installation and artifact reuse is common (e.g., build and test), whereas jobs focused on synchronization or maintenance are less likely to benefit from caching.


\begin{table}[]
\caption{Caching in different CI/CD jobs.}
\centering
\label{tab:cicd_phase}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}CI/CD job\\  types\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of jobs \\ with caching\end{tabular}} & \textbf{Total jobs} & \textbf{\begin{tabular}[c]{@{}c@{}}Caching\\  prevalence ( \%)\end{tabular}} \\ \hline
build                                                               & 247                                                                         & 662                 & 37.31\%                                                                      \\ \hline
test                                                                & 141                                                                         & 543                 & 25.96\%                                                                      \\ \hline
release                                                             & 76                                                                          & 332                 & 22.89\%                                                                      \\ \hline
lint                                                                & 22                                                                          & 79                  & 27.84\%                                                                      \\ \hline
analyze                                                             & 20                                                                          & 126                 & 15.87\%                                                                      \\ \hline
linux                                                               & 6                                                                           & 29                  & 20.69\%                                                                      \\ \hline
integration                                                         & 15                                                                          & 41                  & 36.58\%                                                                      \\ \hline
sync                                                                & 3                                                                           & 59                  & 5.08\%                                                                       \\ \hline
other                                                               & 51                                                                          & 457                 & 11.16\%                                                                      \\ \hline
Total                                                               & 581                                                                         & 2328                & 24.95\%                                                                      \\ \hline
\end{tabular}
\end{table}
\end{table}

\vspace{0.1cm}

\noindent \textbf{Observation 1.5: \textit{Repositories adopt caching through three different caching strategies.}} We derived a taxonomy of cache types used in GitHub Actions workflows: 
\begin{enumerate}
    \item [-] \textbf{Explicit caching:} Caching is configured through an explicit cache step, using \textit{actions/cache} where developers provide cache paths and keys. We define this  “explicit” because caching is enabled only when developers declare a cache step and specify its inputs, which offers flexibility to cache arbitrary directories (e.g., dependency folders, build outputs, tool caches), but requires the most manual configuration. 
    

    \item [-] \textbf{Package manager caching with (setup-* actions):} Caching is enabled through language/tool setup actions (e.g., \texttt{setup-go, setup-node, setup-python}) that either expose a caching option or provide caching behavior as part of the setup interface. We separate this from explicit cache actions because the developer’s configuration is mediated by the setup action, and the cached content is typically tied to dependency management conventions of that ecosystem.
    
    
    \item [-] \textbf{Docker layer caching:} Caching is configured through Docker build tooling (e.g., docker/build-push-action) to reuse previously built layers. This is distinct from the two mechanisms above because the cached units are Docker image layers, and the configuration uses Docker’s caching interface rather than file-path caching.
    \item [-] \textbf{Others:} Any caching configuration that does not fall into the above categories.
\end{enumerate}
\vspace{0.1cm}

\begin{table}[]
\caption{Distribution of cache strategies across different CI/CD job types}
\label{tab:cache_type_phase}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}CI/CD job\\ types\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Explicit \\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Package\\ Manager \\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Docker Layer\\ Caching\end{tabular}} & \textbf{Others} & \textbf{Total} \\ \hline
build                                                              & 282 (73.1\%)                                                         & 71 (18.4\%)                                                                   & 1 (0.3\%)                                                               & 32 (8.3\%)      & 386            \\ \hline
test                                                               & 178 (75.4\%)                                                         & 53 (22.5\%)                                                                   & 0 (0.0\%)                                                               & 5 (2.1\%)       & 236            \\ \hline
release                                                            & 41 (41.0\%)                                                          & 59 (59.0\%)                                                                   & 0 (0.0\%)                                                               & 0 (0.0\%)       & 100            \\ \hline
other                                                              & 75 (80.6\%)                                                          & 17 (18.3\%)                                                                   & 1 (1.1\%)                                                               & 0 (0.0\%)       & 93             \\ \hline
analyze                                                            & 23 (74.2\%)                                                          & 6 (19.4\%)                                                                    & 0 (0.0\%)                                                               & 2 (6.5\%)       & 31             \\ \hline
lint                                                               & 19 (70.4\%)                                                          & 8 (29.6\%)                                                                    & 0 (0.0\%)                                                               & 0 (0.0\%)       & 27             \\ \hline
integration                                                        & 10 (66.7\%)                                                          & 5 (33.3\%)                                                                    & 0 (0.0\%)                                                               & 0 (0.0\%)       & 15             \\ \hline
linux                                                              & 7 (100.0\%)                                                          & 0 (0.0\%)                                                                     & 0 (0.0\%)                                                               & 0 (0.0\%)       & 7              \\ \hline
sync                                                               & 2 (66.7\%)                                                           & 1 (33.3\%)                                                                    & 0 (0.0\%)                                                               & 0 (0.0\%)       & 3              \\ \hline
Total                                                              & 637 (70.9\%)                                                         & 220 (24.5\%)                                                                  & 2 (0.2\%)                                                               & 39 (4.3\%)      & 898   \\ \hline
\end{tabular}
\end{table}


\noindent \textbf{Observation 1.6: \textit{Explicit caching strategies dominate at the step level.}} Table~\ref{tab:cache_type_phase} shows that explicit caching via \texttt{actions/cache} accounts for the majority of cache-related steps (70.9\%). Package-manager dependency caching through \texttt{setup-*} actions is the second most common mechanism (24.5\%). Docker layer caching is rare (0.2\%). 

A plausible explanation for the dominance of explicit caching is its flexibility and configurability. Developers can explicitly specify cache paths and keys, which enables caching beyond dependencies (e.g., build outputs and tool caches)\footnote{https://dev.to/github/caching-dependencies-to-speed-up-workflows-in-github-actions-3efl}. Moreover, \texttt{actions/cache} is extensively documented and commonly referenced in tutorials, blog posts, and Q\&A forums such as Stack Overflow\footnote{https://stackoverflow.com/questions/74401969/what-is-the-logic-in-using-the-restore-keys-field-in-the-github-cache-action}, lowering the barrier to adoption through readily reusable examples \citep{baltes2019usage}. Its long-standing and stable interface may further make it an attractive choice from a maintainability and backward-compatibility perspective, whereas caching support in \texttt{setup-*} actions is mediated by ecosystem-specific conventions and may change over time\footnote{https://github.com/actions/setup-node}. Finally, explicit caching is well aligned with iterative CI optimization, as it supports incremental refinement of cache paths and key design in response to cache misses and performance bottlenecks\footnote{https://docs.github.com/en/actions/reference/workflows-and-actions/dependency-caching}.

\vspace{0.1cm}

\noindent \textbf{Observation 1.7: \textit{ Most cache-related steps appear in build and test jobs.}}  Table~\ref{tab:cache_type_phase} shows that caching is being used frequently in build and test jobs, together representing 69.3\% of total cases. Within these jobs, caching is primarily implemented through explicit caching strategy, followed by package-manager caching. This observation complements the job level view in Table \ref{tab:cicd_phase} and shows how the caching is being configured within the jobs by developers.   



\begin{tcolorbox}[enhanced,width=4.7in,size=fbox,drop shadow southwest,sharp corners]

\textbf{RQ1 Summary:} Our findings suggest that repositories that adopt caching are larger and more active than non-adopters across repository-level activity and popularity metrics. Cache adopting repositories maintain at least one workflow file and job to use and configure caching. At job level, caching is most prevalent in build, integration, lint, and test oriented jobs. At the step level, developers implement caching mainly through explicit caching strategy, followed by package manager caching and docker layer caching strategies.
\end{tcolorbox}



\subsubsection{Repository size and activity.} \yuan{no need subsubseciton, just present findings and show evidence (figure/table)}
% \begin{table}
% \centering
% \caption{Repository characteristics by caching adoption (medians per repository).}
% \label{tab:repo_stats}
% \begin{tabular}{|c|c|c|}
% \hline
%                               & \textbf{Repositories with caching} & \textbf{Repositories without caching} \\ \hline
% Total number of repositories         & 266                         & 680                            \\ \hline
% Median number of contributors & 43.5                        & 29                             \\ \hline
% Median number of commits      & 1005                        & 592                            \\ \hline
% Median number of PRs (closed) & 258.5                       & 114.5                          \\ \hline
% Median starts                 & 728.5                       & 531.5                          \\ \hline
% Median forks                  & 127.0                       & 102.5                          \\ \hline
% Median issues                 & 141.5                       & 73                             \\ \hline
% \end{tabular}
% \end{table}



\begin{table}[]
\caption{Repository characteristics by caching adoption (medians per repository)\yuan{can we do something similar to: A first look at good first issues on GitHub table 1?}}
\centering
\label{tab:repo_stats}
\begin{tabular}{|c|c|c|}
\hline
                                                                         & \textbf{\begin{tabular}[c]{@{}c@{}}Repositories \\ with caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Repositories \\ without caching\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}c@{}}Total number of \\ repositories\end{tabular}  & 266                                                                           & 680                                                                              \\ \hline
\begin{tabular}[c]{@{}c@{}}Median number of \\ contributors\end{tabular} & 43.5                                                                          & 29                                                                               \\ \hline
\begin{tabular}[c]{@{}c@{}}Median number of \\ commits\end{tabular}      & 1005                                                                          & 592                                                                              \\ \hline
\begin{tabular}[c]{@{}c@{}}Median number of\\  PRs (closed)\end{tabular} & 258.5                                                                         & 114.5                                                                            \\ \hline
Median starts                                                            & 728.5                                                                         & 531.5                                                                            \\ \hline
Median forks                                                             & 127.0                                                                         & 102.5                                                                            \\ \hline
Median issues                                                            & 141.5                                                                         & 73                                                                               \\ \hline
\end{tabular}
\end{table}


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.2]{figures/double_sided_repo_v2.png}
    \caption{Distributions of repository characteristics for repositories with and without caching\yuan{wonder if we change to log scale, would it be easier to tell the difference?}}
    \label{fig:doublesided}
\end{figure}

\noindent \textbf{Finding 1: Repositories that adopt  caching are consistently larger and more active than non-adopters across all metrics, \yuan{first sentence should be the finding statement, other details in later part, e.g., shown in which figure/table}as shown in Table \ref{tab:repo_stats}.} Compared to non caching adopted repositories, caching adopted repositories have more contributors, commits, closed PRs, stars, forks and issues. This also exhibit greater community interest, with higher median stars and forks. Higher involvement also indicates the complexity of using caching within the repositories. This reflects that repositories with higher activity and community engagement are more likely to enable caching at one point in their lifecycle to keep CI workloads manageable. \yuan{figure 2 is not referred and discussed here} 


% Table \ref{tab:repo_stats} summarizes median characteristics for two groups repositories that adopted CI caching and those that did not. Our findings reveals that repositories that adopted CI caching are consistently larger and more active than non-adopters across all medians in Table \ref{tab:repo_stats}. Relative to non caching adopted repositories, caching adopted repositories have more contributors, commits, closed PRs, stars, forks and issues. This also exhibit greater community interest, with higher median stars and forks. Higher involvement also indicates the complexity of using caching within the repositories. This reflects that repositories with higher activity and community engagement are more likely to enable caching at one point in their lifecycle to keep CI workloads manageable. 

Since repository characteristics vary with caching adoption, it is worth exploring whether certain language ecosystems with different build and dependency behaviors are more prone to adopting caching.



\subsubsection{Programming language ecosystems.} \yuan{no need subsubsection} \yuan{I am not sure how much our data reflects the adoption popularity at the PL level; our data may be very limited and specific to those with GitHub Actions. the numbers here may just due to popularity of PLs. we could also just focus on what differs from with vs. without caching rather than the numbers we could see from table and similar}
\noindent\textbf{Finding 2: Caching is widely adopted among Python, TypesScript, JavaScript, Java, PHP and Go languages.} Table \ref{tab:language_stats} shows the distribution of programming languages among repositories that adopted CI caching and those that did not. For caching adopters, the most common languages are TypeScript (45 repositories, 16\%), Python (42, 15\%), JavaScript (37, 13\%), and Java (36, 13\%), together accounting for over half of all projects in this group. Non caching adopting repositories also implemented in Python, TypeScript and JavaScript mostly. But Java representing only 5\% of the group (35 repositories) compared to 13\% among caching adopters. 

Since adoption correlates with languages that often require more build steps, the next step is to examine workflow complexity in these repositories—i.e., how many files and jobs their CI/CD setups contain. \yuan{i don't think this is needed, could put in approach, in result, let's just present findings and support.}

% \begin{table}[h]
% \centering
% \caption{Programming languages of repositories with and without caching.}
% \label{tab:language_stats}
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Language} & \textbf{With caching (n=266)} & \textbf{Without caching (n=680)} \\ \hline
% Python      & 42 (15\%) & 146 (21\%) \\ \hline
% TypeScript  & 45 (16\%) & 79 (11\%)  \\ \hline
% JavaScript  & 37 (13\%) & 109 (16\%) \\ \hline
% Java        & 36 (13\%) & 35 (5\%)   \\ \hline
% PHP         & 26 (9\%)  & 22 (3\%)   \\ \hline
% Go          & 22 (8\%)  & 54 (7\%)   \\ \hline
% C++         & 17 (6\%)  & 52 (7\%)   \\ \hline
% Kotlin      & 12 (4\%)  & 21 (2\%)   \\ \hline
% C           & 9 (3\%)   & 38 (5\%)   \\ \hline
% Ruby        & 6 (2\%)   & 28 (4\%)   \\ \hline
% Shell       & 4 (1\%)   & 17 (2\%)   \\ \hline
% Others      & 10 (4\%)  & 79 (12\%)  \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[h]
\caption{Programming languages of repositories with and without caching. \yuan{i am not sure how to interpret this table}} \amit{add ratio here, that's might be more meaningful}
\centering
\label{tab:language_stats}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Language} & \textbf{\begin{tabular}[c]{@{}c@{}}With caching \\ (n=266)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Without caching \\ (n=680)\end{tabular}} \\ \hline
Python            & 42 (15\%)                                                                & 146 (21\%)                                                                  \\ \hline
TypeScript        & 45 (16\%)                                                                & 79 (11\%)                                                                   \\ \hline
JavaScript        & 37 (13\%)                                                                & 109 (16\%)                                                                  \\ \hline
Java              & 36 (13\%)                                                                & 35 (5\%)                                                                    \\ \hline
PHP               & 26 (9\%)                                                                 & 22 (3\%)                                                                    \\ \hline
Go                & 22 (8\%)                                                                 & 54 (7\%)                                                                    \\ \hline
C++               & 17 (6\%)                                                                 & 52 (7\%)                                                                    \\ \hline
Kotlin            & 12 (4\%)                                                                 & 21 (2\%)                                                                    \\ \hline
C                 & 9 (3\%)                                                                  & 38 (5\%)                                                                    \\ \hline
Ruby              & 6 (2\%)                                                                  & 28 (4\%)                                                                    \\ \hline
Shell             & 4 (1\%)                                                                  & 17 (2\%)                                                                    \\ \hline
Others            & 10 (4\%)                                                                 & 79 (12\%)                                                                   \\ \hline
\end{tabular}
\end{table}





\subsubsection{Analyzing configuration file structure}

\begin{table}[h]
\caption{Statistical distribution of files and jobs per repository (266 repos) }
\label{tab:dist_files_jobs}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
                                    & \textbf{Min} & \textbf{Mean} & \textbf{std} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \textbf{Max} \\ \hline
\textbf{\# of files per repository} & 1            & 1             & 1.1          & 1             & 1             & 1             & 8            \\ \hline
\textbf{\# of jobs per repository}  & 1            & 2.46          & 3.98         & 1             & 1             & 3             & 57           \\ \hline
\end{tabular}
\end{table}

\noindent \textbf{Finding 3: Most caching-adopting repositories use a minimal\yuan{compared to what?is this the same for any repo with CI workflow? what's special about those adopted caching?} number of workflow files and jobs.} Section \ref{sec:background} explains the configuration structure of a typical repository that uses caching. Table \ref{tab:dist_files_jobs} shows that the median number of workflow files per repository is 1, with a maximum of 8, indicating that the majority manage their CI/CD configurations within a single file. Similarly, the median number of jobs per repository is 1, although the distribution is skewed by a few large projects with up to 57 jobs. The low medians, coupled with small interquartile ranges, suggest that caching is often adopted in relatively simple workflow setups, while only a small subset of repositories integrate caching into more complex, multi-job pipelines.


To understand how caching is applied within these workflows, we next classify jobs by CI/CD phase.


\subsubsection{Analyzing different caching adopted phases} \yuan{motivation needs to be done in the approach so that we know why this analysis is useful. Methodology needs to be in the section wise approach not in results}


\begin{table}[h]
\caption{Caching in different CI/CD phases in the latest snapshot. \yuan{column names a bit confusing, probably because the granularity of phase is not clearly defined, suggest making it clear in the capture as well.}}
\centering
\label{tab:cicd_phase}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{CI/CD phase} & \begin{tabular}[c]{@{}c@{}}\# of jobs in latest \\ snapshot where \\caching was used\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total jobs \\ in latest snapshot\end{tabular} & \begin{tabular}[c]{@{}c@{}}Percentage of' \\ jobs that use caching\end{tabular} \\ \hline
build       & 247 & 662 & 37.31\% \\ \hline
test        & 141 & 543 & 25.96\% \\ \hline
release     & 76 & 332 & 22.89\% \\ \hline
lint        & 22  & 79  & 27.84\% \\ \hline
analyze     & 20  & 126 & 15.87\% \\ \hline
linux       & 6   & 29  & 20.69\% \\ \hline
integration & 15  & 41  & 36.58\% \\ \hline
sync        & 3   & 59  & 5.08\%  \\ \hline
other       & 51  & 457 & 11.16\% \\ \hline
\textbf{Total} & \textbf{581} & \textbf{2328} & \textbf{24.95\%} \\ \hline
\end{tabular}
\end{table}




% We analyzed all workflow (\texttt{.yml}/\texttt{.yaml}) files from repositories that adopted GitHub Actions caching. To capture the most recent characteristics of these projects, we focused on their latest snapshots. Specifically, we examined the most recent workflow files to identify the jobs in which developers configured caching. We found that out of 266 repositories, 232 repositories use caching in their last snapshot. 34 repositories enabled caching at some point of their lifecycle, but they are not using this anymore in our latest snapshot. For example: aa3326b4480ccc9dd9c2a4d1c7a6152008d7d2ae commit is the very last snapshot of LCUI repository. But it doesn't have any caching related configurations in it. We are not considering the reposiotories which do not have caching utilized in their last snapshot in this analysis. For CI/CD phases, we compared the number of jobs uses caching against the total number of jobs present in the latest snapshot, providing a comprehensive view of caching usage at the job level.

\yuan{i feel it is not clear to readers that this is at job-level rather than file level}To better understand the intended CI/CD tasks represented by these jobs, we categorized them based on job names. Our classification scheme for CI/CD phases was adapted from \citet{bouzenia2024resource}. We began by matching single keywords in job names to preliminary categories and then iteratively refined the taxonomy through manual inspection of ambiguous or unclassified jobs. After several rounds of refinement, we finalized the categorization shown in Table~\ref{tab:cicd_phase}.



% We analyzed all yml files of repositories that adopted GA. To understand the very latest characteristics of repositories, we investigated the latest snapshots. We analyzed the latest yml files and identified in which job level developers used caching. We also compared this with overall jobs available in the latest snapshot to get the full comprehensive look. To better understand the CI/CD tasks that developers want to perform with jobs in a workflow, we categorize jobs based on their names. We adopted the categorization of CI/CD phases from \citep{bouzenia2024resource}. We initially searched for single names and later iteratively enriched our categorization by manually investigating. After several rounds of iteration, we finalize the taxonomoy of Table \ref{tab:cicd_phase}



\noindent \textbf{Finding 4: Caching is most prevalent in build (37.31\%), test (25.96\&), lint (27.84\%)  and integration (36.58\%) jobs.}  Table~\ref{tab:cicd_phase} presents caching usage by CI/CD phase in the most recent workflow snapshot of caching adopters. Caching is most prevalent in build jobs, where 37.31\%. Substantial adoption is also observed in lint (27.84\%), integration (36.58\%), test (25.96\%), and release (22.89\%) jobs. These patterns suggest that caching is strategically used in phases where its benefits are most immediate especially build, test, and integration tasks, which often involve dependency installation, compilation, or artifact preparation. This finding also matches with the findings of \cite{bouzenia2024resource}\yuan{why this related work has similar findings? How does our analysis differ from theirs? this could be put in the motivation for this RQ or methodology}  

By contrast, caching is used far less in analyze (15.87\%), linux environment–specific jobs (20.69.03\%), and particularly sync jobs, where only 5.08\%  enable it. The other category, which covers jobs without a clear phase classification, also shows low usage (11.16\%).




\subsubsection{Analyzing caching strategies} \yuan{now we have so many findings, i don't want them to be 10 subsubsections, it may still be helpful to group them into two or three general types, could they be subrqs? }

\yuan{there should be no approach in results}To understand current caching practices and the nature of the artifacts being cached in GitHub Actions, we performed an empirical analysis of all cache-related configurations found in the latest workflow snapshots of caching-adopting repositories. From this analysis, we derived a taxonomy of cache types used in GitHub Actions workflows:

% To determine the nature of artifacts being cached in the most recent workflow configurations, we analyzed all cache-related configurations in the latest snapshots of caching-adopting repositories. From this analysis, we derived a taxonomy of cache types used in GitHub Actions workflows:

% \begin{enumerate}
%     \item [-] \textbf{File/Folder Caching:} The simplest caching approach, implemented via the \texttt{actions/cache} action, which allows developers to specify one or more files or directories to persist between workflow runs.
%     \item [-] \textbf{Package Manager Caching:} For package managers, GitHub offers language specific actions like \texttt{actions/setup-go}, \texttt{actions/setup-python}, and \texttt{actions/setup-node} etc.
%     \item [-] \textbf{Docker Layer Caching:} For Docker builds, caching unchanged Docker layers helps speed up image builds. docker/build-push-action provides caching for Docker layers. Developers can pass gha as type to cache  files on GitHub’s cache infrastructure.
%     \item [-] Any caching configuration that does not fall into the above categories.
% \end{enumerate}


\begin{enumerate}
    \item [-] \textbf{Direct caching:} The simplest caching approach, implemented via the \texttt{actions/cache} action, which allows developers to specify one or more files or directories to persist between workflow runs.  \yuan{not sure if direct caching is a good name, Explicit caching? why it is the simplest caching approach, i feel it needs more configuration than others..what's the main differences between this one and other options? the differences is not highlighted}
    \item [-] \textbf{Language specific caching:} GitHub offers language specific ways to use caching for different languages. While most of them follow action/cache pattern, there are other different language specific (package manager with setup-*) ways to use caching\footnote{https://github.com/actions/cache} actions like \texttt{actions/setup-go}, \texttt{actions/setup-python}, and \texttt{actions/setup-node} etc. \footnote{https://www.ubicloud.com/blog/github-actions-transparent-cache} 
    \item [-] \textbf{Docker layer caching:} For Docker builds, caching unchanged Docker layers helps speed up image builds. docker/build-push-action provides caching for Docker layers. Developers can pass gha as type to cache  files on GitHub’s cache infrastructure.
    \item [-] \textbf{Others:}Any caching configuration that does not fall into the above categories.
\end{enumerate}



% \begin{table}[h]
% \centering
% \caption{Distribution of cache types in the latest workflow snapshot of caching-adopting repositories.}
% \label{tab:what_cache}
% \begin{tabular}{|c|c|}
% \hline
% Cache type              & Count \\ \hline
% Caching package manager & 217   \\ \hline
% Caching file/folder     & 636   \\ \hline
% Caching docker layer    & 8     \\ \hline
% Others                  & 15    \\ \hline
%                         % & -  \\ \hline
% \end{tabular}
% \end{table}




\noindent \textbf{Finding 5: Caching in GitHub Actions workflows is dominated by direct caching mechanism}, which accounts for 637 instances (70.9\% of all identified cache configurations, as shown in Table \ref{tab:cache_type_phase}). This indicates that developers most frequently use caching to explicitly persist custom build artifacts, compiled binaries, or other intermediate files. The second most common type is Language Specific Caching (220 instances, 24.5\%), used to persist dependencies for package managers. We found only 2 instances of Docker Layer Caching (0.2\%). \yuan{wonder if we could talk about our hypothesis why it is most popular, for instance, Why it dominates:Language-agnostic, Especially attractive for polyglot or non-standard projects, Historically first, Early adopters naturally used it, Maximum control, Better documentation because most tutorials, StackOverflow answers, and blog posts reference actions/cache,Copy-paste friendliness matters, Backward compatibility, Language-specific caching has evolved and changed semantics, actions/cache remains stable. If we could link it to optimization, even better.} \amit{need more clarification on this}


% Upon investigation of the 'Other' category, we found that developers mentioned \textit{cache-key} in those configuration files. In GitHub Actions, a cache key is a unique identifier (often based on file hashes, operating system, or dependency versions) used to determine whether a previously saved cache can be restored in a workflow run. Developers often compute cache key in one job and use it in a different job. This allows them to centralize key generation and ensure consistent cache usage across multiple jobs. While these instances did not match our predefined caching patterns, the presence of a cache key suggests that caching was still being configured or referenced in these workflows. 






% \begin{table}[h]
% \caption{Distribution of cache types across CI/CD phases in the latest workflow snapshot.} 
% \label{tab:cache_type_phase}
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{CI/CD phase} & \textbf{\begin{tabular}[c]{@{}c@{}}Docker Layer\\ caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Direct \\ caching\end{tabular}} & \textbf{Others} & \textbf{\begin{tabular}[c]{@{}c@{}}Language\\ specific\\ caching\end{tabular}} & \textbf{Total} \\ \hline
% build       & 1 & 282 & 32 & 320 & 635 \\ \hline
% test        & 0 & 178 & 5  & 267 & 450 \\ \hline
% release     & 0 & 41  & 0  & 165 & 206 \\ \hline
% other       & 1 & 75  & 0  & 117 & 193 \\ \hline
% lint        & 0 & 19  & 0  & 37  & 56  \\ \hline
% analyze     & 0 & 23  & 2  & 15  & 40  \\ \hline
% integration & 0 & 8   & 0  & 15  & 23  \\ \hline
% linux       & 0 & 7   & 0  & 4   & 11  \\ \hline
% sync        & 0 & 2   & 0  & 3   & 5   \\ \hline
% \textbf{Total} & \textbf{2} & \textbf{635} & \textbf{39} & \textbf{943} & \textbf{1619} \\ \hline
% \end{tabular}
% \end{table}


% \begin{table}[h]
% \caption{Distribution of cache types across CI/CD phases in the latest workflow snapshot.}
% \centering
% \label{tab:cache_type_phase}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}CI/CD \\ phase\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Direct\\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Language\\ Specific\\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Docker Layer\\ Caching\end{tabular}} & \textbf{Others} & \textbf{Total} \\ \hline
% build                                                           & 282                                                               & 71                                                                             & 1                                                                       & 32              & 386            \\ \hline
% test                                                            & 178                                                               & 53                                                                             & 0                                                                       & 5               & 236            \\ \hline
% release                                                         & 41                                                                & 59                                                                             & 0                                                                       & 0               & 100            \\ \hline
% other                                                           & 75                                                                & 17                                                                             & 1                                                                       & 0               & 93             \\ \hline
% analyze                                                         & 23                                                                & 6                                                                              & 0                                                                       & 2               & 31             \\ \hline
% lint                                                            & 19                                                                & 8                                                                              & 0                                                                       & 0               & 27             \\ \hline
% integration                                                     & 8                                                                 & 5                                                                              & 0                                                                       & 0               & 13             \\ \hline
% linux                                                           & 7                                                                 & 0                                                                              & 0                                                                       & 0               & 7              \\ \hline
% sync                                                            & 2                                                                 & 1                                                                              & 0                                                                       & 0               & 3              \\ \hline
% \textbf{Total}                                                  & \textbf{635}                                                      & \textbf{220}                                                                   & \textbf{2}                                                              & \textbf{39}     & \textbf{896}   \\ \hline
% \end{tabular}
% \end{table}







\begin{table}[h]
\caption{Distribution of cache types across CI/CD phases.} \amit{I am planning to exclude others category from this table. Need feedback.} \yuan{first, you need to explain what's the ratio refers to. I am fine with others, for total, maybe you don't need a ratio, what does that refer to? why the total number 898 does not match with any number in table 6?} \amit{The totals in Table \ref{tab:cache_type_phase} count cache configurations (multiple per job are possible), whereas Table \ref{tab:cicd_phase} counts jobs; therefore, the denominators differ.}
\centering
\label{tab:cache_type_phase}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}CI/CD \\ phase\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Direct\\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Language\\ Specific\\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Docker Layer\\ Caching\end{tabular}} & \textbf{Others} & \textbf{Total} \\ \hline
build & 282 (73.1\%) & 71 (18.4\%) & 1 (0.3\%) & 32 (8.3\%) & \textbf{386 (43.0\%)} \\ \hline
test & 178 (75.4\%) & 53 (22.5\%) & 0 (0.0\%) & 5 (2.1\%) & \textbf{236 (26.3\%)} \\ \hline
release & 41 (41.0\%) & 59 (59.0\%) & 0 (0.0\%) & 0 (0.0\%) & \textbf{100 (11.1\%)} \\ \hline
other & 75 (80.6\%) & 17 (18.3\%) & 1 (1.1\%) & 0 (0.0\%) & \textbf{93 (10.4\%)} \\ \hline
analyze & 23 (74.2\%) & 6 (19.4\%) & 0 (0.0\%) & 2 (6.5\%) & \textbf{31 (3.5\%)} \\ \hline
lint & 19 (70.4\%) & 8 (29.6\%) & 0 (0.0\%) & 0 (0.0\%) & \textbf{27 (3.0\%)} \\ \hline
integration & 10 (66.7\%) & 5 (33.3\%) & 0 (0.0\%) & 0 (0.0\%) & \textbf{15 (1.7\%)} \\ \hline
linux & 7 (100.0\%) & 0 (0.0\%) & 0 (0.0\%) & 0 (0.0\%) & \textbf{7 (0.8\%)} \\ \hline
sync & 2 (66.7\%) & 1 (33.3\%) & 0 (0.0\%) & 0 (0.0\%) & \textbf{3 (0.3\%)} \\ \hline
\textbf{Total} & \textbf{637 (70.9\%)} & \textbf{220 (24.5\%)} & \textbf{2 (0.2\%)} & \textbf{39 (4.3\%)} & \textbf{898 (100.0\%)} \\ \hline
\end{tabular}
\end{table}


% \begin{table}[h]
% \caption{Distribution of cache types across CI/CD phases (excluding "other" category).}
% \centering
% \label{tab:cache_type_phase}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}CI/CD \\ phase\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Direct\\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Language\\ Specific\\ Caching\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Docker Layer\\ Caching\end{tabular}} & \textbf{Total} \\ \hline
% build & 282 (73.1\%) & 71 (18.4\%) & 1 (0.3\%) & \textbf{386 (43.0\%)} \\ \hline
% test & 178 (75.4\%) & 53 (22.5\%) & 0 (0.0\%) & \textbf{236 (26.3\%)} \\ \hline
% release & 41 (41.0\%) & 59 (59.0\%) & 0 (0.0\%) & \textbf{100 (11.1\%)} \\ \hline
% analyze & 23 (74.2\%) & 6 (19.4\%) & 0 (0.0\%) & \textbf{31 (3.5\%)} \\ \hline
% lint & 19 (70.4\%) & 8 (29.6\%) & 0 (0.0\%) & \textbf{27 (3.0\%)} \\ \hline
% integration & 10 (66.7\%) & 5 (33.3\%) & 0 (0.0\%) & \textbf{15 (1.7\%)} \\ \hline
% linux & 7 (100.0\%) & 0 (0.0\%) & 0 (0.0\%) & \textbf{7 (0.8\%)} \\ \hline
% sync & 2 (66.7\%) & 1 (33.3\%) & 0 (0.0\%) & \textbf{3 (0.3\%)} \\ \hline
% \textbf{Total} & \textbf{562 (72.0\%)} & \textbf{203 (26.0\%)} & \textbf{1 (0.1\%)} & \textbf{781 (100.0\%)} \\ \hline
% \end{tabular}
% \end{table}



% \noindent \textbf{Finding 6:} Table~\ref{tab:cache_type_phase} reveals a strong interaction between the \emph{type} of caching mechanism employed and the \emph{CI/CD phase} in which it is used. As explained in Section \ref{sec:background}, one job can have multiple type of cache enabled. This is why we noticed a increase in the CI/CD phases in Table \ref{tab:cache_type_phase}. Across all phases, package manager caching dominates, accounting for 943 of the 1,619 identified cache instances (58.2\%), followed by direct file/folder caching at 635 instances (39.2\%). The “Others” category (39 instances, 2.4\%) while Docker layer caching is nearly absent (2 instances, 0.1\%).

\noindent \textbf{Finding 6: The build phase is the most cache-intensive, containing 386 cache instances (43.0\% of all caches).\yuan{it sounds like similar to finding 4, which is prevalence at job type level}} This phase heavily relies on Direct Caching (282 instances; 73.1\% of build caches), with Language Specific Caching playing a smaller role (71 instances; 18.4\%). The test phase (236 total instances; 26.3\% of all caches) shows a similar pattern, also being dominated by Direct Caching (178 instances; 75.4\%) over Language Specific Caching (53 instances; 22.5\%). This suggests that both build and test jobs frequently reuse custom artifacts or intermediate files.


Other phases show more specialized caching patterns. Notably, the release phase (100 total instances) is the only major phase where Language Specific Caching is the preferred strategy (59 instances; 59.0\%) over Direct Caching (41 instances; 41.0\%). \yuan{i don't see how this is supported by the above result}This aligns with the need to rebuild artifacts from reproducible dependency states before packaging.




% Beyond artifact type, configuration choices such as action version and parameter use reveal how up-to-date and fine-tuned caching setups are.

% \subsubsection{Analyzing cache versions}

% GitHub regularly updates their cache services and the most recent one is v4. To examine versioning practices in caching configurations, we analyzed the most recent workflow snapshots from all caching-adopting repositories. 

% \begin{figure} [h]
%     \centering
%     \includegraphics[scale=0.3]{figures/versions.png}
%     \caption{Caption}
%     \label{fig:versions}
% \end{figure}

% \noindent \textbf{Finding 7:} Figure~\ref{fig:versions} shows the distribution. The five most common tags — v4 (25.84\%), v2 (24.35\%), v1 (16.45\%), v3 (15.22\%), and v5 (11.20\%) — collectively account for over 93\% of all observed versions. This indicates a strong preference for major version pinning, aligning with GitHub’s backward-compatibility guarantees for semantic major releases. 


% Despite newer releases being available, legacy versions remain in heavy use: v1 is still used in 254 instances, and v2 in 376. This suggests that many repositories have not updated their workflows to the latest major release, potentially missing performance or security improvements introduced in newer versions.

% Only a small fraction of usages specify full semantic versions (e.g., v3.3.1, v4.2.3), each representing less than 0.5\% of the dataset. This may reflect developer reliance on major version stability rather than minor/patch-level precision.


% We also found some non-standard and potentially risky references. Commit SHAs (1.62\%) guaranteeing exact reproducibility but lacking automatic security patches. Branch names such as master (1.10\%) potentially unstable, as upstream changes may alter behavior without explicit version bumps. Beta or pre-release tags (v2-beta) rare (0.19\%), but indicative of early adopters testing unreleased features.



% \subsubsection{Analyzing cache configuration practices} 

% GitHub’s official caching action supports a range of optional parameters that allow developers to fine-tune caching behavior. To examine the extent of their use in practice, we performed a keyword-based search across all caching-enabled steps in the latest workflow snapshots of the 266 caching-adopting repositories. Specifically, we searched for the following parameter names:
% \texttt{restore-keys}, \texttt{enableCrossOsArchive}, \texttt{fail-on-cache-miss}, and \texttt{lookup-only}.




% % Within the steps, GitHub officially provides a lot of paramters/fuctions to use. We performed a keyword based search to investigate if any repositories are using those configurations or not. We searched for     "restore-keys",
% %     "enableCrossOsArchive",
% %     "fail-on-cache-miss",
% %     "lookup-only" keywords. 


% \noindent \textbf{Finding 8:} Only 120 of the 266 repositories (45.1\%) used any of these advanced cache parameters. Among those, usage was limited exclusively to \texttt{restore-keys} and \texttt{enableCrossOsArchive}; no instances of \texttt{fail-on-cache-miss} or \texttt{lookup-only} were found. This suggests that while nearly half of caching adopters leverage some form of configuration beyond the defaults, adoption is concentrated on parameters that improve cache hit rates (\texttt{restore-keys}) or enable cross-OS cache portability (\texttt{enableCrossOsArchive}). The absence of the other parameters  indicate limited awareness of their existence

\begin{tcolorbox}[enhanced,width=4.7in,size=fbox,drop shadow southwest,sharp corners]

\textbf{RQ1 Summary:} \yuan{first sentence is not our answer but method}We provided a multi-dimensional profile of repositories that adopted GA in their lifecycle. Repositories with caching are tend to be larger, more active projects, often in ecosystems with heavier build requirements. Caching is strategically applied in resource intensive\yuan{what do you mean by resource intensive, do we define this type anywhere before?} CI/CD phases, with direct caching and language specific caching being the dominate strategies. 
\end{tcolorbox}


\yuan{no need this paragraph, the relationship should either mentioned in intro or motivation for RQ2}This RQ captures the latest characteristic, but the process by which repositories arrive at these configurations and whether they migrate to newer cache versions over time remain unexamined. Addressing these dynamic aspects requires moving beyond a static view to analyze the transition patterns of caching-related changes, which we undertake in RQ2.

==> rq2_old.tex <==

\subsection{Motivation}


While RQ1 established the static characteristics of caching adopters, it does not explain how these configurations evolve over time. Caching is rarely a static and  one-time configuration. As projects grow and dependencies change, developers must update cache keys, paths, and strategies to maintain high hit rates and low build times. This research question examines these temporal dynamics and analyzes the evolution of caching configurations across different CI/CD job types. Understanding these evolution patterns is meaningful because it reveals (i) what types of cache maintenance activities are most common, (ii) how quickly configuration updates occur, and (iii) whether these dynamics differ by job type (e.g., build vs. test). These insights benefit (1) practitioners, by setting realistic expectations about the maintenance effort required to keep caching effective and stable, and (2) tool and platform designers, by highlighting where better defaults, diagnostics, or guidance could reduce repeated trial-and-error in cache maintenance.



\subsection{Approach} \amit{working here}

To analyze the evolution of caching configurations, we modeled the sequence of cache-related changes as a first-order Markov model \citep{gagniuc2017markov} \yuan{should be citep rather than cite, i updated a few, please make it consistent across the paper, unless you want to just mention author names}. This approach maps the probabilistic transitions developers make between different cache modification \textit{states} over time. \yuan{for data preprocessing across RQs, better to be put in the general data preprocessing methodology not RQ specific approach} First, we processed the historical commit timeline for each job, classifying the job by its CI/CD phase (per RQ1). We then categorized each cache-related commit into one of seven states described in Section \ref{sec:background}. We then aggregated these state sequences within each CI/CD phase to construct a transition graph (e.g., Figure \ref{fig:build_tran}). For each transition (edge) in the graph, we calculated its probability and the time based statistics in days. We pruned the graph by removing transitions with probabilities lower than 0.05, ensuring a focus on statistically significant relationships \citep{hao2024empirical}. 



\subsection{Results} 


\noindent \textbf{Observation 2.1: \textit{Caching configurations follow a repetitive maintenance pattern.}} Across almost all job types \textit{(build, test, integration, release)}, the most frequent cache maintenance activities are self-loops. This includes Parameter Update $\rightarrow$ Parameter Update ($P\_up \rightarrow P\_up$) and Cache Update $\rightarrow$ Cache Update ($C\_up \rightarrow C\_up$). For example, in \textit{build} jobs, $C\_up \rightarrow C\_up$ accounts for 77.63\% of activity with a median time of 0 days (Table \ref{tab:build_trans_short}). Similarly, in Test jobs, $P\_up \rightarrow P\_up$ occurs 66.05\% of the time (Table \ref{tab:test_trans_short}). 

This indicates that cache maintenance is rarely a static implementation. Once a developer begins tuning parameters or updating cache versions, they tend to continue doing so in a sequence of related commits. This suggests that maintaining a cache is an iterative process requiring sustained attention rather than a single action.


\vspace{0.2cm}

\noindent \textbf{Observation 2.2: \textit{Developers frequently engage in rapid parameter tuning.}} The $P\_up \rightarrow P\_up$ activity is dominant in development job types. In Build jobs, this occurs with 65.53\% probability and a median of 4.08 days (Table \ref{tab:build_trans_short}). In Test jobs, it occurs with 66.05\% probability and a median of just 2.93 days (Table \ref{tab:test_trans_short}).

This reflects an active debugging cycle. Developers tweak a configuration, run the pipeline, and then tweak it again days later to optimize performance.

\vspace{0.2cm}

\noindent \textbf{Observation 2.3: \textit{New caches in Test jobs are often discarded shortly after implementation.}} In Test jobs, the maintenance activity from adding a cache to removing it ($C\_add \rightarrow C\_rm$) happens with a median of 32.49 days (Table \ref{tab:test_trans_short}).

This suggests that approximately one month after adding new caches in test related jobs, developers often remove them. It indicates a trial-and-error process where not all cache additions provide sustainable value. Teams likely discover that the overhead or flakiness of the new cache outweighs its benefits.

\vspace{0.2cm}


\noindent \textbf{Observation 2.4: \textit{Developers frequently add new caches shortly after the initial enablement.}} After the initial cache adoption, developers frequently perform the activity of adding additional caches shortly after enabling the first one. The median time for $EC \rightarrow C\_add$ is 41.97 days for Test jobs (Table \ref{tab:test_trans_short}) and 53.14 days for Build jobs (Table \ref{tab:build_trans_short}). 

This indicates that cache adoption is an incremental process rather than a one-time setup. The delay of approximately 1.5 months suggests that developers typically start with a baseline configuration, and only expand the caching strategy after a period of initial usage.

\vspace{0.2cm}

\noindent \textbf{Observation 2.5: \textit{Cache removal is often part of an immediate replacement.}} In Build jobs, the transition from removing a cache to immediately adding a new one ($C\_rm \rightarrow C\_add$) occurs with 21.84\% probability and a median of 0.01 days (Table \ref{tab:build_trans_short}). Similarly, in Test jobs, this occurs with 30.19\% probability and a median of 0.00 days (Table \ref{tab:test_trans_short}). 

The near-zero median time indicates that developers are not permanently removing caches, they are replacing an old configuration with a new one. This suggests that the initial cache setup was insufficient, prompting a switch to a different strategy (e.g., changing from a generic key to a specific file hash) rather than abandoning caching altogether. 

\vspace{0.2cm}

\noindent \textbf{Observation 2.6: \textit{Build and Test jobs show the most frequent and fastest parameter updates.}} The time between consecutive parameter updates ($P\_up \rightarrow P\_up$) is notably short for these jobs. The median time is 4.08 days for Build jobs (Table \ref{tab:build_trans_short}) and 2.93 days for Test jobs (Table \ref{tab:test_trans_short}). \amit{need some more rework}

This indicates that developers frequently modify the configuration settings (such as cache paths or keys) for these jobs. The short interval suggests that getting these parameters right often requires repeated adjustments or fine-tuning to ensure the cache works correctly. 
\vspace{0.2cm}

\noindent \textbf{Observation 2.7: \textit{Integration and Release jobs exhibit long intervals between cache maintenance activities.}} In contrast to Build and Test jobs, the maintenance activity of updating parameters ($P\_up \rightarrow P\_up$) happens much less often. The median time between these updates is 87.25 days for Integration jobs (Table \ref{tab:integration_trans_short}) and 61.95 days for Release jobs (Table \ref{tab:release_trans_short}). Furthermore, the time from enabling cache to the first parameter update ($EC \rightarrow P\_up$) in Integration jobs has a median of 203.39 days.

This indicates that cache configurations in these job types are occasionally modified. Unlike Build or Test jobs where changes happen frequently, developers do not often update the cache settings for Integration and Release jobs once they are established.

\vspace{0.2cm}

\noindent \textbf{Observation 2.8: \textit{Sync and Lint jobs show different post-adoption cache maintenance activities.}}  In Sync jobs, the first maintenance activity after enabling the cache ($EC$) is typically a parameter update ($P\_up$), which occurs with a median of 72.96 days (Table \ref{tab:sync_trans_short}). In contrast, Lint jobs are more likely to undergo a cache version update ($C\_up$) after enabling, with a median of 160.59 days (Table \ref{tab:lint_trans_short}).

This indicates that developers managing Sync jobs focus on adjusting configuration settings (such as paths) several months after adoption. Conversely, Lint jobs remain unchanged for a longer period, with the primary maintenance activity being an update to the cache version.
\vspace{0.2cm}

\noindent \textbf{Observation 2.9: \textit{In Integration jobs, cache version updates are mostly followed by parameter updates.}}  In Integration jobs, the transition from updating a cache version to updating parameters ($C\_up \rightarrow P\_up$) has a probability of 90.00\% with a median of 64 days (Table \ref{tab:integration_trans_short}). This indicates that if developers update the cache version, they almost certainly must update the parameters shortly after. This implies integration caches are more sensitive to version changes than build or test caches.
\vspace{0.2cm}

\noindent \textbf{Observation 2.10: \textit{}}  Shortly after enabling cache ($EC$), developers engage in parameter tuning ($EC \rightarrow P\_up$) relatively quickly, with a median of 105.93 days for Build jobs (Table \ref{tab:build_trans_short}). However, the maintenance activity of updating the cache version ($EC \rightarrow C\_up$) occurs after a significantly longer period. It has a median of 270.37 days in Release jobs (Table \ref{tab:release_trans_short}) and 384.02 days in Analyze jobs (Table \ref{tab:analyze_trans_short}).

This indicates that once a stable cache version is adopted, developers are reluctant to change it. While they may tweak how the cache is saved (parameters), they often let the core cache version run for over a year before risking an update.
\amit{How about putting the large tables in appendix and only keep the transition graphs? Currently it's looking too noisy with tables. Need feedback.}
\subsubsection{Build}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/build.png}
    \caption{Transitions of states of build phase \yuan{recheck this caption, as i don't think we generally conclude build phase, we only conclude cache-related maintenance activities for build jobs that once enabled cache. }}
    \label{fig:build_tran}
\end{figure*}

%\usepackage{multirow} % put this in your preamble

%\yuan{make the cache change to cache version update, make the terms consistent}





\begin{table}[h]
\centering
\caption{Build-phase transition statistics (days). Abbreviations: P\_up = Parameter update, P\_add = Parameter added, P\_rm = Parameter removed, C\_up = Cache update, C\_add = Cache added, C\_rm = Cache removed, EC = Enable cache.}
\label{tab:build_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba} & \textbf{Proba (\%)} \\ \hline
T1  & C\_up $\rightarrow$ C\_up             & 177 & 59.56  & 0.00   & 0.00  & 668.08 & 138.32 & 0.78 & 77.63\% \\ \hline
T2  & P\_up $\rightarrow$ P\_up             & 135 & 45.40  & 4.08   & 0.00  & 941.90 & 105.61 & 0.66 & 65.53\% \\ \hline
T3  & EC $\rightarrow$ C\_up                & 69  & 637.14 & 587.98 & 6.35  & 1615.93 & 448.74 & 0.29 & 29.49\% \\ \hline
T4  & EC $\rightarrow$ EC                   & 62  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 0.26 & 26.50\% \\ \hline
T5  & C\_rm $\rightarrow$ C\_rm             & 48  & 13.73  & 0.00   & 0.00  & 390.89 & 66.32  & 0.55 & 55.17\% \\ \hline
T6  & EC $\rightarrow$ P\_up                & 40  & 173.07 & 105.93 & 0.00  & 874.04 & 221.14 & 0.17 & 17.09\% \\ \hline
T7  & EC $\rightarrow$ C\_rm                & 39  & 422.58 & 343.82 & 0.00  & 1514.81 & 428.02 & 0.17 & 16.67\% \\ \hline
T8  & P\_up $\rightarrow$ C\_up             & 31  & 173.03 & 104.80 & 0.00  & 1366.00 & 277.52 & 0.15 & 15.05\% \\ \hline
T9  & C\_up $\rightarrow$ P\_up             & 27  & 148.09 & 79.07  & 0.00  & 592.69 & 179.24 & 0.12 & 11.84\% \\ \hline
T10 & C\_add $\rightarrow$ C\_add           & 26  & 28.03  & 0.00   & 0.00  & 462.91 & 93.91  & 0.35 & 34.67\% \\ \hline
T11 & P\_up $\rightarrow$ C\_rm             & 24  & 152.99 & 43.29  & 0.00  & 902.66 & 222.58 & 0.12 & 11.65\% \\ \hline
T12 & EC $\rightarrow$ C\_add               & 21  & 153.44 & 53.14  & 0.00  & 504.87 & 177.26 & 0.09 & 8.97\% \\ \hline
T13 & C\_add $\rightarrow$ C\_rm            & 19  & 112.31 & 0.00   & 0.00  & 750.21 & 219.41 & 0.25 & 25.33\% \\ \hline
T14 & C\_rm $\rightarrow$ C\_add            & 19  & 47.11  & 0.01   & 0.00  & 445.13 & 105.93 & 0.22 & 21.84\% \\ \hline
T15 & C\_up $\rightarrow$ C\_rm             & 18  & 270.58 & 328.70 & 0.00  & 707.67 & 225.37 & 0.08 & 7.89\% \\ \hline
T16 & C\_add $\rightarrow$ P\_up            & 16  & 106.70 & 51.16  & 0.05  & 419.07 & 132.88 & 0.21 & 21.33\% \\ \hline
T17 & C\_add $\rightarrow$ C\_up            & 14  & 373.24 & 309.69 & 0.00  & 1080.84 & 342.69 & 0.19 & 18.67\% \\ \hline
T18 & P\_up $\rightarrow$ C\_add            & 11  & 25.17  & 4.73   & 1.74  & 177.96 & 52.00  & 0.05 & 5.34\%  \\ \hline
T19 & C\_rm $\rightarrow$ P\_up            & 9   & 55.79  & 30.82  & 0.00  & 321.98 & 101.96 & 0.10 & 10.34\% \\ \hline
T20 & C\_rm $\rightarrow$ C\_up             & 7   & 220.73 & 0.00   & 0.00  & 1374.41 & 510.42 & 0.08 & 8.05\%  \\ \hline
T21 & P\_add $\rightarrow$ C\_up            & 3   & 59.94  & 0.00   & 0.00  & 179.82 & 103.82 & 0.43 & 42.86\% \\ \hline
T22 & P\_rm $\rightarrow$ C\_rm             & 2   & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 0.50 & 50.00\% \\ \hline
T23 & P\_rm $\rightarrow$ P\_up             & 2   & 117.53 & 117.53 & 0.00  & 235.06 & 166.21 & 0.50 & 50.00\% \\ \hline
T24 & P\_add $\rightarrow$ P\_up            & 2   & 3.16   & 3.16   & 0.00  & 6.31   & 4.46   & 0.29 & 28.57\% \\ \hline
T25 & P\_add $\rightarrow$ P\_add           & 1   & 0.00   & 0.00   & 0.00  & 0.00   & --     & 0.14 & 14.29\% \\ \hline
T26 & P\_add $\rightarrow$ P\_rm            & 1   & 0.00   & 0.00   & 0.00  & 0.00   & --     & 0.14 & 14.29\% \\ \hline
\end{tabular}}
\end{table}


\begin{table}[h]
\centering
\caption{Build-phase transition statistics (days). Abbreviations: P\_up = Parameter update, P\_add = Parameter added, P\_rm = Parameter removed, C\_up = Cache update, C\_add = Cache added, C\_rm = Cache removed, EC = Enable cache.\yuan{i am expectation that the transitions are sorted globally, which is not the case, can we change the design, e.g., adding unnamed row for each cluster and highlight that in caption?}} 
\label{tab:build_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba} & \textbf{Proba (\%)} \\ \hline
T1  & C\_add $\rightarrow$ C\_add           & 26  & 28.03  & 0.00   & 0.00  & 462.91 & 93.91  & 0.35 & 34.67\% \\ \hline
T2  & C\_add $\rightarrow$ C\_rm            & 19  & 112.31 & 0.00   & 0.00  & 750.21 & 219.41 & 0.25 & 25.33\% \\ \hline
T3  & C\_add $\rightarrow$ P\_up            & 16  & 106.70 & 51.16  & 0.05  & 419.07 & 132.88 & 0.21 & 21.33\% \\ \hline
T4  & C\_add $\rightarrow$ C\_up            & 14  & 373.24 & 309.69 & 0.00  & 1080.84 & 342.69 & 0.19 & 18.67\% \\ \hline
T5  & P\_add $\rightarrow$ C\_up            & 3   & 59.94  & 0.00   & 0.00  & 179.82 & 103.82 & 0.43 & 42.86\% \\ \hline
T6  & P\_add $\rightarrow$ P\_up            & 2   & 3.16   & 3.16   & 0.00  & 6.31   & 4.46   & 0.29 & 28.57\% \\ \hline
T7  & P\_add $\rightarrow$ P\_add           & 1   & 0.00   & 0.00   & 0.00  & 0.00   & --     & 0.14 & 14.29\% \\ \hline
T8  & P\_add $\rightarrow$ P\_rm            & 1   & 0.00   & 0.00   & 0.00  & 0.00   & --     & 0.14 & 14.29\% \\ \hline
T9  & C\_up $\rightarrow$ C\_up             & 177 & 59.56  & 0.00   & 0.00  & 668.08 & 138.32 & 0.78 & 77.63\% \\ \hline
T10 & C\_up $\rightarrow$ P\_up             & 27  & 148.09 & 79.07  & 0.00  & 592.69 & 179.24 & 0.12 & 11.84\% \\ \hline
T11 & C\_up $\rightarrow$ C\_rm             & 18  & 270.58 & 328.70 & 0.00  & 707.67 & 225.37 & 0.08 & 7.89\% \\ \hline
T12 & EC $\rightarrow$ C\_up                & 69  & 637.14 & 587.98 & 6.35  & 1615.93 & 448.74 & 0.29 & 29.49\% \\ \hline
T13 & EC $\rightarrow$ EC                   & 62  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 0.26 & 26.50\% \\ \hline
T14 & EC $\rightarrow$ P\_up                & 40  & 173.07 & 105.93 & 0.00  & 874.04 & 221.14 & 0.17 & 17.09\% \\ \hline
T15 & EC $\rightarrow$ C\_rm                & 39  & 422.58 & 343.82 & 0.00  & 1514.81 & 428.02 & 0.17 & 16.67\% \\ \hline
T16 & EC $\rightarrow$ C\_add               & 21  & 153.44 & 53.14  & 0.00  & 504.87 & 177.26 & 0.09 & 8.97\% \\ \hline
T17 & C\_rm $\rightarrow$ C\_rm             & 48  & 13.73  & 0.00   & 0.00  & 390.89 & 66.32  & 0.55 & 55.17\% \\ \hline
T18 & C\_rm $\rightarrow$ C\_add            & 19  & 47.11  & 0.01   & 0.00  & 445.13 & 105.93 & 0.22 & 21.84\% \\ \hline
T19 & C\_rm $\rightarrow$ P\_up             & 9   & 55.79  & 30.82  & 0.00  & 321.98 & 101.96 & 0.10 & 10.34\% \\ \hline
T20 & C\_rm $\rightarrow$ C\_up             & 7   & 220.73 & 0.00   & 0.00  & 1374.41 & 510.42 & 0.08 & 8.05\% \\ \hline
T21 & P\_rm $\rightarrow$ C\_rm             & 2   & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 0.50 & 50.00\% \\ \hline
T22 & P\_rm $\rightarrow$ P\_up             & 2   & 117.53 & 117.53 & 0.00  & 235.06 & 166.21 & 0.50 & 50.00\% \\ \hline
T23 & P\_up $\rightarrow$ P\_up             & 135 & 45.40  & 4.08   & 0.00  & 941.90 & 105.61 & 0.66 & 65.53\% \\ \hline
T24 & P\_up $\rightarrow$ C\_up             & 31  & 173.03 & 104.80 & 0.00  & 1366.00 & 277.52 & 0.15 & 15.05\% \\ \hline
T25 & P\_up $\rightarrow$ C\_rm             & 24  & 152.99 & 43.29  & 0.00  & 902.66 & 222.58 & 0.12 & 11.65\% \\ \hline
T26 & P\_up $\rightarrow$ C\_add            & 11  & 25.17  & 4.73   & 1.74  & 177.96 & 52.00  & 0.05 & 5.34\%  \\ \hline
\end{tabular}}
\end{table}




%\safwat{highlight the interseting the patterns in the table.}

%\subsubsection{Job specific pattern}

Each build job typically begins with \textit{enable cache}, after which developers either move on to updating cache contents or tuning related parameters. Over time, maintenance activity is reflected in repeated cache updates and parameter changes.
\yuan{usually the finding numbering is continuous}



\noindent \textbf{Findings 1:} \yuan{We should make it clear why we want to group them based on fast/slow transition, when we identify findings for RQ2, we follow a specific systematic approach? if so, can we put them in RQ2's approach} Several transitions show developers making multiple related changes\yuan{what do you mean by related changes? i feel you mean continue the same activity, A to A, B to B.} in quick succession, often within the same commit or day (median = 0 days). \textbf{The transition C\_up → C\_up (T1) is the most frequent in the entire dataset (Count=177) and has a very high probability (77.63\%).}\yuan{why this is related to your finding 1?.} The median of 0 days indicates that when a developer updates one cache, they frequently update others in the same session. The high mean (59.56) and std (138.32) reveal that despite this common batching behavior, there are occasional, very long gaps between update cycles that pull the average up. \textbf{Similarly, P\_up → P\_up (T2) has a high probability (65.53\%) and a low median of 4.08 days.} However, the massive gap between the median (4.08 days) and mean (45.40 days), coupled with a high standard deviation (105.61), points to a bimodal behavior. Most parameter edits happen in quick succession, but a significant number occur after long periods of stability, suggesting major reconfigurations or infrequent maintenance.

\noindent \textbf{Findings 2:} Transitions starting from Enable Cache (EC) often lead to significant actions\yuan{what does significant action mean?} after very long delays. \textbf{The most likely action after enabling a cache is EC → C\_up (T3, 29.49\% probability) \yuan{inconsistent as you show a transition pattern after "is", which we expect a target status, i.e., C\_up}.} However, the median delay of 587.98 days (over 1.5 years) shows that the first version update is not immediate maintenance but a long-term event. The high mean (637.14) and standard deviation (448.74) confirm that while most delays are long, there is wide variability, with some updates happening much sooner or later than the median. \textbf{A significant finding\yuan{what do you mean by significant finding} is that enabling a cache has a 16.67\% probability of ending in removal EC → C\_rm (T7).} The median delay of 343.82 days (almost a year) indicates this is not a quick experiment but a deliberate decision made after substantial real-world use. The high standard deviation (428.02) suggests this reassessment happens at highly variable times across different projects. \yuan{why not put the below sentence as the finding}\textbf{The data shows that after setting up a cache, developers are more likely to eventually update it (29.49\%) than to remove it (16.67\%)}, but removal is a non-trivial outcome. The long delays for both actions highlight that the true effectiveness and overhead of a cache strategy are often only understood after a prolonged period.



\noindent \textbf{Finding 3:} \textbf{Cache additions and removals are sometimes reversed instantly.} The bi-transitions between C\_add and C\_rm (T13, T14) have medians of 0 days, showing that developers sometimes add a cache configuration and remove it (or vice-versa) in the same commit or within a single day. This is a clear signal of rapid experimentation or correcting a mistaken configuration.












\noindent \textbf{Finding 4:} \yuan{this is also about what happens after enabling, why we need to highlight it separately, and whether we really need to highlight it?} We also noticed updating cache parameters after enabling the cache for the very first time (T6). The median time 105 days suggest developers changed the parameters near after three months. 



% \noindent \textbf{Finding 7:}  We noticed some quick patterns. Developers quickly added caching after removing (T12).

\yuan{i feel finding 5 and 6 are similar, not sure why they are insightful}
\noindent \textbf{Finding 5:} Transitions from cache additions to updates (\textit{T17}) occur after long delays (median = 310 days). This suggests that developers first add new cache, let them run for a while, and only later revisit to update versions.



\noindent \textbf{Finding 6:} The link from C\_add to P\_up (T16) is much quicker (51 days) than the link from C\_add to C\_up (T17, 310 days). This reveals a lifecycle. A new cache is first tuned (parameter changes), then left alone, and only much later updated (version changes).












\subsubsection{Test}



\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/test.png}
    \caption{Transitions of states of test phase}
    \label{fig:test_tran}
\end{figure}



\begin{table}[h]
\centering
\caption{Transitions of states in the test phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache).}
\label{tab:test_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 142 & 62.75  & 2.93   & 0.00  & 986.95  & 156.46 & 0.66  & 66.05 \\ \hline
T2  & C\_up $\rightarrow$ C\_up             & 114 & 58.67  & 0.00   & 0.00  & 713.59  & 137.94 & 0.68  & 68.26 \\ \hline
T3  & C\_add $\rightarrow$ C\_add           & 48  & 24.83  & 0.00   & 0.00  & 463.22  & 93.51  & 0.36  & 36.09 \\ \hline
T4  & EC $\rightarrow$ P\_up                & 45  & 263.33 & 85.03  & 0.00  & 981.44  & 347.74 & 0.24  & 24.32 \\ \hline
T5  & C\_rm $\rightarrow$ C\_rm             & 44  & 39.12  & 0.00   & 0.00  & 448.01  & 105.53 & 0.42  & 41.51 \\ \hline
T6  & C\_add $\rightarrow$ C\_rm            & 42  & 112.53 & 32.49  & 0.00  & 485.66  & 152.93 & 0.32  & 31.58 \\ \hline
T7  & EC $\rightarrow$ C\_up                & 41  & 515.49 & 351.05 & 0.20  & 1549.93 & 457.35 & 0.22  & 22.16 \\ \hline
T8  & EC $\rightarrow$ EC                   & 38  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.21  & 20.54 \\ \hline
T9  & C\_up $\rightarrow$ P\_up             & 33  & 76.46  & 0.00   & 0.00  & 433.71  & 120.17 & 0.20  & 19.76 \\ \hline
T10 & C\_rm $\rightarrow$ C\_add            & 32  & 21.35  & 0.00   & 0.00  & 445.13  & 80.79  & 0.30  & 30.19 \\ \hline
T11 & P\_up $\rightarrow$ C\_up             & 31  & 111.24 & 31.50  & 0.00  & 584.03  & 152.83 & 0.14  & 14.42 \\ \hline
T12 & EC $\rightarrow$ C\_rm                & 30  & 243.13 & 120.77 & 0.00  & 1271.64 & 304.07 & 0.16  & 16.22 \\ \hline
T13 & EC $\rightarrow$ C\_add               & 29  & 172.12 & 41.97  & 0.01  & 962.46  & 243.45 & 0.16  & 15.68 \\ \hline
T14 & C\_add $\rightarrow$ P\_up            & 21  & 105.59 & 8.47   & 0.00  & 973.79  & 219.12 & 0.16  & 15.79 \\ \hline
T15 & P\_up $\rightarrow$ C\_rm             & 19  & 221.16 & 7.24   & 0.00  & 1154.81 & 393.51 & 0.09  & 8.84  \\ \hline
T16 & P\_up $\rightarrow$ C\_add            & 16  & 64.67  & 43.66  & 0.00  & 323.27  & 85.87  & 0.07  & 7.44  \\ \hline
T17 & C\_add $\rightarrow$ C\_up            & 15  & 340.95 & 231.83 & 0.01  & 1294.85 & 356.57 & 0.11  & 11.28 \\ \hline
T18 & C\_up $\rightarrow$ C\_rm             & 12  & 150.41 & 94.56  & 0.00  & 435.59  & 148.67 & 0.07  & 7.19  \\ \hline
T19 & C\_rm $\rightarrow$ P\_rm             & 10  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.09  & 9.43  \\ \hline
T20 & C\_rm $\rightarrow$ P\_up             & 9   & 85.85  & 13.21  & 0.00  & 584.88  & 189.00 & 0.08  & 8.49  \\ \hline
T21 & P\_rm $\rightarrow$ C\_add            & 8   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.62  & 61.54 \\ \hline
T22 & C\_rm $\rightarrow$ C\_up             & 8   & 265.57 & 269.97 & 0.00  & 557.51  & 180.03 & 0.08  & 7.55  \\ \hline
T23 & C\_add $\rightarrow$ P\_add           & 7   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.05  & 5.26  \\ \hline
T24 & P\_add $\rightarrow$ C\_add           & 5   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.28  & 27.78 \\ \hline
T25 & P\_add $\rightarrow$ P\_up            & 5   & 186.87 & 140.78 & 0.00  & 628.32  & 257.22 & 0.28  & 27.78 \\ \hline
T26 & P\_rm $\rightarrow$ C\_rm             & 3   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.23  & 23.08 \\ \hline
T27 & P\_add $\rightarrow$ P\_add           & 3   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.17  & 16.67 \\ \hline
T28 & P\_add $\rightarrow$ C\_up            & 3   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.17  & 16.67 \\ \hline
T29 & P\_rm $\rightarrow$ C\_up             & 2   & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 0.15  & 15.38 \\ \hline
T30 & P\_add $\rightarrow$ C\_rm            & 1   & 875.94 & 875.94 & 875.94& 875.94  & -      & 0.06  & 5.56  \\ \hline
T31 & P\_add $\rightarrow$ EC               & 1   & 0.00   & 0.00   & 0.00  & 0.00    & -      & 0.06  & 5.56  \\ \hline
\end{tabular}
}
\end{table}

\yuan{i do expect a similar summary for figure 4, like what you did for build, cause findings are all around direct transition patterns rather than global view}

\noindent \textbf{Finding 1:} \textbf{Test jobs exhibit identical\yuan{which one? be specific. this seems to go beyond finding 1? then why we put it as the summary sentence for finding1} maintenance behaviors to build jobs.} Being a popular job (described in RQ2), regular parameter maintenance and up to date cache versions seems like a frequent step. \textbf{P\_up → P\_up} shows a high probability (66.05\%) and very low median (2.93 days), confirming that parameter tuning happens very quickly. However, the massive gap between median and mean (62.75 days), plus the high standard deviation (156.46), reveals that most changes happen within days, while occasional major reconfigurations occur after much longer periods. \textbf{Similarly, C\_up → C\_up} has the highest probability (68.26\%) and a median of 0 days, indicating cache version updates are typically happen r in the same commit. The mean (58.67 days) and standard deviation (137.94) again show this pattern is occasionally interrupted by long update cycles.

\textbf{Finding 2:} \textbf{After enabling cache, test jobs follow different paths with significantly different timing patterns.} \yuan{is this the same or different from build? should we just highlight the differences in other findings? maybe finding 1 summary all similar patterns. I could not tell what are surprising new findings in test job analysis}

- T13 shows the pattern of adding new cache in the configuration files with 15.68\% probability and a relatively quick median of 41.97 days. This suggests developers often expand their cache configuration within weeks of initial setup. However, the high mean (172.12 days) and standard deviation (243.45) indicate some teams delay this expansion significantly.


- T4 shows parameter updates after enabling the caching and happens 24.32\% of the time with a median of 85.03 days, notably quicker than the build phase equivalent. 


- T7 shows the version change of caching. Developers relies on version so very long time (median 351 days).











\noindent \textbf{Finding 4:} \textbf{We also noticed cache removal patterns.} T6 represents cache removal after adding a new cache. This process took around 32 days. This indicates developers often get rid of unused/ extra caching techniques.


\noindent \textbf{Finding 5:} \textbf{Interestingly, we found cache removals after enabling the caching (T12).} with 16.22\% probability and a median of 120.77 days, much sooner than the 343 days observed in build jobs.This indicates developers might find the caching not useful enough. 

\noindent \textbf{Finding 6.} After adding cache, developers either: (i) update parameters relatively soon \emph{(T14, median = 8.47 days)}, or (ii) defer version updates for much longer \emph{(T17, median = 231.83 days)}.




\subsubsection{Integration}





\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/integration.png}
    \caption{Transitions of states of integration phase}
    \label{fig:inte_trans}
\end{figure}









\begin{table}[h]
\centering
\caption{Transitions of states of integration phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:integration_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 25 & 137.45 & 87.25  & 13.03 & 538.19 & 124.44 & 67.57 \\ \hline
T2  & P\_up $\rightarrow$ C\_up             & 10 & 235.11 & 141.92 & 0.00  & 1366.00 & 405.25 & 27.03 \\ \hline
T3  & C\_up $\rightarrow$ P\_up             & 9  & 78.27  & 64.22  & 0.00  & 292.84 & 97.34  & 90.00 \\ \hline
T4  & EC $\rightarrow$ P\_up                & 8  & 180.66 & 203.39 & 0.00  & 300.88 & 91.09  & 50.00 \\ \hline
T5  & C\_rm $\rightarrow$ C\_add            & 4  & 19.20  & 0.00   & 0.00  & 76.79  & 38.39  & 80.00 \\ \hline
T6  & C\_add $\rightarrow$ C\_rm            & 4  & 82.21  & 1.54   & 0.00  & 325.75 & 162.37 & 50.00 \\ \hline
T7  & EC $\rightarrow$ C\_up                & 3  & 474.73 & 326.13 & 273.13& 824.91 & 304.42 & 18.75 \\ \hline
T8  & EC $\rightarrow$ C\_rm                & 3  & 184.33 & 252.89 & 46.30 & 253.81 & 119.54 & 18.75 \\ \hline
T9  & C\_add $\rightarrow$ C\_add           & 2  & 5.21   & 5.21   & 0.00  & 10.42  & 7.37   & 25.00 \\ \hline
T10 & EC $\rightarrow$ C\_add               & 2  & 438.48 & 438.48 & 261.21& 615.76 & 250.70 & 12.50 \\ \hline
T11 & P\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 100.00 \\ \hline
T12 & P\_add $\rightarrow$ C\_up            & 1  & 584.03 & 584.03 & 584.03& 584.03 & 0.00   & 50.00 \\ \hline
T13 & P\_add $\rightarrow$ P\_up            & 1  & 161.81 & 161.81 & 161.81& 161.81 & 0.00   & 50.00 \\ \hline
T14 & C\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 20.00 \\ \hline
T15 & C\_add $\rightarrow$ C\_up            & 1  & 584.03 & 584.03 & 584.03& 584.03 & 0.00   & 12.50 \\ \hline
T16 & C\_add $\rightarrow$ P\_up            & 1  & 8.47   & 8.47   & 8.47  & 8.47   & 0.00   & 12.50 \\ \hline
T17 & C\_up $\rightarrow$ C\_rm             & 1  & 285.92 & 285.92 & 285.92& 285.92 & 0.00   & 10.00 \\ \hline
\end{tabular}
}
\end{table}


% \safwat{make another table like category in the job speciifc table. }

% \safwat{pr, issue, in every event. }

% \safwat{TODO: how many evidence we ahve for the transion, see the in the stack overflow}

%\subsubsection{Job specific pattern}
\yuan{missing summary for figure 5}
Integration phase show similar dominat patterns (T1 and T2) with slower cadence than test/build. Teams tend to (i) keep tuning parameters regularly, (ii) occasionally move between parameter and version updates.

\noindent \textbf{Finding 1:} \textbf{For integration phase, the most frequent transition is T1 (P\_up $\rightarrow$ P\_up). This represents regular cache maintenance.} Among all transitions that start at parameter changed within integration jobs, about 67.6\% of the time the next state is parameter changed again.  However, the median of 87.25 days (vs. 4 days in build and 3 days in test) reveals a dramatically slower tuning cycle. 

\noindent \textbf{Finding 2:} Caching is a evolving mechanism\yuan{i think the whole RQ2 is about evolving}. Developers publish new versions of caching with a lot of improvements. After maintain the cache related settings for a while developers often update the cache versions (pattern T2). 
P\_up → C\_up occurs with 27.03\% probability and a median of 141.92 days, showing that parameter changes eventually lead to cache version updates about every 5 months\yuan{i think this is a trigger analysis}. The extremely high standard deviation (405.25) and maximum (1366 days) indicate enormous variability in this cycle.

% The median time 141 days indicates that it takes around 5 months to update the cache version which is followed by a parameter settings changed. The larger mean again reflects right-skew, suggesting occasional much-later cache updates.



\noindent \textbf{Finding 3:} T3 makes sense as after updating the versions, in order to maintain the cache, developers update the parameters within them. Developers usually take 64 days after the cache update to perform a parameter update. 



\noindent \textbf{Finding 4:} T4 represents the transitions that start at enable cache within integration jobs, about 50.0\% of the time the next state is parameter changed. When that happens, it typically occurs 6–7 months later (median = 203.39 days; mean = 180.66 days). \textbf{This refers that developers often relies on their initial cache settings for months.}

\noindent \textbf{Finding 5:} We also noticed other different patterns described in table \ref{tab:integration_trans_short}. T5 represents the immediate cache adoptions right after removing cache. We also noticed cache settings removal after adding the cache. The median time 1.54 days suggests that developers might removed caching after adding a new one. 



\subsubsection{Release}



\begin{table}[h]
\centering
\caption{Transitions of states of release phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:release_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 30 & 90.86  & 61.95  & 0.00  & 311.97 & 86.46  & 63.83 \\ \hline
T2  & EC $\rightarrow$ C\_rm                & 18 & 273.29 & 85.34  & 0.00  & 1170.03& 377.79 & 33.96 \\ \hline
T3  & C\_up $\rightarrow$ C\_up             & 13 & 137.12 & 0.00   & 0.00  & 520.81 & 200.97 & 50.00 \\ \hline
T4  & EC $\rightarrow$ C\_up                & 13 & 445.71 & 270.37 & 0.25  & 1298.49& 473.25 & 24.53 \\ \hline
T5  & EC $\rightarrow$ P\_up                & 12 & 203.64 & 125.98 & 0.00  & 512.00 & 197.30 & 22.64 \\ \hline
T6  & P\_up $\rightarrow$ C\_up             & 11 & 166.19 & 137.67 & 0.00  & 557.50 & 153.70 & 23.40 \\ \hline
T7  & C\_rm $\rightarrow$ C\_rm             & 10 & 14.50  & 0.00   & 0.00  & 145.03 & 45.86  & 55.56 \\ \hline
T8  & C\_up $\rightarrow$ P\_up             & 8  & 70.56  & 18.06  & 0.00  & 292.02 & 107.20 & 30.77 \\ \hline
T9  & C\_rm $\rightarrow$ C\_add            & 6  & 74.19  & 0.00   & 0.00  & 445.13 & 181.73 & 33.33 \\ \hline
T10 & EC $\rightarrow$ C\_add               & 5  & 71.33  & 11.93  & 1.08  & 309.99 & 133.69 & 9.43  \\ \hline
T11 & EC $\rightarrow$ EC                   & 5  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 9.43  \\ \hline
T12 & C\_add $\rightarrow$ C\_add           & 4  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 33.33 \\ \hline
T13 & C\_add $\rightarrow$ C\_up            & 4  & 150.73 & 117.86 & 0.04  & 367.15 & 172.97 & 33.33 \\ \hline
T14 & C\_up $\rightarrow$ C\_rm             & 4  & 371.48 & 429.10 & 34.54 & 593.18 & 238.07 & 15.38 \\ \hline
T15 & P\_up $\rightarrow$ C\_rm             & 4  & 91.89  & 85.88  & 59.81 & 135.99 & 31.95  & 8.51  \\ \hline
T16 & C\_add $\rightarrow$ C\_rm            & 2  & 0.49   & 0.49   & 0.00  & 0.99   & 0.70   & 16.67 \\ \hline
T17 & P\_add $\rightarrow$ C\_up            & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 100.00\\ \hline
T18 & C\_add $\rightarrow$ P\_add           & 1  & 0.42   & 0.42   & 0.42  & 0.42   & 0.00   & 8.33  \\ \hline
T19 & C\_add $\rightarrow$ P\_up            & 1  & 55.04  & 55.04  & 55.04 & 55.04  & 0.00   & 8.33  \\ \hline
T20 & C\_rm $\rightarrow$ C\_up             & 1  & 35.09  & 35.09  & 35.09 & 35.09  & 0.00   & 5.56  \\ \hline
T21 & C\_rm $\rightarrow$ P\_up             & 1  & 36.92  & 36.92  & 36.92 & 36.92  & 0.00   & 5.56  \\ \hline
\end{tabular}
}
\end{table}



\noindent \textbf{Finding 1:} \textbf{T1 is the most frequent transition.}\yuan{this is straightforward...not a meaningful summary} This represents a steady rhythm of caching parameter maintenance to ensure release activities.


\noindent \textbf{Finding 2:}: T2 represents enable\_cache → removing\_cache is the second most frequent transition (33.96\% probability) with a median of 85.34 days. This suggests teams give caches a full quarter to prove value before removal in production. The huge standard deviation (377.79) and maximum (1170 days) show some caches persist for years before being deemed unnecessary.

\noindent \textbf{Finding 3:} Version updates of caching happens mostly in the same commits (T3). However, the higher mean (137.12 days) and maximum (520.81 days) compared to test phase indicate longer intervals. 

\noindent \textbf{Finding 4:} Developers tend to stay on a specific cache versions (T4) after enabling the cache for the first time. The median time 270.37 days reflects the trust towards the version. 

\noindent \textbf{Finding 5:} T15 represents adding\_cache → removing\_cache shows a median of just 0.49 days, indicating some cache additions are reverted almost immediately in release environments, likely due to immediate performance issues or compatibility problems.




\subsubsection{Lint}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/lint.png}
    \caption{Transition diagram of lint phase}
    \label{fig:lint_trans}
\end{figure}






\begin{table}[h]
\centering
\caption{Transitions of states of lint phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:lint_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & EC $\rightarrow$ C\_up                & 11 & 476.04 & 160.59 & 0.01  & 1413.24 & 530.04 & 47.83 \\ \hline
T2  & P\_up $\rightarrow$ C\_up             & 8  & 244.19 & 134.07 & 11.38 & 648.94  & 247.46 & 44.44 \\ \hline
T3  & P\_up $\rightarrow$ P\_up             & 8  & 116.10 & 103.77 & 27.75 & 263.80  & 83.99  & 44.44 \\ \hline
T4  & C\_up $\rightarrow$ C\_up             & 8  & 188.50 & 190.79 & 0.00  & 508.01  & 185.58 & 38.10 \\ \hline
T5  & C\_rm $\rightarrow$ C\_rm             & 7  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 58.33 \\ \hline
T6  & C\_up $\rightarrow$ P\_up             & 7  & 60.67  & 0.03   & 0.00  & 224.30  & 88.67  & 33.33 \\ \hline
T7  & EC $\rightarrow$ C\_rm                & 4  & 428.71 & 340.82 & 115.27& 917.91  & 382.73 & 17.39 \\ \hline
T8  & EC $\rightarrow$ P\_up                & 4  & 263.36 & 99.76  & 23.89 & 830.04  & 380.50 & 17.39 \\ \hline
T9  & C\_add $\rightarrow$ C\_add           & 3  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 42.86 \\ \hline
T10 & P\_add $\rightarrow$ C\_up            & 2  & 814.58 & 814.58 & 263.15& 1366.00 & 779.83 & 50.00 \\ \hline
T11 & P\_rm $\rightarrow$ C\_up             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 50.00 \\ \hline
T12 & P\_rm $\rightarrow$ C\_rm             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 50.00 \\ \hline
T13 & C\_add $\rightarrow$ C\_up            & 2  & 201.12 & 201.12 & 35.09 & 367.15  & 234.80 & 28.57 \\ \hline
T14 & C\_rm $\rightarrow$ C\_add            & 2  & 222.57 & 222.57 & 0.00  & 445.13  & 314.76 & 16.67 \\ \hline
T15 & C\_rm $\rightarrow$ P\_rm             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 16.67 \\ \hline
T16 & P\_up $\rightarrow$ C\_rm             & 2  & 535.55 & 535.55 & 202.90& 868.20  & 470.44 & 11.11 \\ \hline
T17 & C\_up $\rightarrow$ C\_rm             & 2  & 2.04   & 2.04   & 0.00  & 4.08    & 2.88   & 9.52  \\ \hline
T18 & C\_up $\rightarrow$ P\_rm             & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 9.52  \\ \hline
T19 & EC $\rightarrow$ EC                   & 2  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 8.70  \\ \hline
T20 & P\_add $\rightarrow$ C\_add           & 1  & 89.77  & 89.77  & 89.77 & 89.77   & 0.00   & 25.00 \\ \hline
T21 & P\_add $\rightarrow$ P\_up            & 1  & 0.15   & 0.15   & 0.15  & 0.15    & 0.00   & 25.00 \\ \hline
T22 & C\_add $\rightarrow$ P\_add           & 1  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 14.29 \\ \hline
T23 & C\_add $\rightarrow$ C\_rm            & 1  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 14.29 \\ \hline
T24 & C\_rm $\rightarrow$ C\_up             & 1  & 0.00   & 0.00   & 0.00  & 0.00    & 0.00   & 8.33  \\ \hline
\end{tabular}
}
\end{table}




\noindent \textbf{Finding 1:} \textbf{Lint phase shows different dominate pattern.} After enabling caching for the very first time (T1), developers tend to update the version after around 160 days. The massive standard deviation (530.04) and maximum (1413 days) reveal two distinct behaviors. Some teams update within 5-6 months, while others run the same cache version for nearly 4 years. 

\noindent \textbf{Finding 2:} Parameters are maintained, but not as tightly as test/build. (T3)


\noindent \textbf{Finding 3:} The second most frequent pattern updating\_parameter → cache\_version\_update happens with 44.44\% probability and a median of 134.07 days, showing parameter changes eventually lead to version updates about every 4-5 month.



\subsubsection{Analyze}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/analyze.png}
    \caption{Transition diagram of analyze phase}
    \label{fig:tran_analyze}
\end{figure}







\begin{table}[h]
\centering
\caption{Transitions of states of analyze phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:analyze_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & P\_up $\rightarrow$ P\_up             & 46 & 120.01 & 26.14  & 0.20 & 611.55 & 173.33 & 92.00 \\ \hline
T2  & EC $\rightarrow$ P\_up                & 19 & 151.56 & 94.53  & 0.01 & 369.06 & 133.79 & 54.29 \\ \hline
T3  & EC $\rightarrow$ C\_up                & 10 & 517.14 & 384.02 & 0.01 & 1549.93 & 542.26 & 28.57 \\ \hline
T4  & C\_up $\rightarrow$ C\_up             & 6  & 199.45 & 190.42 & 0.00 & 431.84 & 218.27 & 60.00 \\ \hline
T5  & C\_rm $\rightarrow$ C\_rm             & 5  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 50.00 \\ \hline
T6  & C\_rm $\rightarrow$ C\_add            & 4  & 56.72  & 3.91   & 0.00 & 219.07 & 108.25 & 40.00 \\ \hline
T7  & C\_add $\rightarrow$ C\_rm            & 3  & 251.84 & 250.30 & 119.62 & 385.59 & 132.99 & 50.00 \\ \hline
T8  & EC $\rightarrow$ C\_rm                & 3  & 196.91 & 3.48   & 0.01 & 587.24 & 338.04 & 8.57  \\ \hline
T9  & P\_up $\rightarrow$ C\_up             & 3  & 269.95 & 257.62 & 0.00 & 552.24 & 276.33 & 6.00  \\ \hline
T10 & C\_add $\rightarrow$ C\_up            & 2  & 250.48 & 250.48 & 0.00 & 500.96 & 354.23 & 33.33 \\ \hline
T11 & C\_up $\rightarrow$ C\_add            & 2  & 7.10   & 7.10   & 0.00 & 14.21  & 10.05  & 20.00 \\ \hline
T12 & EC $\rightarrow$ EC                   & 2  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 5.71  \\ \hline
T13 & P\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 100.00 \\ \hline
T14 & C\_add $\rightarrow$ P\_up            & 1  & 217.80 & 217.80 & 217.80 & 217.80 & 0.00   & 16.67 \\ \hline
T15 & C\_up $\rightarrow$ C\_rm             & 1  & 4.08   & 4.08   & 4.08 & 4.08   & 0.00   & 10.00 \\ \hline
T16 & C\_up $\rightarrow$ P\_up             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 10.00 \\ \hline
T17 & C\_rm $\rightarrow$ P\_rm             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 10.00 \\ \hline
\end{tabular}
}
\end{table}


\noindent \textbf{Finding 1:} The most dominant transition is T1 (P\_up $\rightarrow$ P\_up) and developers usually updates the parameters in 26 days. This shows monthly tuning cycles, but the massive gap between median and mean (120.01 days) and high standard deviation (173.33) reveals  frequent minor adjustments and occasional major reconfigurations after much longer periods (up to 611.55 days).

\noindent \textbf{Finding 2:} Around 94 days after first enabling the cache, developers tend to change cache related parameters. This 3-month parameter tuning cycle suggests analyze caches require significant calibration after initial setup.

\noindent \textbf{Finding 3:} Developers tend to stay in their initial cache versions for 384.02 days after enabling cache (T3). The enormous standard deviation (542.26) and maximum (1549.93 days) reveal that some analyze cache versions run for more than 4 years without updates.

\noindent \textbf{Finding 4:} T4 represents that version updates happen nearly after 190 days. Analyze jobs hold versions steady longer than test/integration/release phases.




\subsubsection{Linux}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/linux.png}
    \caption{Transition diagram of linux phase}
    \label{fig:linux_trans}
\end{figure}


\begin{table}[h]
\centering
\caption{Transitions of states of linux phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:linux_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1 & C\_up $\rightarrow$ C\_up          & 4 & 230.93 & 196.61 & 0.00  & 530.50 & 272.48 & 80.00 \\ \hline
T2 & EC $\rightarrow$ C\_up              & 4 & 452.34 & 476.09 & 15.77 & 841.42 & 442.51 & 57.14 \\ \hline
T3 & P\_up $\rightarrow$ P\_up           & 3 & 191.71 & 200.53 & 110.81& 263.80 & 76.88  & 60.00 \\ \hline
T4 & P\_up $\rightarrow$ C\_up           & 2 & 150.85 & 150.85 & 104.80& 196.90 & 65.13  & 40.00 \\ \hline
T5 & EC $\rightarrow$ C\_add             & 2 & 71.45  & 71.45  & 0.96  & 141.95 & 99.70  & 28.57 \\ \hline
T6 & C\_add $\rightarrow$ C\_up          & 1 & 282.87 & 282.87 & 282.87& 282.87 & 0.00   & 100.00 \\ \hline
T7 & C\_up $\rightarrow$ P\_up           & 1 & 210.97 & 210.97 & 210.97& 210.97 & 0.00   & 20.00 \\ \hline
T8 & EC $\rightarrow$ P\_up              & 1 & 133.90 & 133.90 & 133.90& 133.90 & 0.00   & 14.29 \\ \hline
\end{tabular}
}
\end{table}


\noindent \textbf{Finding 1:} The most dominant pattern T1 represents cache version update which is a vital part of software maintenance. The median time 196 days reflects the reliance of cache versions. While adding new cache is present (T5), but while updating the versions (T2) after enabling the cache for the first time, developers take more than 1 year. 


\subsubsection{Sync}

\begin{figure} [h]
    \centering
    \includegraphics[width=\linewidth]{figures/sync.png}
    \caption{Transition diagram of sync phase}
    \label{fig:trans_sync}
\end{figure}



\begin{table}[h]
\centering
\caption{Transitions of states of sync phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
\label{tab:sync_trans_short}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|r|r|r|r|r|r|r|}
\hline
\textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
T1  & EC $\rightarrow$ P\_up                & 28 & 250.33 & 72.96  & 0.00 & 693.07 & 284.48 & 90.32 \\ \hline
T2  & P\_up $\rightarrow$ P\_up             & 18 & 409.30 & 288.65 & 0.69 & 698.58 & 220.85 & 48.65 \\ \hline
T3  & C\_add $\rightarrow$ C\_add           & 11 & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 45.83 \\ \hline
T4  & C\_add $\rightarrow$ P\_up            & 11 & 108.01 & 8.47   & 7.78 & 685.42 & 209.03 & 45.83 \\ \hline
T5  & P\_up $\rightarrow$ C\_rm             & 11 & 115.62 & 13.15  & 7.07 & 244.66 & 123.56 & 29.73 \\ \hline
T6  & P\_rm $\rightarrow$ C\_add            & 6  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 54.55 \\ \hline
T7  & C\_rm $\rightarrow$ P\_rm             & 6  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 46.15 \\ \hline
T8  & P\_rm $\rightarrow$ C\_rm             & 5  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 45.45 \\ \hline
T9  & C\_rm $\rightarrow$ C\_add            & 5  & 0.00   & 0.00   & 0.00 & 0.01  & 0.00   & 38.46 \\ \hline
T10 & P\_up $\rightarrow$ P\_rm             & 4  & 23.02  & 7.07   & 7.07 & 70.85  & 31.89  & 10.81 \\ \hline
T11 & C\_up $\rightarrow$ P\_up             & 2  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 100.00 \\ \hline
T12 & EC $\rightarrow$ C\_rm                & 2  & 52.97  & 52.97  & 3.99 & 101.94 & 69.26  & 6.45  \\ \hline
T13 & P\_up $\rightarrow$ C\_add            & 2  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 5.41  \\ \hline
T14 & P\_add $\rightarrow$ C\_add           & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 50.00 \\ \hline
T15 & P\_add $\rightarrow$ C\_up            & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 50.00 \\ \hline
T16 & C\_rm $\rightarrow$ C\_rm             & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 7.69  \\ \hline
T17 & C\_rm $\rightarrow$ P\_add            & 1  & 0.00   & 0.00   & 0.00 & 0.00   & 0.00   & 7.69  \\ \hline
\end{tabular}
}
\end{table}








\noindent \textbf{Finding 1:} The most dominant pattern T1, is EC $\rightarrow$ P\_up which represents the reliance on the very first cache settings. developers change the parameters typically in 72 days. The average is 250.33 days, and the standard deviation is 284.48. This indicates that while most parameter updates after enabling cache happen within about 73 days, there are some that take much longer (up to 693 days) which pulls the average up. 

\noindent \textbf{Finding 2:} T2 shows regular parameter updates but the median time is 288 days which is quite long.


% \subsubsection{Others} \amit{I feel we can exclude the 'other' cateogry from here, as we are not focusing on this in next RQs. Requesting suggestion from Yuan and Safwat.} \yuan{yes, we don't need others}

% \begin{table}[h]
% \centering
% \caption{Transitions of states of other phase (abbreviations: P\_up=Parameter update, P\_add=Parameter added, P\_rm=Parameter removed, C\_up=Cache update, C\_add=Cache added, C\_rm=Cache removed, EC=Enable cache)}
% \label{tab:other_trans_short}
% \scriptsize
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|l|r|r|r|r|r|r|r|}
% \hline
% \textbf{ID} & \textbf{Transition} & \textbf{Count} & \textbf{Avg} & \textbf{Med} & \textbf{Min} & \textbf{Max} & \textbf{Std} & \textbf{Proba (\%)} \\ \hline
% T1  & P\_up $\rightarrow$ P\_up             & 99 & 28.39  & 0.00   & 0.00  & 347.11 & 76.40  & 77.34 \\ \hline
% T2  & C\_up $\rightarrow$ C\_up             & 62 & 65.27  & 0.00   & 0.00  & 668.54 & 150.08 & 72.09 \\ \hline
% T3  & C\_add $\rightarrow$ C\_add           & 35 & 16.83  & 0.00   & 0.00  & 300.62 & 53.40  & 54.69 \\ \hline
% T4  & EC $\rightarrow$ C\_up                & 17 & 396.81 & 384.02 & 0.04  & 841.42 & 270.91 & 27.87 \\ \hline
% T5  & C\_add $\rightarrow$ P\_up            & 15 & 107.14 & 27.10  & 0.00  & 460.36 & 154.60 & 23.44 \\ \hline
% T6  & EC $\rightarrow$ C\_rm                & 13 & 98.33  & 17.11  & 0.00  & 424.82 & 136.59 & 21.31 \\ \hline
% T7  & P\_up $\rightarrow$ C\_up             & 12 & 180.42 & 104.80 & 0.00  & 609.79 & 216.23 & 9.38  \\ \hline
% T8  & EC $\rightarrow$ EC                   & 11 & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 18.03 \\ \hline
% T9  & EC $\rightarrow$ C\_add               & 10 & 174.83 & 1.87   & 0.01  & 530.11 & 237.40 & 16.39 \\ \hline
% T10 & P\_rm $\rightarrow$ C\_rm             & 9  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 64.29 \\ \hline
% T11 & C\_rm $\rightarrow$ C\_add            & 9  & 155.73 & 86.31  & 0.00  & 538.67 & 188.81 & 28.12 \\ \hline
% T12 & C\_rm $\rightarrow$ C\_rm             & 9  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 28.12 \\ \hline
% T13 & EC $\rightarrow$ P\_up                & 9  & 75.10  & 39.11  & 0.02  & 209.82 & 76.96  & 14.75 \\ \hline
% T14 & C\_rm $\rightarrow$ P\_rm             & 8  & 23.91  & 0.00   & 0.00  & 191.32 & 67.64  & 25.00 \\ \hline
% T15 & C\_up $\rightarrow$ P\_up             & 8  & 67.18  & 14.03  & 0.00  & 292.84 & 105.38 & 9.30  \\ \hline
% T16 & P\_up $\rightarrow$ C\_add            & 8  & 177.95 & 63.64  & 3.40  & 903.97 & 299.33 & 6.25  \\ \hline
% T17 & C\_up $\rightarrow$ C\_rm             & 7  & 89.71  & 21.07  & 0.27  & 410.12 & 147.65 & 8.14  \\ \hline
% T18 & P\_up $\rightarrow$ C\_rm             & 7  & 29.00  & 2.12   & 0.00  & 88.95  & 37.24  & 5.47  \\ \hline
% T19 & P\_add $\rightarrow$ C\_up            & 5  & 237.34 & 276.54 & 0.00  & 584.03 & 246.11 & 41.67 \\ \hline
% T20 & C\_add $\rightarrow$ C\_up            & 5  & 87.77  & 19.96  & 0.00  & 276.54 & 119.99 & 7.81  \\ \hline
% T21 & C\_add $\rightarrow$ C\_rm            & 5  & 96.02  & 42.58  & 0.00  & 313.87 & 130.32 & 7.81  \\ \hline
% T22 & C\_up $\rightarrow$ P\_add            & 5  & 2.64   & 0.00   & 0.00  & 13.18  & 5.89   & 5.81  \\ \hline
% T23 & P\_add $\rightarrow$ C\_add           & 4  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 33.33 \\ \hline
% T24 & C\_rm $\rightarrow$ P\_up             & 4  & 13.11  & 7.76   & 0.00  & 36.92  & 17.28  & 12.50 \\ \hline
% T25 & P\_rm $\rightarrow$ C\_up             & 2  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 14.29 \\ \hline
% T26 & P\_rm $\rightarrow$ P\_rm             & 2  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 14.29 \\ \hline
% T27 & P\_add $\rightarrow$ P\_add           & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 8.33  \\ \hline
% T28 & P\_add $\rightarrow$ P\_rm            & 1  & 86.94  & 86.94  & 86.94 & 86.94  & 0.00   & 8.33  \\ \hline
% T29 & P\_add $\rightarrow$ P\_up            & 1  & 0.00   & 0.00   & 0.00  & 0.00   & 0.00   & 8.33  \\ \hline
% T30 & P\_rm $\rightarrow$ P\_add            & 1  & 94.21  & 94.21  & 94.21 & 94.21  & 0.00   & 7.14  \\ \hline
% \end{tabular}
% }
% \end{table}

% \begin{figure} [h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/other.png}
%     \caption{Transition diagram of other phase}
%     \label{fig:other_trans}
% \end{figure}




\noindent \textbf{Finding 1:} Two dominant transitions T1 and T2, mostly happen in same commits. This follows similar patterns of build, test jobs. In T2, the higher mean (65.27 days) and standard deviation (150.08) indicate more variability in version update frequency.

\noindent \textbf{Finding 2:} After enabling the cache for the first time, developers adds new cache almost immediately (T9), but while updating them, it shows prolong delay. We also noticed removing caching (T6). 

\section{Cross phase observations}\yuan{i wonder if we should just put this as our findings, others could be in appendix or supplementary}

% Based on the characteristics of the patterns across all phases, we categorize them in three different categorizes to provide cross phase insights. 


% \subsubsection{Maintenance pattern}

\amit{remove the other from section 6, remove the tables to appendix, keep the transition graph as of now, we will see}

\noindent \textbf{Observation 1:} \textbf{Across almost all phases (build, test, integration, release, analyze, other), the most frequent transitions are P\_up $\rightarrow$ P\_up and C\_up $\rightarrow$ C\_up).} This indicates a universal, ongoing maintenance rhythm for caching configurations. \textbf{The median times between transitions vary significantly by phases}, reflecting their different roles and stability requirements in the CI/CD pipeline. We noticed three patterns: 
\begin{itemize}
    \item \textbf{Rapid iteration phases (build, test):} These phases show the quickest cadence. For example, P\_up $\rightarrow$ P\_up has a median of 4.08 days (build) and 2.93 days (test). This aligns with their frequent execution during development, requiring constant tweaks for optimal performance.
    \item \textbf{Slower phases} (integration, release, analyze): These phases exhibit longer cycles. P\_up $\rightarrow$ P\_up has medians of 87.25 days (integration) and 61.95 days (release), while EC $\rightarrow$ P\_up in integration takes a median of 203.39 days. This suggests that configurations in these less-frequently run, more critical pipelines are treated with more caution and are changed less often. 
    \item Specialized Phases (sync, lint): These phases show unique dominant patterns. sync is characterized by an initial parameter tuning phase after enabling cache (EC $\rightarrow$ P\_up, median 72.96 days), while lint is dominated by eventual version updates (EC $\rightarrow$ C\_up, median 160.59 days).


\end{itemize}

%\subsubsection{Action after initial cache adoption}


\noindent \textbf{Observation 2:} \textbf{A common lifecycle pattern is observed after caching is initially enabled (EC).} The subsequent actions reveal a process of refinement and, in some cases, abandonment. 

\begin{itemize}
    \item \textbf{Shortly after enabling cache (EC), developers often engage in parameter tuning (EC → P\_up). }This happens relatively \textbf{quickly}, across phases, with build phase showing median 105.93 days (min 0.00, max 874.04, std 221.14), test phase at median 85.03 days (min 0.00, max 981.44, std 347.74), and integration phase at median 203.39 days (min 0.00, max 300.88, std 91.09). This suggests an initial period of configuration and optimization to get the cache working effectively for a specific job.

    \item \textbf{The transition EC → C\_up is common but occurs after a significantly longer period} (median times: 160.59 days in lint, 270.37 days in release, 384.02 days in analyze and other). This indicates that once a stable cache version is adopted, developers are reluctant to change it, often letting it run for many months or even over a year before updating.

    \item  Unlike other phases where cache updates dominate, sync phase is dominated by EC → P\_up at 90.32\% probability with median 72.96 days (min 0.00, max 693.07, std 284.48), indicating parameter optimization is the primary concern after cache enablement. 


    % \item  \textbf{A notable finding is the tendency to remove cache after it has been enabled, particularly in the release and build phases (EC → C\_rm).} In release, this is the second most frequent transition (T2), happening after a median of 85.34 days. This points to stability or performance issues where caching in critical pipelines like release is deemed more harmful than beneficial after a trial period.
\end{itemize}

%\subsubsection{Cache adding and removing patterns}

\noindent \textbf{Observation 3:} \textbf{A notable finding is the tendency to remove cache after it has been enabled, particularly in the release and build phases (EC → C\_rm).} In release, this is the second most frequent transition (T2), happening after a median of 85.34 days. This points to stability or performance issues where caching in critical pipelines like release is deemed more harmful than beneficial after a trial period.

\noindent \textbf{Observation 3:} \textbf{The transition from Enable Cache (EC) → Cache Added (C\_add) reveals a critical pattern.} After the initial cache adoption, developers don't stop at a single cache configuration. The data shows they frequently add additional caches, but the timing and context vary significantly by phase:

\begin{itemize}
    \item In test jobs, EC → C\_add occurs with a median of 41.97 days. Developers relatively quickly identify additional dependencies or build artifacts that benefit from caching beyond their initial setup.
    \item In build jobs, this transition happens at a similar pace (median 53.14 days), suggesting parallel optimization across complementary phases.


\end{itemize}
\yuan{only observation 4 is specific to a job type?}
\noindent \textbf{Observation 4:} However, in test jobs, we see C\_add → C\_rm with a median of 32.49 days approximately the same timeframe as EC → C\_add. \textbf{This suggests that approximately one month after adding new caches, developers remove them}, indicating that not all cache additions provide sustainable value. 

\noindent \textbf{Observation 5:} \textbf{As per our data, developers tend to stay in their initial cache adoption settings.} We found the fastest expansion in release phase, developers added new cache after 11 days of enabling caching. Test, build and linux phases added new cache after 41, 53, 71 days respectively. Even integration phase added after 438 days.  


% \noindent \textbf{Insight 6:} Unlike other phases where cache updates dominate, sync phase is dominated by EC → P\_up at 90.32\% probability with median 72.96 days (min 0.00, max 693.07, std 284.48), indicating parameter optimization is the primary concern after cache enablement. 






% \begin{tcolorbox}[enhanced,width=4.7in,size=fbox,drop shadow southwest,sharp corners]

% \textbf{RQ2 Summary: Our analysis of caching transitions reveals that developer practices are highly phase-specific. In high-frequency phases like build and test, we observe rapid, iterative tuning of cache parameters and versions. In contrast, critical phases like release and integration exhibit slower, more cautious update cycles, with release showing a significant tendency to remove caches after initial adoption. A common lifecycle emerges: after enabling a cache, developers first refine its parameters before eventually updating its version many months later. Furthermore, caching strategies often expand as developers add new caches to a job, but this is frequently followed by removal, indicating a trial-and-error approach to optimization. These distinct patterns demonstrate that the evolution of cache configurations is not uniform but is instead shaped by the specific role and criticality of each CI/CD phase. } 
% \end{tcolorbox}




\begin{tcolorbox}[enhanced,width=4.7in,size=fbox,drop shadow southwest,sharp corners]
\textbf{RQ2 Summary: Our analysis of caching transitions reveals highly phase-specific developer behavior. High-frequency jobs (\texttt{build}, \texttt{test}) are characterized by rapid, iterative tuning of both parameters and versions. In contrast, other jobs (\texttt{release}, \texttt{integration}) exhibit slower, more cautious update cycles. Notably, a common lifecycle involves enabling a cache, refining its parameters, and only updating its version many months later. This pattern, along with frequent  additions and removals, demonstrates that cache evolution is shaped by the specific demands of each CI/CD phase.}
\end{tcolorbox}

\yuan{no expecation of content after RQ2's answer box, again, motivation for RQ3 should be in RQ3's section}
RQ2 unveils what cache modifications occur and when they happen, revealing distinct, phase-specific patterns. However, these quantitative data points do not explain why developers make these changes. To answer this, RQ3 analyzes the commit messages, PR discussions, and trigger sources to understand the actual motivation driving each transition. This shift from observing what happens to explaining why it happens provides crucial insights into the real-world challenges of cache management and creates a foundation for evidence-based improvements in tooling and practice.

% The patterns uncovered in RQ2 describe the symptoms of cache configuration evolution, but RQ3 investigates the diagnosis. For example, the frequent parameter update cycles (P\_up→P\_up) that dominate most phases could indicate either careful iterative optimization or persistent configuration instability. Similarly, the prolonged delays before cache version updates might reflect either satisfaction with current performance or neglect of dependency maintenance. To distinguish between these competing explanations, RQ3 analyzes the commit messages, PR discussions, and trigger sources to understand the actual motivations driving each transition. This shift from observing what happens to explaining why it happens provides crucial insights into the real-world challenges of cache management and creates a foundation for evidence-based improvements in tooling and practice.








==> rq3_old.tex <==

prev:

RQ2 unveils what cache modifications occur and when they happen, revealing distinct, phase-specific patterns. However, these quantitative data points do not explain why developers make these changes. To answer this, RQ3 analyzes the commit messages, PR discussions, and trigger sources to understand the actual motivation driving each transition. This shift from observing what happens to explaining why it happens provides crucial insights into the real-world challenges of cache management and creates a foundation for evidence-based improvements in tooling and practice.




The quantitative patterns uncovered in RQ2 describe what types of cache transitions happen and when they occur relative to each other within specific CI/CD phases. We observed distinct lifecycles, such as the rapid, iterative tuning of parameters in build and test phases and  slower updates in release phase. However, these patterns alone do not explain the underlying intent. For example, the frequent updating parameters could indicate proactive, careful optimization, or it could signal persistent configuration instability and reactive bug fixing. Similarly, the long delays before a caching version update might reflect satisfaction with current performance or simple neglect of dependency maintenance. 


To move from observation to explanation, this research question investigates the why behind the what. We propose  two parts sub research questions:

\begin{itemize}
    \item \textbf{RQ 3.1: What are the primary targets and patterns of cache evolution? \yuan{RQ2 and RQ3 both discuss about pattern of cache evolution, why it is specific to 3.1}}   This aims to quantify the granular level trends in cache transition. It identifies the dominant target transitions and characterize them with respect to time. \yuan{why this is needed? not really provide the motivation}
 
    \item \textbf{RQ 3.2: What are the underlying drivers and triggers for these cache modifications?}  This aims to provide the qualitative explanation for the patterns identified in RQ3.1. It investigates the intent and the initiators (the triggers, such as 'human' vs. 'bot') of the changes. This allows us to understand why developers make specific cache modifications and explains the root causes of the observed temporal patterns.
\end{itemize}






% While RQ2 findings revealed distinct patterns in how cache configurations evolve across CI/CD phases, understanding why these transitions occur is equally critical. Cache configuration changes represent significant engineering decisions that impact build performance, reliability, and maintenance overhead. Without understanding the drivers behind these changes, we cannot determine whether they represent proactive optimizations based on performance monitoring, reactive fixes to address build failures or security concerns, incidental changes resulting from broader pipeline modifications, automated updates triggered by dependency management bots.

% The trigger source (human vs. bot) provides crucial context for interpreting the temporal patterns observed in RQ2. For instance, a rapid sequence of version updates  could indicate either careful iterative optimization or desperate attempts to update a recent cache. Similarly, long delays between version updates might reflect either satisfaction with current performance or neglect of dependency maintenance.

\subsection{Approach}


For RQ 3.1, to  comprehensively understand caching evolution behaviors, we therefore aggregate transitions by target state, analyzing all source transitions that lead to a given caching action. This approach allows us to understand the full spectrum of motivations driving each type of caching change, represented in Table \ref{tab:rq3}.


For RQ 3.2, to build a taxonomy of these rationales, we conducted a qualitative analysis on a significant random sample (90\% confidence interval and 10\% margin of error) of transitions for each target state. We manually analyzed 86, 87, 77, 28, 79, 32 samples from \textit{cache version update}, \textit{updating parameters}, \textit{adding cache}, \textit{adding parameter}, \textit{removing cache} and \textit{removing parameter} respectively. To capture the full rational behind the change, we focused on \textbf{what} is being changed in code which points out the particular change, \textbf{why} the change is being made explained in pull requests, commits  which indicate the main driver of developer and \textbf{who} is responsible the change (bot/human) which point out the trigger source of the change. 

To structure this analysis, we first refined the high-level target states (e.g., cache version update) into a more granular taxonomy of specific modification actions (e.g., Upgrade, Downgrade). We then used this taxonomy to map the developer's underlying driver. Finally, we cross-reference the quantitative findings from RQ 3.1 with the qualitative taxonomies from RQ 3.2 to find observable patterns to their root causes.



\subsection{Results}

\subsubsection{RQ 3.1: What are the primary targets and temporal patterns of cache evolution?}

Table \ref{tab:rq3} summarizes the quantitative overview of state transitions, aggregated by their target states. This quantitative overview establishes the key phenomena that require qualitative explanation.
\yuan{missing findings from this table, what's the purpose of this table if there is no discussion or findings from it? or it could be combined with 3.2}

% \begin{table}[h]
% \centering
% \caption{Statistics of observed transitions, aggregated by target state}
% \scriptsize
% \label{tab:rq3}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% From                   & To                     & Count & Total & \begin{tabular}[c]{@{}c@{}}Significant\\ sample\end{tabular} & Avg    & Med    & Std    & Min    & Max     & \%    \\ \hline
% cache version update &                        & 378   &       &                                                              & 70.60  & 0.00   & 149.79 & 0.00   & 713.59  & 51.85 \\ \cline{1-1} \cline{6-11} 
% enable cache          &                        & 168   &       &                                                              & 543.33 & 384.13 & 447.09 & 0.01   & 1615.93 & 23.05 \\ \cline{1-1} \cline{6-11} 
% updating parameter    &                        & 104   &       &                                                              & 172.52 & 104.80 & 241.06 & 0.00   & 1366.00 & 14.27 \\ \cline{1-1} \cline{6-11} 
% adding cache          & cache version update & 44    & 745   & 86                                                          & 298.89 & 231.83 & 310.83 & 0.00   & 1294.85 & 6.04  \\ \cline{1-1} \cline{6-11} 
% removing cache        &                        & 18    &       &                                                              & 210.66 & 95.11  & 334.78 & 0.00   & 1374.41 & 2.47  \\ \cline{1-1} \cline{6-11} 
% adding parameter      &                        & 12    &       &                                                              & 179.04 & 0.00   & 392.71 & 0.00   & 1366.00 & 1.65  \\ \cline{1-1} \cline{6-11} 
% removing parameter    &                        & 5     &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 0.69  \\ \hline
% updating parameter    &                        & 497   &       &                                                              & 75.36  & 4.29   & 148.32 & 0.00   & 986.95  & 58.20 \\ \cline{1-1} \cline{6-11} 
% enable cache          &                        & 166   &       &                                                              & 207.31 & 115.90 & 260.34 & 0.00   & 981.44  & 19.44 \\ \cline{1-1} \cline{6-11} 
% cache version update &                        & 92    &       &                                                              & 95.24  & 0.23   & 136.98 & 0.00   & 592.69  & 10.77 \\ \cline{1-1} \cline{6-11} 
% adding cache          & updating parameter    & 66    &       &                                                              & 106.08 & 18.14  & 176.34 & 0.00   & 973.79  & 7.73  \\ \cline{1-1} \cline{6-11} 
% removing cache        &                        & 23    & 854   & 87                                                          & 59.31  & 14.83  & 132.34 & 0.00   & 584.88  & 2.69  \\ \cline{1-1} \cline{6-11} 
% adding parameter      &                        & 8     &       &                                                              & 100.00 & 3.23   & 220.22 & 0.00   & 628.32  & 0.94  \\ \cline{1-1} \cline{6-11} 
% removing parameter    &                        & 2     &       &                                                              & 117.53 & 117.53 & 166.21 & 0.00   & 235.06  & 0.23  \\ \hline
% adding cache          &                        & 129   &       &                                                              & 19.54  & 0.00   & 76.00  & 0.00   & 463.22  & 35.64 \\ \cline{1-1} \cline{6-11} 
% removing cache        &                        & 80    &       &                                                              & 49.43  & 0.00   & 121.76 & 0.00   & 538.67  & 22.10 \\ \cline{1-1} \cline{6-11} 
% enable cache          &                        & 72    &       &                                                              & 158.53 & 46.39  & 212.73 & 0.00   & 962.46  & 19.89 \\ \cline{1-1} \cline{6-11} 
% updating parameter    & adding cache          & 39    & 362   & 77                                                          & 70.13  & 10.86  & 153.92 & 0.00   & 903.97  & 10.77 \\ \cline{1-1} \cline{6-11} 
% cache version update &                        & 18    &       &                                                              & 54.97  & 16.83  & 96.33  & 0.00   & 380.01  & 4.97  \\ \cline{1-1} \cline{6-11} 
% removing parameter    &                        & 14    &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 3.87  \\ \cline{1-1} \cline{6-11} 
% adding parameter      &                        & 10    &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 2.76  \\ \hline
% adding cache          &                        & 11    &       &                                                              & 0.04   & 0.00   & 0.13   & 0.00   & 0.42    & 28.21 \\ \cline{1-1} \cline{6-11} 
% updating parameter    &                        & 9     &       &                                                              & 96.68  & 4.92   & 253.28 & 0.00   & 769.43  & 23.08 \\ \cline{1-1} \cline{6-11} 
% cache version update &                        & 6     &       &                                                              & 2.20   & 0.00   & 5.38   & 0.00   & 13.18   & 15.38 \\ \cline{1-1} \cline{6-11} 
% enable cache          & adding parameter      & 5     & 39    & 28                                                           & 1.01   & 0.00   & 2.27   & 0.00   & 5.07    & 12.82 \\ \cline{1-1} \cline{6-11} 
% adding parameter      &                        & 4     &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 10.26 \\ \cline{1-1} \cline{6-11} 
% removing cache        &                        & 3     &       &                                                              & 57.74  & 0.00   & 100.02 & 0.00   & 173.23  & 7.69  \\ \cline{1-1} \cline{6-11} 
% removing parameter    &                        & 1     &       &                                                              & 94.21  & 94.21  &  0.00    & 94.21  & 94.21   & 2.56  \\ \hline
% removing cache        &                        & 117   &       &                                                              & 21.59  & 0.00   & 79.25  & 0.00   & 448.01  & 26.65 \\ \cline{1-1} \cline{6-11} 
% enable cache          &                        & 111   &       &                                                              & 293.62 & 129.68 & 362.73 & 0.00   & 1514.81 & 25.28 \\ \cline{1-1} \cline{6-11} 
% adding cache          &                        & 76    &       &                                                              & 110.33 & 4.25   & 167.29 & 0.00   & 750.21  & 17.31 \\ \cline{1-1} \cline{6-11} 
% updating parameter    & removing cache        & 69    & 439   & 79                                                          & 168.77 & 43.29  & 270.95 & 0.00   & 1154.81 & 15.72 \\ \cline{1-1} \cline{6-11} 
% cache version update &                        & 45    &       &                                                              & 201.85 & 125.65 & 205.24 & 0.00   & 707.67  & 10.25 \\ \cline{1-1} \cline{6-11} 
% removing parameter    &                        & 20    &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 4.56  \\ \cline{1-1} \cline{6-11} 
% adding parameter      &                        & 1     &       &                                                              & 875.94 & 875.94 & 0.00    & 875.94 & 875.94  & 0.23  \\ \hline
% removing cache        &                        & 26    &       &                                                              & 7.36   & 0.00   & 37.52  & 0.00   & 191.32  & 54.17 \\ \cline{1-1} \cline{6-11} 
% updating parameter    &                        & 10    &       &                                                              & 16.26  & 7.07   & 24.39  & 0.00   & 70.85   & 20.83 \\ \cline{1-1} \cline{6-11} 
% adding cache          &                        & 3     &       &                                                              & 1.09   & 0.00   & 1.89   & 0.00   & 3.27    & 6.25  \\ \cline{1-1} \cline{6-11} 
% cache version update & removing parameter    & 3     &       &                                                              & 57.31  & 0.00   & 99.26  & 0.00   & 171.93  & 6.25  \\ \cline{1-1} \cline{6-11} 
% adding parameter      &                        & 2     & 47    & 32                                                           & 43.47  & 43.47  & 61.48  & 0.00   & 86.94   & 4.17  \\ \cline{1-1} \cline{6-11} 
% enable cache          &                        & 2     &       &                                                              & 432.13 & 432.13 & 433.11 & 125.88 & 738.39  & 4.17  \\ \cline{1-1} \cline{6-11} 
% removing parameter    &                        & 2     &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 4.17  \\ \hline
% \end{tabular}
% \end{table}




\begin{table}[h]
\centering
\caption{Statistics of observed transitions, aggregated by target state} \amit{table 17: remove the things we are not using}
\scriptsize
\label{tab:rq3}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
From                 & To                   & Count & Total & Avg    & Med    & Std    & Min    & Max     & \%    \\ \hline
cache version update &                      & 378   &       & 70.60  & 0.00   & 149.79 & 0.00   & 713.59  & 51.85 \\ \cline{1-1} \cline{5-10} 
enable cache         &                      & 168   &       & 543.33 & 384.13 & 447.09 & 0.01   & 1615.93 & 23.05 \\ \cline{1-1} \cline{5-10} 
updating parameter   &                      & 104   &       & 172.52 & 104.80 & 241.06 & 0.00   & 1366.00 & 14.27 \\ \cline{1-1} \cline{5-10} 
adding cache         & cache version update & 44    & 745   & 298.89 & 231.83 & 310.83 & 0.00   & 1294.85 & 6.04  \\ \cline{1-1} \cline{5-10} 
removing cache       &                      & 18    &       & 210.66 & 95.11  & 334.78 & 0.00   & 1374.41 & 2.47  \\ \cline{1-1} \cline{5-10} 
adding parameter     &                      & 12    &       & 179.04 & 0.00   & 392.71 & 0.00   & 1366.00 & 1.65  \\ \cline{1-1} \cline{5-10} 
removing parameter   &                      & 5     &       & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 0.69  \\ \hline
updating parameter   &                      & 497   &       & 75.36  & 4.29   & 148.32 & 0.00   & 986.95  & 58.20 \\ \cline{1-1} \cline{5-10} 
enable cache         &                      & 166   &       & 207.31 & 115.90 & 260.34 & 0.00   & 981.44  & 19.44 \\ \cline{1-1} \cline{5-10} 
cache version update &                      & 92    &       & 95.24  & 0.23   & 136.98 & 0.00   & 592.69  & 10.77 \\ \cline{1-1} \cline{5-10} 
adding cache         & updating parameter   & 66    &       & 106.08 & 18.14  & 176.34 & 0.00   & 973.79  & 7.73  \\ \cline{1-1} \cline{5-10} 
removing cache       &                      & 23    & 854   & 59.31  & 14.83  & 132.34 & 0.00   & 584.88  & 2.69  \\ \cline{1-1} \cline{5-10} 
adding parameter     &                      & 8     &       & 100.00 & 3.23   & 220.22 & 0.00   & 628.32  & 0.94  \\ \cline{1-1} \cline{5-10} 
removing parameter   &                      & 2     &       & 117.53 & 117.53 & 166.21 & 0.00   & 235.06  & 0.23  \\ \hline
adding cache         &                      & 129   &       & 19.54  & 0.00   & 76.00  & 0.00   & 463.22  & 35.64 \\ \cline{1-1} \cline{5-10} 
removing cache       &                      & 80    &       & 49.43  & 0.00   & 121.76 & 0.00   & 538.67  & 22.10 \\ \cline{1-1} \cline{5-10} 
enable cache         &                      & 72    &       & 158.53 & 46.39  & 212.73 & 0.00   & 962.46  & 19.89 \\ \cline{1-1} \cline{5-10} 
updating parameter   & adding cache         & 39    & 362   & 70.13  & 10.86  & 153.92 & 0.00   & 903.97  & 10.77 \\ \cline{1-1} \cline{5-10} 
cache version update &                      & 18    &       & 54.97  & 16.83  & 96.33  & 0.00   & 380.01  & 4.97  \\ \cline{1-1} \cline{5-10} 
removing parameter   &                      & 14    &       & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 3.87  \\ \cline{1-1} \cline{5-10} 
adding parameter     &                      & 10    &       & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 2.76  \\ \hline
adding cache         &                      & 11    &       & 0.04   & 0.00   & 0.13   & 0.00   & 0.42    & 28.21 \\ \cline{1-1} \cline{5-10} 
updating parameter   &                      & 9     &       & 96.68  & 4.92   & 253.28 & 0.00   & 769.43  & 23.08 \\ \cline{1-1} \cline{5-10} 
cache version update &                      & 6     &       & 2.20   & 0.00   & 5.38   & 0.00   & 13.18   & 15.38 \\ \cline{1-1} \cline{5-10} 
enable cache         & adding parameter     & 5     & 39    & 1.01   & 0.00   & 2.27   & 0.00   & 5.07    & 12.82 \\ \cline{1-1} \cline{5-10} 
adding parameter     &                      & 4     &       & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 10.26 \\ \cline{1-1} \cline{5-10} 
removing cache       &                      & 3     &       & 57.74  & 0.00   & 100.02 & 0.00   & 173.23  & 7.69  \\ \cline{1-1} \cline{5-10} 
removing parameter   &                      & 1     &       & 94.21  & 94.21  & 0.00   & 94.21  & 94.21   & 2.56  \\ \hline
removing cache       &                      & 117   &       & 21.59  & 0.00   & 79.25  & 0.00   & 448.01  & 26.65 \\ \cline{1-1} \cline{5-10} 
enable cache         &                      & 111   &       & 293.62 & 129.68 & 362.73 & 0.00   & 1514.81 & 25.28 \\ \cline{1-1} \cline{5-10} 
adding cache         &                      & 76    &       & 110.33 & 4.25   & 167.29 & 0.00   & 750.21  & 17.31 \\ \cline{1-1} \cline{5-10} 
updating parameter   & removing cache       & 69    & 439   & 168.77 & 43.29  & 270.95 & 0.00   & 1154.81 & 15.72 \\ \cline{1-1} \cline{5-10} 
cache version update &                      & 45    &       & 201.85 & 125.65 & 205.24 & 0.00   & 707.67  & 10.25 \\ \cline{1-1} \cline{5-10} 
removing parameter   &                      & 20    &       & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 4.56  \\ \cline{1-1} \cline{5-10} 
adding parameter     &                      & 1     &       & 875.94 & 875.94 & 0.00   & 875.94 & 875.94  & 0.23  \\ \hline
removing cache       &                      & 26    &       & 7.36   & 0.00   & 37.52  & 0.00   & 191.32  & 54.17 \\ \cline{1-1} \cline{5-10} 
updating parameter   &                      & 10    &       & 16.26  & 7.07   & 24.39  & 0.00   & 70.85   & 20.83 \\ \cline{1-1} \cline{5-10} 
adding cache         &                      & 3     &       & 1.09   & 0.00   & 1.89   & 0.00   & 3.27    & 6.25  \\ \cline{1-1} \cline{5-10} 
cache version update & removing parameter   & 3     &       & 57.31  & 0.00   & 99.26  & 0.00   & 171.93  & 6.25  \\ \cline{1-1} \cline{5-10} 
adding parameter     &                      & 2     & 47    & 43.47  & 43.47  & 61.48  & 0.00   & 86.94   & 4.17  \\ \cline{1-1} \cline{5-10} 
enable cache         &                      & 2     &       & 432.13 & 432.13 & 433.11 & 125.88 & 738.39  & 4.17  \\ \cline{1-1} \cline{5-10} 
removing parameter   &                      & 2     &       & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 4.17  \\ \hline
\end{tabular}
\end{table}


\subsubsection{RQ3.2: What are the underlying drivers and triggers for cache modifications?} \yuan{isn't this RQ3?}

To understand the underlying drivers for the quantitative patterns observed in RQ 3.1, we first conduct a finer-grained qualitative analysis of what these changes represent. Section \ref{sec:background} defined the high level target states for our quantitative analysis. 

\yuan{cache modification actions, how it differs from table1's cache-related maintenance activities}
\yuan{is the below part methodology or results?}
\noindent \textbf{Taxonomy of Cache Modification Actions:} For RQ 3.2, we qualitatively analyzed these states and classified them into a fine-grained taxonomy of modification actions. Each category represents a specific intent or nature of modification within caching configurations. This taxonomy serves as bridge between the quantitative patterns of RQ 3.1 and the developer's underlying motivations.


\begin{itemize}
    \item \textbf{Update:} Refers to textual modifications within the caching configuration where developers adjust parameter names, paths, or cache keys without changing versions.\footnote{\url{https://github.com/lc-soft/LCUI/commit/8e06b4eb0524cd164aabb2501d858ddb5abb7f7b}} 
    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{code_examples/param_update.png}
        \caption{Example of an \textit{Update} action.}
        \label{fig:update_example}
    \end{figure}
    
    \item \textbf{Upgrade:} Represents incremental version updates within caching configurations, where developers move to a newer version of the caching action or \amit{remove the figures}dependency.\footnote{\url{https://github.com/cedricziel/idea-php-typo3-plugin/commit/bc692a59705d761bb85fc4c81f6c012c2c727508}}
    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{code_examples/upgrade.png}
        \caption{Example of an \textit{Upgrade} action.}
        \label{fig:upgrade_example}
    \end{figure}
    
    \item \textbf{Downgrade:} Occurs when developers revert to an older version within caching configurations, often to restore compatibility or resolve issues introduced by newer versions.\footnote{\url{https://github.com/pubkey/rxdb/commit/d01a87cc88c9ea72c712bf59f4340e09c7501d47}}
    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{code_examples/downgrade.png}
        \caption{Example of a \textit{Downgrade} action.}
        \label{fig:downgrade_example}
    \end{figure}
    
    \item \textbf{Add and Remove:} These actions capture the addition\footnote{https://github.com/storybookjs/react-inspector/commit/5aa36d10d4672f789674c8d4d5402ed366646b22} or removal\footnote{https://github.com/harveysimpsondata/ot-node/commit/bd23d94f83877a316fa9107ed87eeacff4fc4bb4} of caching configurations and their associated parameters. 

        \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{code_examples/add.png}
        \caption{Example of a \textit{Add} action.}
        \label{fig:add_example}
    \end{figure}

            \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{code_examples/remove.png}
        \caption{Example of a \textit{Remove} action.}
        \label{fig:remove_example}
    \end{figure}
\end{itemize}

Next, building upon these actions, we classified the underlying drivers ("why") and triggers ("who") for the changes. Table \ref{tab:caching-taxonomy} details this classification.

\noindent \textbf{Taxonomy of Change Drivers and Triggers:} \yuan{this is probably result rather than methodology} Building upon the change taxonomy, we developed a classification of the underlying drivers and initiators behind cache configuration modifications, as detailed in Table \ref{tab:caching-taxonomy}.

                                                            



\begin{table}[h]
\centering
\caption{Taxonomy of caching-related changes}
\tiny
\label{tab:caching-taxonomy}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Driver for \\ responding\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Trigger \\ Source\end{tabular}} & \textbf{Definition (D) - Example (E)}                                                                                                                                                          & \textbf{Freq.} \\ \hline
\begin{tabular}[c]{@{}l@{}}Update \\ dependencies\end{tabular}            & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers update, upgrade, downgrade dependencies of \\ caching configurations \\ E :  'Update Go dependencies'\end{tabular}                                   & 91             \\ \hline
\begin{tabular}[c]{@{}l@{}}Improve \\ cache\end{tabular}                  & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers perform changes in caching to \\ improve caching performance   \\ E :  improved github workflows\end{tabular}                                        & 47             \\ \hline
Bot alert                                                                 & Bots                                                               & \begin{tabular}[c]{@{}l@{}}D : Developers update dependency due to bot \\ alerts (dependabot, renovatebot etc)   \\ E :  Bump actions/cache from 4.0.0 to 4.0.2\end{tabular}                   & 40             \\ \hline
\begin{tabular}[c]{@{}l@{}}Extend \\ cache\end{tabular}                   & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers adds additional caching configuration in the yml file \\ for various reasons (add test, expand support etc)   \\ E :  use multiple jobs\end{tabular} & 28             \\ \hline
\begin{tabular}[c]{@{}l@{}}Fix caching \\ issues\end{tabular}             & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers address/fix issues related to caching.    \\ E :  Fix cmake.yml cache issues\end{tabular}                                                            & 23             \\ \hline
Migration                                                                 & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers migrate to different workflow (such as pnpm)   \\ E :  migrate to pnpm\end{tabular}                                                                  & 14             \\ \hline
Clean up                                                                  & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers cleanup,reconfigure, refactor yml files   \\ E :  Simplify pipeline\end{tabular}                                                                     & 14             \\ \hline
Remove tests                                                              & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers removes specific job/test after a specific period of time  \\ E :  Remove legacy tests and style guide\end{tabular}                                  & 13             \\ \hline
\begin{tabular}[c]{@{}l@{}}Fix security \\ issues\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Human \&\\  Bot\end{tabular}            & \begin{tabular}[c]{@{}l@{}}D : Developers address security concerns by updating the \\ caching configurations triggered by human and bots   \\ E :  ci: Harden GitHub Actions\end{tabular}     & 6              \\ \hline
Disable cache                                                             & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Developers disable caching  \\ E :  Removed caching of compiled contracts\end{tabular}                                                                          & 4              \\ \hline
\begin{tabular}[c]{@{}l@{}}Fix deprecated \\ versions\end{tabular}        & Human                                                              & \begin{tabular}[c]{@{}l@{}}D : Fixing nearly deprecated version/addressing warning    \\ E :  Change GitHub Action version to address deprecation\end{tabular}                                 & 2              \\ \hline
Other                                                                     & -                                                                  & Reason not stated or unclear in commit/PR.                                                                                                                                                     & 107            \\ \hline
\end{tabular}
\end{table}







% \safwat{change the CI to 90 from 95 and 10 of margin of error. >> this will reduce the samples a lot and help to label. cite the paper .  add the unique commit number in the description when we describe the table.}

% \begin{table}[h]
% \centering
% \caption{Statistics of observed transitions, aggregated by target state}
% \scriptsize
% \label{tab:rq3}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% From                   & To                     & Count & Total & \begin{tabular}[c]{@{}c@{}}Significant\\ sample\end{tabular} & Avg    & Med    & Std    & Min    & Max     & \%    \\ \hline
% cache\_version\_update &                        & 378   &       &                                                              & 70.60  & 0.00   & 149.79 & 0.00   & 713.59  & 51.85 \\ \cline{1-1} \cline{6-11} 
% enable\_cache          &                        & 168   &       &                                                              & 543.33 & 384.13 & 447.09 & 0.01   & 1615.93 & 23.05 \\ \cline{1-1} \cline{6-11} 
% updating\_parameter    &                        & 104   &       &                                                              & 172.52 & 104.80 & 241.06 & 0.00   & 1366.00 & 14.27 \\ \cline{1-1} \cline{6-11} 
% adding\_cache          & cache\_version\_update & 44    & 745   & 86                                                          & 298.89 & 231.83 & 310.83 & 0.00   & 1294.85 & 6.04  \\ \cline{1-1} \cline{6-11} 
% removing\_cache        &                        & 18    &       &                                                              & 210.66 & 95.11  & 334.78 & 0.00   & 1374.41 & 2.47  \\ \cline{1-1} \cline{6-11} 
% adding\_parameter      &                        & 12    &       &                                                              & 179.04 & 0.00   & 392.71 & 0.00   & 1366.00 & 1.65  \\ \cline{1-1} \cline{6-11} 
% removing\_parameter    &                        & 5     &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 0.69  \\ \hline
% updating\_parameter    &                        & 497   &       &                                                              & 75.36  & 4.29   & 148.32 & 0.00   & 986.95  & 58.20 \\ \cline{1-1} \cline{6-11} 
% enable\_cache          &                        & 166   &       &                                                              & 207.31 & 115.90 & 260.34 & 0.00   & 981.44  & 19.44 \\ \cline{1-1} \cline{6-11} 
% cache\_version\_update &                        & 92    &       &                                                              & 95.24  & 0.23   & 136.98 & 0.00   & 592.69  & 10.77 \\ \cline{1-1} \cline{6-11} 
% adding\_cache          & updating\_parameter    & 66    &       &                                                              & 106.08 & 18.14  & 176.34 & 0.00   & 973.79  & 7.73  \\ \cline{1-1} \cline{6-11} 
% removing\_cache        &                        & 23    & 854   & 87                                                          & 59.31  & 14.83  & 132.34 & 0.00   & 584.88  & 2.69  \\ \cline{1-1} \cline{6-11} 
% adding\_parameter      &                        & 8     &       &                                                              & 100.00 & 3.23   & 220.22 & 0.00   & 628.32  & 0.94  \\ \cline{1-1} \cline{6-11} 
% removing\_parameter    &                        & 2     &       &                                                              & 117.53 & 117.53 & 166.21 & 0.00   & 235.06  & 0.23  \\ \hline
% adding\_cache          &                        & 129   &       &                                                              & 19.54  & 0.00   & 76.00  & 0.00   & 463.22  & 35.64 \\ \cline{1-1} \cline{6-11} 
% removing\_cache        &                        & 80    &       &                                                              & 49.43  & 0.00   & 121.76 & 0.00   & 538.67  & 22.10 \\ \cline{1-1} \cline{6-11} 
% enable\_cache          &                        & 72    &       &                                                              & 158.53 & 46.39  & 212.73 & 0.00   & 962.46  & 19.89 \\ \cline{1-1} \cline{6-11} 
% updating\_parameter    & adding\_cache          & 39    & 362   & 77                                                          & 70.13  & 10.86  & 153.92 & 0.00   & 903.97  & 10.77 \\ \cline{1-1} \cline{6-11} 
% cache\_version\_update &                        & 18    &       &                                                              & 54.97  & 16.83  & 96.33  & 0.00   & 380.01  & 4.97  \\ \cline{1-1} \cline{6-11} 
% removing\_parameter    &                        & 14    &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 3.87  \\ \cline{1-1} \cline{6-11} 
% adding\_parameter      &                        & 10    &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 2.76  \\ \hline
% adding\_cache          &                        & 11    &       &                                                              & 0.04   & 0.00   & 0.13   & 0.00   & 0.42    & 28.21 \\ \cline{1-1} \cline{6-11} 
% updating\_parameter    &                        & 9     &       &                                                              & 96.68  & 4.92   & 253.28 & 0.00   & 769.43  & 23.08 \\ \cline{1-1} \cline{6-11} 
% cache\_version\_update &                        & 6     &       &                                                              & 2.20   & 0.00   & 5.38   & 0.00   & 13.18   & 15.38 \\ \cline{1-1} \cline{6-11} 
% enable\_cache          & adding\_parameter      & 5     & 39    & 28                                                           & 1.01   & 0.00   & 2.27   & 0.00   & 5.07    & 12.82 \\ \cline{1-1} \cline{6-11} 
% adding\_parameter      &                        & 4     &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 10.26 \\ \cline{1-1} \cline{6-11} 
% removing\_cache        &                        & 3     &       &                                                              & 57.74  & 0.00   & 100.02 & 0.00   & 173.23  & 7.69  \\ \cline{1-1} \cline{6-11} 
% removing\_parameter    &                        & 1     &       &                                                              & 94.21  & 94.21  & NaN    & 94.21  & 94.21   & 2.56  \\ \hline
% removing\_cache        &                        & 117   &       &                                                              & 21.59  & 0.00   & 79.25  & 0.00   & 448.01  & 26.65 \\ \cline{1-1} \cline{6-11} 
% enable\_cache          &                        & 111   &       &                                                              & 293.62 & 129.68 & 362.73 & 0.00   & 1514.81 & 25.28 \\ \cline{1-1} \cline{6-11} 
% adding\_cache          &                        & 76    &       &                                                              & 110.33 & 4.25   & 167.29 & 0.00   & 750.21  & 17.31 \\ \cline{1-1} \cline{6-11} 
% updating\_parameter    & removing\_cache        & 69    & 439   & 79                                                          & 168.77 & 43.29  & 270.95 & 0.00   & 1154.81 & 15.72 \\ \cline{1-1} \cline{6-11} 
% cache\_version\_update &                        & 45    &       &                                                              & 201.85 & 125.65 & 205.24 & 0.00   & 707.67  & 10.25 \\ \cline{1-1} \cline{6-11} 
% removing\_parameter    &                        & 20    &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 4.56  \\ \cline{1-1} \cline{6-11} 
% adding\_parameter      &                        & 1     &       &                                                              & 875.94 & 875.94 & NaN    & 875.94 & 875.94  & 0.23  \\ \hline
% removing\_cache        &                        & 26    &       &                                                              & 7.36   & 0.00   & 37.52  & 0.00   & 191.32  & 54.17 \\ \cline{1-1} \cline{6-11} 
% updating\_parameter    &                        & 10    &       &                                                              & 16.26  & 7.07   & 24.39  & 0.00   & 70.85   & 20.83 \\ \cline{1-1} \cline{6-11} 
% adding\_cache          &                        & 3     &       &                                                              & 1.09   & 0.00   & 1.89   & 0.00   & 3.27    & 6.25  \\ \cline{1-1} \cline{6-11} 
% cache\_version\_update & removing\_parameter    & 3     &       &                                                              & 57.31  & 0.00   & 99.26  & 0.00   & 171.93  & 6.25  \\ \cline{1-1} \cline{6-11} 
% adding\_parameter      &                        & 2     & 47    & 32                                                           & 43.47  & 43.47  & 61.48  & 0.00   & 86.94   & 4.17  \\ \cline{1-1} \cline{6-11} 
% enable\_cache          &                        & 2     &       &                                                              & 432.13 & 432.13 & 433.11 & 125.88 & 738.39  & 4.17  \\ \cline{1-1} \cline{6-11} 
% removing\_parameter    &                        & 2     &       &                                                              & 0.00   & 0.00   & 0.00   & 0.00   & 0.00    & 4.17  \\ \hline
% \end{tabular}
% \end{table}



\subsubsection{Cross Sub-RQ Findings} 
\yuan{a bit lost in the logic for answering RQ3 and purpose of different taxonomies}
\yuan{i feel below are real results of RQ3}
We now connect the quantitative targets (from RQ3.1) with the qualitative drivers (from RQ3.2). Table \ref{tab:rq3_table_1} maps the target states to the specific modification action and the underlying driver. The Other category (N=107) is excluded from this specific analysis, as its high frequency is due to commit messages lacking clear rationale and it provides no insight into specific drivers.




\begin{table}[h]
\centering
\caption{Summary of caching change targets, extended actions, and underlying reasons.}
\label{tab:rq3_table_1}
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|c|}
\hline
\textbf{Target} & \textbf{Modification} & \textbf{Drivers} & \textbf{Total} \\ \hline

\multirow{3}{*}{\textbf{Cache version update}} 
 & Update   & Fix security issues (1) & 1 \\ \cline{2-4}
 & Upgrade  & \begin{tabular}[c]{@{}l@{}}Update dependencies (41)\\ Bot alert (40)\\ Fix deprecated versions (2)\\ Other (1)\end{tabular} & 84 \\ \cline{2-4}
 & Downgrade& Update dependencies (1) & 1 \\ \hline

\multirow{3}{*}{\textbf{Parameter update}} 
 & Update   & \begin{tabular}[c]{@{}l@{}}Fix caching issues (9)\\ Update dependencies (7)\\ Improve cache (1)\\ Fix security issues (1)\\ Migration (1)\\ Other (22)\end{tabular} & 41 \\ \cline{2-4}
 & Upgrade  & \begin{tabular}[c]{@{}l@{}}Update dependencies (35)\\ Fix caching issues (5)\\ Fix security issues (1)\\ Clean up (1)\\ Other (1)\end{tabular} & 43 \\ \cline{2-4}
 & Downgrade& \begin{tabular}[c]{@{}l@{}}Fix deprecated versions (2)\\ Update dependencies (1)\end{tabular} & 3 \\ \hline

\textbf{Adding cache} 
 & Add      & \begin{tabular}[c]{@{}l@{}}Extend cache (28)\\ Improve cache (17)\\ Fix caching issues (4)\\ Fix security issues (3)\\ Migration (2)\\ Other (23)\end{tabular} & 77 \\ \hline

\textbf{Removing cache} 
 & Remove   & \begin{tabular}[c]{@{}l@{}}Improve cache (14)\\ Remove tests (13)\\ Clean up (10)\\ Migration (4)\\ Disable cache (4)\\ Fix caching issues (1)\\ Other (33)\end{tabular} & 79 \\ \hline

\textbf{Adding parameter} 
 & Add      & \begin{tabular}[c]{@{}l@{}}Improve cache (12)\\ Update dependencies (4)\\ Fix caching issues (2)\\ Migration (2)\\ Clean up (1)\\ Other (7)\end{tabular} & 28 \\ \hline

\textbf{Removing parameter} 
 & Remove   & \begin{tabular}[c]{@{}l@{}}Migration (5)\\ Update dependencies (2)\\ Clean up (2)\\ Improve cache (1)\\ Other (22)\end{tabular} & 32 \\ \hline

\end{tabular}
}
\end{table}







\begin{table}[h]
\caption{Distribution of Modification Actions by Driver\yuan{put the row other at the end}} \amit{how we interpret this, move the row to 2nd colmun,  }
\tiny
\label{tab:my-table}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Categories}                                                & \textbf{\begin{tabular}[c]{@{}c@{}}Adding\\ Cache\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Adding\\ Parameter\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Cache \\ Version\\ Update\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Removing\\ Cache\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Removing\\ Parameter\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Parameter\\ Update\end{tabular}} & \textbf{Total} \\ \hline
Other                                                              & 23 (21.5\%)                                                     & 7 (6.5\%)                                                           & 1 (0.9\%)                                                                  & 33 (30.8\%)                                                       & 22 (20.6\%)                                                           & 21 (19.6\%)                                                         & 107            \\ \hline
\begin{tabular}[c]{@{}c@{}}Update \\ dependencies\end{tabular}     & 0 (0.0\%)                                                       & 4 (4.4\%)                                                           & 42 (46.2\%)                                                                & 0 (0.0\%)                                                         & 2 (2.2\%)                                                             & 43 (47.3\%)                                                         & 91             \\ \hline
\begin{tabular}[c]{@{}c@{}}Improve \\ cache\end{tabular}           & 17 (36.2\%)                                                     & 12 (25.5\%)                                                         & 0 (0.0\%)                                                                  & 14 (29.8\%)                                                       & 1 (2.1\%)                                                             & 3 (6.4\%)                                                           & 47             \\ \hline
\begin{tabular}[c]{@{}c@{}}Bot \\ alert\end{tabular}               & 0 (0.0\%)                                                       & 0 (0.0\%)                                                           & 40 (100.0\%)                                                               & 0 (0.0\%)                                                         & 0 (0.0\%)                                                             & 0 (0.0\%)                                                           & 40             \\ \hline
\begin{tabular}[c]{@{}c@{}}Extend \\ cache\end{tabular}            & 28 (100.0\%)                                                    & 0 (0.0\%)                                                           & 0 (0.0\%)                                                                  & 0 (0.0\%)                                                         & 0 (0.0\%)                                                             & 0 (0.0\%)                                                           & 28             \\ \hline
\begin{tabular}[c]{@{}c@{}}Fix caching\\ issues\end{tabular}       & 4 (17.4\%)                                                      & 2 (8.7\%)                                                           & 0 (0.0\%)                                                                  & 1 (4.3\%)                                                         & 0 (0.0\%)                                                             & 16 (69.6\%)                                                         & 23             \\ \hline
\begin{tabular}[c]{@{}c@{}}Clean \\ up\end{tabular}                & 0 (0.0\%)                                                       & 1 (7.1\%)                                                           & 0 (0.0\%)                                                                  & 10 (71.4\%)                                                       & 2 (14.3\%)                                                            & 1 (7.1\%)                                                           & 14             \\ \hline
Migration                                                          & 2 (14.3\%)                                                      & 2 (14.3\%)                                                          & 0 (0.0\%)                                                                  & 4 (28.6\%)                                                        & 5 (35.7\%)                                                            & 1 (7.1\%)                                                           & 14             \\ \hline
\begin{tabular}[c]{@{}c@{}}Remove \\ tests\end{tabular}            & 0 (0.0\%)                                                       & 0 (0.0\%)                                                           & 0 (0.0\%)                                                                  & 13 (100.0\%)                                                      & 0 (0.0\%)                                                             & 0 (0.0\%)                                                           & 13             \\ \hline
\begin{tabular}[c]{@{}c@{}}Fix security \\ issues\end{tabular}     & 3 (50.0\%)                                                      & 0 (0.0\%)                                                           & 1 (16.7\%)                                                                 & 0 (0.0\%)                                                         & 0 (0.0\%)                                                             & 2 (33.3\%)                                                          & 6              \\ \hline
\begin{tabular}[c]{@{}c@{}}Disable \\ cache\end{tabular}           & 0 (0.0\%)                                                       & 0 (0.0\%)                                                           & 0 (0.0\%)                                                                  & 4 (100.0\%)                                                       & 0 (0.0\%)                                                             & 0 (0.0\%)                                                           & 4              \\ \hline
\begin{tabular}[c]{@{}c@{}}Fix deprecated \\ versions\end{tabular} & 0 (0.0\%)                                                       & 0 (0.0\%)                                                           & 2 (100.0\%)                                                                & 0 (0.0\%)                                                         & 0 (0.0\%)                                                             & 0 (0.0\%)                                                           & 2              \\ \hline
\end{tabular}
\end{table}


\noindent \textbf{Finding 1: The most frequent cache activity, parameter updating, is fast and human-driven.} RQ2 and RQ3.1 findings show a dominant, high-frequency loop of P\_up $\rightarrow$ P\_up (N=497), with a rapid median of 4.29 days (Table \ref{tab:rq3}). Table \ref{tab:rq3_table_1} reveals that this action is overwhelmingly driven by humans, not bots. The primary drivers are updating dependency (N=43) and, critically, fixing caching issues (N=16). In fact, as shown in Table \ref{tab:my-table}, when a developer's intent is to Fix caching issues, their corrective action is up\_param in 69.6\% of cases. This reframes the "rapid iteration" seen in RQ2. It is not just fine-tuning, but a reactive, trial-and-error debugging cycle.

\smallskip


\noindent \textbf{Finding 2: Cache version updates are not performance driven optimizations but long-term, dependency maintenance, triggered by bots and humans.} Along with fast parameter updates, RQ2 showed that version updates (EC $\rightarrow$ C\_up) are "long-delayed actions." Table \ref{tab:rq3} confirms this, showing the median time from enable cache to the first cache version update is a very long 384.13 days. Table \ref{tab:rq3_table_1} explains this delay as the cache version update action (N=86 samples) is almost exclusively an Upgrade (N=84). The drivers for this upgrade are split between human-led updating dependency (N=41) and automated bot alert (N=40). This evidence indicates that developers tend to stay in their initial cache versions. Also, while bots ensure dependency currency, humans retain responsibility for complex version management decisions.

\smallskip


\noindent \textbf{Finding 3: Bots are exclusively focused on version maintenance, leaving all cognitive work of optimization and debugging to humans.} Table \ref{tab:my-table} shows that 100\% of all changes driven by Bot alert (N=40) target cache version update. Bots are entirely absent from all other, more complex cache management tasks. All actions related to Improve cache (N=47), Fix caching issues (N=23), Extend cache (N=28), and Clean up (N=14) are performed by humans. This highlights a significant gap where automation only handles the simplest task (version bumping) and provides no support for the more critical, performance-oriented, or corrective actions. We also noticed presence of security bot which informs developers when there's a vulnerability in used caching configurations.
\smallskip


\noindent \textbf{Finding 4: Cache removal shows two distinct  patterns.} RQ2 noted that cache removals happen at different cadences. Our RQ3 findings confirms and explains both behaviors. Table \ref{tab:rq3} shows the transition adding cache $\rightarrow$ removing cache has a median of just 4.25 days. This is often driven by improve cache (N=14, Table \ref{tab:rq3_table_1}), indicating a clear picture of a failed optimization: a developer adds a cache, it proves ineffective, and it is removed almost immediately.

In contrast, the enable cache $\rightarrow$ removing cache transition (N=111) has a median of 129.68 days. The drivers here are not just about failed caching. As Table \ref{tab:rq3_table_1} shows, this is a collection of several important rationales. The most common drivers are remove test (N=13) and clean up (N=10), indicating caches are removed as a side-effect of deleting the CI/CD jobs they supported. Disable cache (N=4) is an important driver, where developers explicitly remove a cache that is no longer deemed beneficial or may be causing persistent instability. We also see migration (N=4) as a key driver, where caches for old build systems (e.g., npm) are removed as part of a move to a new system (e.g., pnpm).
\smallskip




\noindent \textbf{Finding 5: Adding a cache is a proactive, human-led strategy for functional expansion and optimization.} Adding cache (N=362) is a deliberate, intentional act. Table \ref{tab:rq3_table_1} shows this action is driven by three distinct, non-maintenance-related rationales. Extending cache (N=28) s the most common driver. It represents a major functional addition to the CI pipeline, such as adding an entirely new job (e.g., a new test suite, a security scanner, or a new build variant) that requires its own cache to be effective. Improving cache (N= 17) which is a proactive optimization step where developers add an additional cache to an existing job. Less dominant but important migration (N=2), when developers migrate their build system (e.g., from npm to pnpm, or changing package managers), they must add new cache configurations tailored to the new tooling's dependencies and file structures. This aligns with RQ2's finding that EC $\rightarrow$ C\_add happens relatively quickly in build/test phases (medians of 40-55 days), as developers actively refine their pipelines after initial setup.


\smallskip


\noindent \textbf{Finding 6: Security is a minor but important driver for cache changes, addressed through multiple different actions.} While infrequent (N=6, Table \ref{tab:caching-taxonomy}), the Fix security issues driver is not addressed by a single action. As Table \ref{tab:my-table} shows, developers respond by adding cache (N=3, 50.0\%), up\_param (N=2, 33.3\%), and cache version update (N=1, 16.7\%). This suggests that security hardening in CI/CD caching is a nuanced process, potentially involving adding new scanner caches, reconfiguring parameters, or updating to a patched version.
\smallskip

\noindent \textbf{Finding 7: Cache downgrades are a rare but critical reactive tactic.} While Upgrade actions dominate version changes (N=84), our sample captured 4 instances of a downgrade (Table \ref{tab:rq3_table_1}). These actions were split between targeting cache version update (N=1) and updating parameter (N=3) and were driven by update dependency (N=2) and fixing deprecated versions (N=2). This finding is crucial because it represents the "failure" mode of the maintenance cycle. It directly contradicts the Bot alert logic (Finding 3), which assumes upgrades are always safe. A bot or human performs an upgrade, that change breaks the build or introduces an error (as exemplified in Figure \ref{fig:downgrade_example}), and a human developer must then spend time debugging and manually reverting the change. This downgrade is a clear, data-backed example of a reactive, human-led fix to a problem likely introduced by automated or manual dependency maintenance. 




% \safwat{exclude others and put some explanation in the text. Sort the table 18. Change why to driver. Make the description improved. Think about the naming.  }

\begin{tcolorbox}[enhanced,width=4.7in,size=fbox,drop shadow southwest,sharp corners]

\textbf{RQ3 Summary: Our analysis reveals that humans perform all complex debugging and optimization, while bots only handle simple version updates. The most frequent change, parameter updating, is not an optimization planned in advance but is driven by humans fixing problems (fixing caching issues) on a rapid 4.29 day median. In contrast, version updates occur infrequently (384.13 day median), triggered by either human-led dependency checks or bot alerts. Cache removal is either a rapid 4.25 day reversal of a failed optimization or a slow 129.68 day removal driven by pipeline refactoring. Finally, rare downgrade actions (N=4) show humans must manually recover from failed automated upgrades.} 

\end{tcolorbox}




